Measurement of the $WW+WZ$ cross section and limits on anomalous triple gauge couplings using final states with one lepton, missing transverse momentum, and two jets with the ATLAS detector at $\sqrt{\rm{s}} = 7$ TeV

The production of a $W$ boson decaying to $e\nu$ or $\mu\nu$ in association with a $W$ or $Z$ boson decaying to two jets is studied using $4.6 \mathrm{fb}^{-1}$ of proton--proton collision data at $\sqrt{\rm{s}} = 7$ TeV recorded with the ATLAS detector at the LHC. The combined $WW+WZ$ cross section is measured with a significance of 3.4$\sigma$ and is found to be $68 \pm 7 \ \mathrm{(stat.)} \pm 19 \ \mathrm{(syst.)} \ pb$, in agreement with the Standard Model expectation of $61.1 \pm 2.2 \ \mathrm{pb}$. The distribution of the transverse momentum of the dijet system is used to set limits on anomalous contributions to the triple gauge coupling vertices and on parameters of an effective-field-theory model.

==> AnalysisStrategy.tex <==

Candidate  $\WVtolvjj$ events are required to contain exactly one lepton (electron or muon),
large missing transverse momentum $\MET$, and exactly two jets. The selected events are accepted 
if they pass a set of kinematic cuts chosen  
to enhance the signal-to-background ratio. The invariant mass distribution of 
the two jets ($\Mjj$), representing the candidate decay products of the hadronically 
decaying boson, is obtained from all the selected events. The  $WW+WZ$ signal yield ($N^{WV}$) is
obtained by performing a binned maximum-likelihood fit 
to the $\Mjj$ distribution using templates based on MC simulations. The fit is performed on events in an $\Mjj$ range much larger than the range where the signal peaks, allowing the nearly signal-free $\Mjj$ regions to constrain the rate of the $\Wjet$ events, which are the largest background. Because of the finite dijet mass resolution, there is considerable overlap between the $\Mjj$ peaks from $\WWtolvqq$ and $\WZtolvqq$ decays.  Given the expected uncertainties in this measurement,
and the relatively small contribution from the $WZ$ process (about 20\% of the total
signal yield), no attempt is made to distinguish between the $WW$ and $WZ$ contributions in this 
analysis. Instead, the signal yield is obtained under the assumption 
that the ratio of the $WW$ and $WZ$ cross sections is equal to the SM prediction.

The fiducial cross section ($\sigmafid$) is evaluated from the measured signal yield.
The fiducial phase space is defined to be as close as possible to the phase space defined by the reconstructed event selection.
The fiducial cross-section measurement is obtained as:
\begin{eqnarray}
\label{eq:simple1}
\sigmafid  = \sum_{\ell=e,\mu} \frac{N^{WV}_{\ell}}{\Lumi \cdot \Dfid{_{,\ell}}}\,,
\end{eqnarray}
where \Lumi~is the integrated luminosity and $\Dfid{_{,\ell}}$ are 
factors that correct for the difference between the number of
$\WVtolvjj$ events produced
in the fiducial phase space and the number of reconstructed events passing
the event selection.
The total cross section ($\sigmatot$) is obtained by extrapolating the 
fiducial cross section to the full phase space using theoretical predictions:  
\begin{eqnarray}
\label{eq:simple3}
\sigmatot  =  \sum_{\ell=e,\mu} \frac{N^{WV}_{\ell}} {\Lumi \cdot \Dtot{_{,\ell}}},
\end{eqnarray}
where $\Dtot{_{,\ell}}$ are factors that depend on acceptances,
reconstruction efficiencies, and the branching fractions for $\WWtolvjj$ and $\WZtolvjj$.
Details of the maximum-likelihood fit and the precise definition of the fiducial-volume 
and of the factors $\Dfid{_{,\ell}}$ and $\Dtot{_{,\ell}}$ are given 
in section~\ref{sec:xsecAndFitMethod}.

Lastly, the transverse momentum distribution of the hadronically decaying $V$ 
candidates ($\pTjj$) is used to set limits on the aTGCs affecting 
the $WWZ$ and $WW\gamma$ vertices. The event selection is the same as
the one used for the cross-section measurement, except that the dijet mass is 
required to be close to the masses of the $W/Z$ bosons in order to 
increase the signal-to-background 
ratio.  The aTGC limits are calculated 
by performing a binned maximum-likelihood fit to the $\pTjj$ distributions. 
The ratio of the $WW$ and $WZ$ cross sections at each aTGC point is 
assumed to be that predicted by theory, including the aTGC contribution.
Details of the limit extraction are given in section~\ref{sec:atgc}. 


==> AnomalousCouplings.tex <==
The measured $WV$ cross section agrees well with the SM predictions; 
in this section limits are set on anomalous triple gauge couplings affecting
the $WWZ$ and $WW\gamma$ vertices.
Anomalous couplings tend to enhance the diboson cross section at high
boson $\pT$.  Limits  on the anomalous couplings are set by
fitting the distribution of the transverse momentum of the reconstructed hadronically decaying $V$, $\pTjj$.
The event selection is the same as used for the cross-section measurement, except
that $\Mjj$ is additionally required to be between 75 and 95 $\gev$ to improve
the signal-to-background ratio. The $\Mjj$ range and the binning of the $\pTjj$ histogram are chosen to optimise the expected aTGC limits. 


To quantify possible deviations from the SM affecting triple gauge
boson vertices, the couplings of the $WWZ$ and $WW\gamma$ vertices are described 
in terms of five dimensionless parameters: $\lambdag$, $\lambdaz$, $\kg$, $\kz$, and
$\gz$, only considering couplings that conserve $C$ and $P$ and satisfy electromagnetic gauge 
invariance~\cite{Hagiwara:1986vm}.  No form factors are applied to these parameters
in this analysis.
 In the SM, $\lambdag=\lambdaz=0$, and $\kg=\kz=\gz=1$.
Various assumptions can be made to decrease the number of
free parameters. In this analysis, limits are given using the so-called LEP scenario~\cite{altarelli1996physics} in which the following additional 
constraints, derived from $SU(2)\times U(1)$ gauge invariance, are imposed:
\begin{eqnarray}
\lambdag & = & \lambdaz \equiv \lambda\,, \\
\dkz     & = & \dgz - \dkg {\rm tan}^2 \theta_{\rm w}\,,
\end{eqnarray}
where $\dkg \equiv \kg - 1$,  $\dkz\equiv \kz - 1$, and  $\dgz \equiv \gz - 1$.   
In this scenario, there are three
free parameters: $\lambda$, $\dkg$, and $\dgz$.  

An alternative approach to the aTGC parametrisation 
describes deviations from the SM in terms of an effective-field-theory (EFT), valid 
only up to some mass scale $\Lambda$.  This EFT~\cite{HISZ:1993,Degrande:2012wf} contains three 
$C$- and $P$-conserving dimension-6 operators. The coefficients of these operators
are denoted by $\cwp$, $\cbp$, and $\cwwwp$, and can be related 
to the LEP-scenario parameters by the following equations: 
\begin{eqnarray}
\cwf & = & \frac{2}{m_Z^2}\dgz\,, \\
\cbf & = & \frac{2}{m_W^2}\dkg  - \frac{2}{m_Z^2}\dgz\,, \\ 
\cwwwf & = &  \frac{2}{3 g^2 m_W^2} \lambda\,,
\end{eqnarray}
where $g$ is the electroweak coupling constant.


The diboson signal with anomalous couplings is modeled using 
the same generator (\mcatnlo+\herwig) as for the SM signal.
The dijet $\pT$ distribution is shown in figure~\ref{fig:DataVsMCaTGC} for data and MC simulation, 
along with the signal prediction for an aTGC of $\lambda=0.05$.
%
\begin{figure}[hp]
\begin{center}
\subfigure[]{
 \label{subfig:pTjjElec}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{pTjj_dataMC_aTGC_elec.pdf}
}
\subfigure[]{
  \label{subfig:pTjjMuon}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{pTjj_dataMC_aTGC_muon.pdf}
}
\caption{
The observed distribution of the transverse momentum of the two jets, compared to the expectation for SM signal plus
background, for (a) the electron channel and (b) the
muon channel. 
The error bars represent statistical uncertainties, 
and the stacked histograms are background and signal predictions as described in the legend.
The effect of an aTGC of
$\lambdaz=\lambdag=0.05$ is shown for comparison (white histogram) on top of the SM predictions (coloured histograms). 
 The rightmost bin includes overflow.
The bottom panels show the ratio between the data and the SM prediction overlaid
with the systematic uncertainty on the shape of the $\pTjj$ distribution.  The binning in the plots is
the same as that one used to perform the calculation of the limits. The red vertical line indicates
that the event selection is different for \pTjj\ less than and greater than 250~\gev, as described
in section~\ref{sec:EventSelection}.
}
\label{fig:DataVsMCaTGC}
\end{center}
\end{figure}
The limits on the anomalous couplings are calculated by performing a binned maximum-likelihood fit to the
$\pTjj$ spectrum. To determine whether a point $\vec{\alpha}$ in 
the anomalous coupling parameter space is excluded by the data, the likelihood
ratio $\lkl(\vec{\alpha})/\lkl(\vec{\alpha}_{\rm max})$ is computed, 
where $\vec{\alpha}_{\rm max}$
is the value of the anomalous coupling(s) that maximizes the likelihood.
Then the probability of observing such a small likelihood ratio is determined
through pseudo-experiments, in which pseudo-data are generated by randomly
sampling the probability density function.  Systematic uncertainties are 
incorporated in the fit via nuisance parameters which affect the rates and $\pTjj$ distribution shapes of
the signal and background processes.  The same sources of systematic uncertainty
are included as are described for the $\Mjj$ fit in section~\ref{sec:sys},
except for those found to be negligible, such as the effect of PDF uncertainties on 
the signal.
In addition, an uncertainty is included
 on the $\pTjj$ distribution shape of the signal due to increasing and decreasing the scales 
by a factor of two.  The factorisation and renormalisation scales are 
varied simultaneously by the same amount.
As can be seen in figure~\ref{fig:DataVsMCaTGC}, at very high $\pTjj$ the statistical 
uncertainties dominate, whereas at lower values of $\pTjj$ the systematic uncertainties
are more important.  

The  expected and observed 95\% CL limits 
for $\lambda$, $\dkg$, and $\dgz$ in the LEP scenario are given in table~\ref{tab:aTGC_LEP}.
 If there were no systematic uncertainties at all, the expected aTGC limits would improve by about 25\%.

\begin{table}
  \begin{center}
  \caption{The observed and expected 95\% CL limits on the anomalous triple gauge coupling parameters $\lambda$, $\dkg$, and $\dgz$ in the LEP scenario
with no form factor applied. 
The limits on each parameter are calculated while fixing the other two parameters to zero.}
\label{tab:aTGC_LEP}
\begin{tabular}{lcc}
  \hline \hline
Parameter   &  Observed Limit & Expected Limit  \\
\hline
\lambdaz = \lambdag & [$-0.039$, 0.040] &  [$-0.048$, 0.047]\\
\dkg & [$-0.21$, 0.22] & [$-0.23$, 0.25] \\
\dgz & [$-0.055$, 0.071] &  [$-0.072$, 0.085] \\
\hline  \hline
\end{tabular}
\end{center}
\end{table}

In figure~\ref{fig:aTGCcompare}, the observed limits are compared with previous limits from 
ATLAS~\cite{ATLAS:2012mec,Aad:2012twa,Aad:2013izg}, CMS~\cite{Chatrchyan:2013yaa,Chatrchyan:2012bd,Chatrchyan:2013fya},
D0~\cite{Abazov:2012ze}, and LEP~\cite{Schael:2013ita}, in a variety of channels including
$WW\to\ell\nu\ell\nu$, $WZ\to\ell\nu\ell\ell$, $\WVtolvjj$, and $W\gamma\to\ell\nu\gamma$. 
All limits are given at 95\% CL, and calculated within the LEP scenario.  
The form factor $\Lambda_{\rm FF}$ used for each limit calculation is specified on the figure~\ref{fig:aTGCcompare};
$\Lambda_{\rm FF}=\infty$ is equivalent to no form factor. The limits for each parameter are obtained while fixing the other two parameters to zero.  
In the CMS $\lvjj$ analysis and the in ATLAS and CMS $W\gamma$ analyses, no limits on
$\dgz$ were given.  The ATLAS $WW$ and $WZ$ analyses gave limits on $\dgz$, but 
with $\dkz=0$ rather than $\dkg=0$, so they are not comparable with these results
and are thus excluded.  For the ATLAS $WW$ result, the published limits
on $\dkz$ are converted to limits on $\dkg$ using the 
formula $\dkz = - \dkg {\rm tan}^2 \theta_{\rm w}$.
The ATLAS $WZ$ analysis published limits on $\dkz$, which can also be converted
to $\dkg$, but those limits are not shown, since they are much larger than 
the other limits in this figure.
\begin{figure}[h!]
\begin{center}
 \includegraphics[width=0.8\textwidth,keepaspectratio]{aTGCcomparison2.pdf}
\caption{
Comparison of limits on anomalous triple gauge coupling parameters obtained in this analysis with limits quoted by other
experiments and/or in different channels (see text for details).  }
\label{fig:aTGCcompare}
\end{center}
\end{figure}
%
%
The limits obtained in this analysis are competitive with the limits from the other
analyses.  Compared to the fully leptonic $WW$ analyses from hadron colliders, the limits
shown here are 
slightly more stringent for $\lambda$ and $\dgz$ and slightly worse for $\dkg$.
%

In table~\ref{tab:aTGC_noConstraint}, the limits are shown for each of the five aTGC parameters
when no relationship between the different parameters is imposed. In this scenario,
$\dgz$ has very little effect on the $WW$ process, whereas $\dkz$ has very little effect
on the $WZ$ process. 
\begin{table}[hp]
  \begin{center}
  \caption{The observed and expected 95\% CL limits on the anomalous triple gauge parameters 
$\lambdaz$, $\dkz$, $\dgz$, $\lambdag$, and $\dkg$, not subjected to any constraints between them.  
No form factors are applied to the aTGC parameters.
The limits on each parameter are calculated while fixing the other four parameters to zero.}
\label{tab:aTGC_noConstraint}
\begin{tabular}{lcc}
  \hline \hline
Parameter   &  Observed Limit & Expected Limit  \\
\hline
\lambdaz & [$-0.043$, 0.044] & [$-0.056$, 0.056]\\
\dkz & [$-0.090$, 0.105] & [$-0.11$, 0.12] \\
\dgz & [$-0.073$, 0.095] &  [$-0.11$, 0.12] \\
\lambdag & [$-0.15$, 0.15] & [$-0.17$, 0.16] \\
\dkg & [$-0.19$, 0.23] & [$-0.22$, 0.25] \\
\hline  \hline
\end{tabular}
\end{center}
\end{table}

Thus, analyses that restrict themselves to either the $WW$ process or
the $WZ$ process have limited sensitivity to at least one of the aTGC parameters.
In contrast, this analysis combines the two processes, and therefore has good 
sensitivity to all five aTGC parameters.  As an illustration, this analysis has four times
better expected limits on $\dgz$ than the ATLAS $\WWtolvlv$ analysis~\cite{ATLAS:2012mec}, and four
times better expected limits on $\dkz$ than the ATLAS  $\WZtolvll$ analysis~\cite{Aad:2012twa}.
%
%


Finally, table~\ref{tab:results_EFT}, gives limits on the EFT parameters.  
The limits on the EFT parameters $\cwp$, $\cbp$, and $\cwwwp$ are in the 
range (10--70)$\times (\Lambda/{\rm TeV})^2$.
In all cases, when computing the limits on one parameter, all the other parameters are
fixed to zero.


\begin{table}[h]
  \begin{center}
  \caption{The observed and expected 95\% CL limits on the effective field theory parameters $\cwww$, $\cb$, and $\cw$.
The limits on each parameter are calculated while fixing the other two parameters to zero.}
\label{tab:results_EFT}
\begin{tabular}{lcc}
  \hline \hline
Parameter   &  Observed Limit & Expected Limit  \\
\hline
\cwww & [$-9.5$, 9.6] \tevminSq  & [$-11.6$, 11.5]  \tevminSq  \\
\cb & [$-64$, 69] \tevminSq  & [$-73$, 79]  \tevminSq  \\
\cw & [$-13$, 18] \tevminSq  &  [$-17$, 21]  \tevminSq  \\
\hline  \hline
\end{tabular}
\end{center}
\end{table}





\begin{figure}[hp]
\begin{center}
\subfigure[]{
\includegraphics[width=0.47\textwidth]{toyLimits_lambda_vs_delkG.pdf}
}
\subfigure[]{
\includegraphics[width=0.47\textwidth]{toyLimits_lambda_vs_delgZ.pdf}
}
\subfigure[]{
\includegraphics[width=0.47\textwidth]{toyLimits_delkG_vs_delgZ.pdf}
}
\caption{
The observed two-dimensional 95\% CL contours for the anomalous 
triple gauge couplings (a) $\lambda$ versus $\dkg$, (b) $\lambda$ versus
$\dgz$, and (c) $\dkg$ versus $\dgz$. The limits are for the LEP
scenario without a form factor.
}
\label{fig:observedaTGCLimits2D}
\end{center}
\end{figure}



\begin{figure}[hp]
\begin{center}
\subfigure[]{
\includegraphics[width=0.47\textwidth]{toyLimits_cWWW_vs_cB.pdf}
}
\subfigure[]{
\includegraphics[width=0.47\textwidth]{toyLimits_cWWW_vs_cW.pdf}
}
\subfigure[]{
\includegraphics[width=0.47\textwidth]{toyLimits_cB_vs_cW.pdf}
}
\caption{
The observed two-dimensional 95\% CL contours for the effective field theory
parameters (a) $\cwww$ versus $\cb$, (b) $\cwww$ versus
$\cw$, and (c) $\cb$ versus $\cw$. 
}
\label{fig:observedEFTLimits2D}
\end{center}
\end{figure}


The observed two-dimensional 95\% CL limits  are shown in figure~\ref{fig:observedaTGCLimits2D}
for the LEP scenario.  The limits on $\dkg$ and $\dgz$ are significantly correlated, but
the limits on the other pairs of parameters do not have large correlations.
In addition, the observed two-dimensional 95\% CL limits on the EFT parameters
are shown in figure~\ref{fig:observedEFTLimits2D}. None of the EFT parameter pairs
exhibit strong correlations.





==> AuxilliaryPlots.tex <==
\section{Auxiliary plots}

\begin{figure}[h!]
\begin{center}
\subfigure[]{
  \label{subfig:DataFubEl}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{DataSubEl.pdf}
}
\subfigure[]{
 \label{subfig:DataSubMu}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{DataSubMu.pdf}
}
\caption{
 Distributions of the background-subtracted data (solid circles) for (a) the electron and (b) the muon channels. 
The error bars represent the statistical 
error on the data. The superimposed 
histograms show the fitted signal obtained from
the simultaneous fit to the electron and muon channels. 
The hatched 
bands show the systematic uncertainty on the background after profiling
the nuisance parameters. 
}
\label{fig:DataSubElAndMu}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\subfigure[]{
  \label{subfig:tempElSig}
  \includegraphics[width=0.47\textwidth,keepaspectratio]{TemplatesEleSig.pdf}
}
\subfigure[]{
  \label{subfig:tempMuSig}
  \includegraphics[width=0.47\textwidth,keepaspectratio]{TemplatesMuonSig.pdf}
}
\caption{\small  The nominal signal distributions for the reconstructed dijet invariant 
mass for the electron (a) and the muon (b) channels. The distributions for $WW$ and $WZ$ are shown separately and are obtained from MC. Both distributions are normalised to the expected number of events in each lepton channel.}
\label{fig:templatesSig}
\end{center}
\end{figure}


\begin{figure}[h!]
\begin{center}
\subfigure[]{
  \label{subfig:Jet1PreFit}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_Jet1_pT_EMU_SysBand.pdf}
}
\subfigure[]{
 \label{subfig:Jet2PreFit}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_Jet2_pT_EMU_SysBand.pdf}
}
\caption{
Distributions of the leading jet $\pT$ (a) and second-leading jet $\pT$ (b), for the sum of the electron and muon channels before doing the likelihood fit. The solid circles are data and the stacked histograms are SM predictions. The lower panel displays the ratio between the data and the SM prediction.  The systematic band only contains systematic uncertainties that affect the shape of the background and signal processes.
}
\label{fig:JetpTbeforeFit}
\end{center}
\end{figure}


\begin{figure}[h!]
\begin{center}
\subfigure[]{
  \label{subfig:dRJ1J2PreFit}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_dRJet1Jet2_EMU_SysBand.pdf}
}
\subfigure[]{
 \label{subfig:METPreFit}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_MET_EMU_SysBand.pdf}
}
\caption{
Distributions of $\Delta R(j_1,j_2)$ (a) and $\met$ (b), for the sum of the electron and muon channels before doing the likelihood fit. The solid circles are data and the stacked histograms are SM predictions. The lower panel displays the ratio between the data and the SM prediction.  The systematic band only contains systematic uncertainties that affect the shape of the background and signal processes.
}
\label{fig:dRAndMETbeforeFit}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\subfigure[]{
  \label{subfig:MtPreFit}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_mTMETLep_EMU_SysBand.pdf}
}
\subfigure[]{
 \label{subfig:LepPtPreFit}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_Lepton_pT_EMU_SysBand.pdf}
}
\caption{
Distributions of $\MT$ (a) and lepton $\pT$ (b), for the sum of the electron and muon channels before doing the likelihood fit. The solid circles are data and the stacked histograms are SM predictions. The lower panel displays the ratio between the data and the SM prediction.  The systematic band only contains systematic uncertainties that affect the shape of the background and signal processes.
}
\label{fig:MtAndLepPtbeforeFit}
\end{center}
\end{figure}


\begin{figure}[h!]
\begin{center}
 \includegraphics[width=0.80\textwidth,keepaspectratio]{toySignificance_Ue_JESJERUnsmooth_bbbCoherent.pdf}
\caption{
Distribution of the likelihood ratio $\lambda\equiv \lkl(N_{\rm sig}=0) / \lkl(N_{\rm sig}=N_{\rm sig, best}) $,
for background-only (red points) and signal+background
(blue points) pseudo-experiments. The expected value of $-{\rm log}~\lambda$ for the signal+background hypothesis is
shown as a vertical violet dashed line while the observed value is shown as a vertical black solid line.
}
\label{fig:SignificancePseudoExp}
\end{center}
\end{figure}



\begin{figure}[h!]
\begin{center}
 \includegraphics[width=0.8\textwidth,keepaspectratio]{aTGCcomparison.pdf}
\caption{
Comparison of aTGC limits obtained in this analysis with limits obtained by other
experiments.  All limits are given at 95\% CL, and calculated within the LEP scenario.  
The form-factor $\Lambda_{\rm FF}$ used in each analysis is listed; 
$\Lambda_{\rm FF}=\infty$ is equivalent to no form-factor.
The limits for each parameter are obtained fixing the other two parameters to zero.  
In the CMS $\lvjj$ analysis, $\dgz$ was fixed to zero throughout, so no limit on this
parameter was calculated.
}
\label{fig:aTGCcompareSimplified}
\end{center}
\end{figure}


==> CrossSection_alt.tex <==
As discussed in section~\ref{sec:AnalysisStrategy}, $\WVtolvjj$ candidates are selected 
in a fiducial phase space designed to increase the signal-to-background ratio. 
The fiducial phase space, which is identical for the electron and muon channels, is defined 
for Monte Carlo events by applying to the particle-level objects a selection as close as possible to the 
analysis selection described in section~\ref{sec:EventSelection}. This selection requires a $W$ boson decaying 
leptonically and a $W$ or $Z$ boson decaying hadronically. $W\to\tau\nu$ decays are not included in the definition of the fiducial cross section.

The leptonically decaying $W$ boson is required to decay to an electron or a muon with $\pT > 25$~GeV and $|\eta|<2.47$. The lepton  $\pT$
is obtained by summing together the lepton transverse momentum  and the transverse momenta of all photons
within $\DR =0.1$ of the selected lepton. 
The transverse mass of the leptonically decayed $W$ boson is required to be $\MT > 40$~GeV. 

Events must contain a hadronically decaying $W$ or $Z$ boson and two particle-level jets separated by $\DR >0.5$ from 
the selected leptons. Particle-level jets are reconstructed from particles 
with a mean decay length $c\tau>10$~mm
using the anti-$k_t$ algorithm with radius parameter $R$ = 0.4.  Decay products from 
leptonically decaying $W/Z$ bosons (including photons within $\DR=0.1$ of the charged
leptons) are excluded from the particle-level jets.
The two selected jets must lie within $|\eta|<2.0$ and have $\pT > 25$~GeV with at 
least one of them having $\pT > 30$~GeV. Events containing 
more than two particle-level jets with $\pT > 25$~GeV and $|\eta|<2.8$ are rejected. 
Moreover, the two selected jets must 
satisfy $|\DEtajj|<1.5$,  $25 < \Mjj <250$~GeV and $\DRjj > 0.7$. 

The last condition is applied only if the transverse momentum of the
dijet system is $\pTjj < 250$ GeV.
Finally the  $\MET$, defined as the transverse momentum of the neutrino from the leptonically decaying $W$ boson, is required to 
satisfy $\MET > 30$ GeV and $|\Delta \phi( \MET,j_1 )|>0.8 $. 

The signal event yield in the fiducial-volume is determined from a 
simultaneous maximum-likelihood fit to the $\Mjj$ distributions in the electron 
and muon channels. This method takes advantage of the difference between the shapes of 
the $\Mjj$ distributions of the various processes to separate the 
signal from the large underlying background. The $\Mjj$ templates, normalised 
to unit area, for the various processes contributing to the total expected $\Mjj$ 
distribution are shown in figure~\ref{fig:templates}.

\begin{figure}[htbp]
\begin{center}
\subfigure[]{
  \label{subfig:tempEl}
  \includegraphics[width=0.47\textwidth,keepaspectratio]{TemplatesEle.pdf}
}
\subfigure[]{
  \label{subfig:tempMu}
  \includegraphics[width=0.47\textwidth,keepaspectratio]{TemplatesMuon.pdf}
}
\caption{\small  The nominal templates for the reconstructed dijet invariant 
mass for (a) the electron and (b) the muon channels. 
The templates for $WW/WZ$, $\Vjet$ and top quarks, including single-top production, 
are obtained from MC, while the multijet template is obtained using a 
data-driven method. All templates are normalised to unit area.}
\label{fig:templates}
\end{center}
\end{figure}

Systematic uncertainties (described in section~\ref{sec:sys}) on 
the signal and background normalisation as well as on the $\Mjj$ shapes are 
included by introducing nuisance parameters ($\vec{\alpha}$) into the fit. 
The combined likelihood function ($\lkl$) is expressed as:
\begin{eqnarray}
\label{eq:L}
\lkl(\beta,\ \vec{\alpha}) = \prod_{ \ell}\prod_{b} {\mathrm{Poisson}}(n_{ \ell b} | ( \nu^{\rm bkg}_{\ell b} + \beta \nu^{\rm sig}_{\ell b}) (\vec{\alpha}))\cdot \prod_{p}f_p(\alpha_p),
\end{eqnarray}
where $\beta$ is the  parameter of interest extracted from the fit and is a 
multiplicative factor applied to the signal normalisation; $n_{\ell b}$ is the number of 
data events in bin $b$ and channel $\ell$, with  $\ell=e,\mu$; $\nu^{\rm bkg}_{\ell b}$  
and $\nu^{\rm sig}_{\ell b}$ are the number of expected events  for background 
and signal processes respectively  in bin $b$ and channel $\ell$; 
and $f_p$ are Gaussian constraints on the nuisance parameters $\alpha_p$. 
The expected number of signal events $\nu^{\rm sig}_{\ell b}$  contains 
contributions from both the $WW$ and $WZ$ processes. The measured signal yield 
$N^{WV}_{\ell}$ is 
obtained from the product of the fitted $\beta$ value and the 
expected number of signal events as $N^{WV}_{\ell } = \beta \cdot \sum_{b} \nu^{\rm sig}_{\ell b}$.


The diboson fiducial cross section ($\sigmafid$) is extracted  from $N^{WV}_{\ell }$
using eq.~(\ref{eq:simple1}).
The factors $\Dfid{_{,\ell}} $ account for the fact that two processes, $\WWtolvjj$ 
and $\WZtolvjj$, contribute to the signal yield with different cross sections,  
acceptances and correction factors and are defined as:
\begin{eqnarray}
\label{eq:simple2}
\Dfid{_{,\ell}}  =   \fWWfid \cdot C^{WW}_\ell + (1-\fWWfid) \cdot C^{WZ}_\ell ,
\end{eqnarray}
where 
$C^{WV}_{\ell}$ are the ratios of the detector-level signal yield after all 
analysis cuts to the signal yield in the fiducial phase space for the respective 
processes and lepton flavour. 
The values of $C^{WW}$ and $C^{WZ}$ vary between $0.61$ and $0.74$ and depend on the process and 
on the channel (electron, muon) considered.
The factor $\fWWfid$ represents the ratio of the $WW$ to 
the $WW+WZ$ fiducial cross sections. The two processes are
not separated by this analysis, so $\fWWfid$ is fixed to the 
SM value of $0.82$, calculated with \mcatnlo.

The total cross section is obtained by extrapolating the fiducial event yield 
to the full phase space using 
eq.~(\ref{eq:simple3}). The factors $\Dtot{_{,\ell}}$ are obtained from theoretical predictions and are defined as:
\begin{eqnarray}
\label{eq:Dtotal}
\Dtot{_{,\ell}} = \fWWtot \cdot C^{WW}_\ell \cdot \BR^{WW}_\ell \cdot A^{WW}_\ell + (1-\fWWtot) \cdot C^{WZ}_\ell \cdot \BR^{WZ}_\ell \cdot A^{WZ}_\ell
\end{eqnarray}
where the acceptances $A^{WW}_\ell$ and $A^{WZ}_\ell$ are calculated as the fraction of signal events satisfying 
the fiducial-volume selection criteria;  they vary in the range 0.08--0.09 depending on the 
process and are independent of the lepton flavour.  $\BR^{WW}_\ell$ and $\BR^{WZ}_\ell$ are the 
branching fractions for the decays \WWtolvjj~and \WZtolvjj~respectively~\cite{Beringer:1900zz}.  



\section{Systematic uncertainties}\label{sec:sys}
\input{systematics}


\section{Cross-section results}\label{sec:CrossSectionResults}

The $\Mjj$ maximum-likelihood fit, including all the nuisance parameters,
is performed on the data, and yields a value of $\beta = 1.11 \pm 0.26$,
where $\beta$ is defined in eq.~(\ref{eq:L}).
The uncertainty includes all the systematic uncertainties 
from the profiled sources; the purely statistical uncertainty on $\beta$ is $10\%$. 
The total systematic uncertainty on the signal yield, including
unprofiled systematic uncertainties, is $26\%$. The measured signal yields 
are  $N^{WV}_{e}  =  1970 \pm 200 \ \mathrm{(stat.)} \pm \ 500 \ \mathrm{(syst.)} $ 
and $N^{WV}_{ \mu}  =  2190 \pm 220  \ \mathrm{(stat.)} \pm \ 560 \ \mathrm{(syst.)} $ 
in the electron and muon channels respectively. 
This signal yield translates into a fiducial cross section of
 \begin{eqnarray}
 \sigmafid  = \xSecWVresultfid
 \end{eqnarray}
for the $WW$ and $WZ$ production processes summed over the muon and electron 
channels, and a total cross section of
\begin{eqnarray}
\sigmatot  =  68 \pm 7 \ \mathrm{(stat.)} \pm 19 \ \mathrm{(syst.)}{\rm ~pb}\,,
\end{eqnarray}
in good agreement with the Standard Model prediction obtained with \mcatnlo\ 
of $\sigmatot  =  \xSecWVpredictiontot$.

The signal yield significance is estimated using the likelihood 
ratio, defined as the ratio of the maximum-likelihood 
with the signal fixed to zero, to the maximum-likelihood including 
the signal component in the fit~\cite{ATLAS:2011tau,CMSCombination}.
The expected significance is estimated to be $\expectSignif$ by performing 
fits with and without the signal component to pseudo-data generated 
from MC samples with and without the signal component. The observed 
significance is $\obsSignif$.  The effect of systematic uncertainties is 
included in the significance calculations.

The $\Mjj$ distribution of the data overlaid with the fit result is
shown in figure~\ref{fig:MjjafterFit} for the sum of the electron and muon channels.
In addition, the background-subtracted data is shown overlaid 
with the fitted signal distribution.

\begin{figure}[ht!]
\begin{center}
\subfigure[]{
  \label{subfig:MjjPostFitElMu}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_Mjj_ElMu_AfterFit_withBottomPlot.pdf}

}
\subfigure[]{
 \label{subfig:DataSub}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{DataSubElMu.pdf}
}
\caption{
(a) Distributions of the dijet invariant mass for the sum of the electron and muon channels
after the likelihood fit.
The error bars represent statistical uncertainties, and the 
stacked histograms are the signal and background contributions.
The normalisations and shapes of the histograms are obtained from the best fit to the data, after being 
allowed to vary within their systematic uncertainties. 
The lower panel displays the ratio between the data and the total fit result, including
both signal and backgrounds.  The hatched
band shows the systematic uncertainty on the fitted signal plus background.
(b) Distribution of the background-subtracted data 
for the sum of the electron and muon channels. The error bars represent the statistical 
error on the data. The superimposed 
histogram shows the fitted signal 
and the hatched 
band shows the systematic uncertainty on the background after profiling
the nuisance parameters. 
}
\label{fig:MjjafterFit}
\end{center}
\end{figure}

As a cross-check, separate fits to the electron and muon channels 
were performed to extract the 
most probable $\beta$ values for the two channels. The values obtained, 
$1.00 \pm 0.37$ for the electron channel and $1.13 \pm 0.36$ for the 
muon channel, are  in 
agreement with the value obtained with the simultaneous fit.





==> EventSelection.tex <==
The $WV$ candidates are selected by requiring exactly one high-$\pT$ lepton, missing transverse momentum, and exactly two jets. 
Events are required to contain exactly one reconstructed lepton candidate with $\pT> 25$~\GeV; 
events with more 
than one identified lepton are rejected in order
to suppress the $Z+$jets and $t\bar t$ backgrounds. 
The lepton candidate must be the one that triggered the event.
Furthermore, events are required to have $\met > 30$~\GeV\ in order to 
account for the presence of the unobserved neutrino from the $W\to\ell\nu$ decays.  
The transverse mass of the leptonically decaying $W$ boson candidate is defined as 
$\MT = \sqrt{2 \cdot \pT(\ell) \cdot \met \cdot (1 - \cos \Delta\phi)}$, where 
$\Delta\phi$ is the azimuthal angle between 
the lepton momentum and missing transverse momentum vectors, and is required to satisfy $\MT>40 \gev$.
The $\met$ and $\MT$ criteria highly suppress the multijet background.
To further suppress the multijet background the azimuthal angular separation between the leading jet transverse momentum and the 
missing transverse momentum vectors must fulfil $|\Delta\phi(\met,j_1)| > 0.8$. Backgrounds containing top quark decays are highly reduced 
by vetoing events that contain more than two jets with $\pT>25$~GeV and $|\eta|<2.8$.
Events are required to contain exactly two jets with $|\eta|<2.0$ and $\pT > 25$~GeV,  with a $\pT > 30$~GeV requirement for the leading jet.
In order to improve the signal-to-background ratio, the two jets are required to satisfy $|\DEtajj|<1.5$.
The angular distance between the two jets must satisfy $\DRjj > 0.7$ if the $\pT$ of the 
dijet system is less than $250$~GeV.  
Finally, the dijet invariant mass must be in the range $25<\Mjj<250$~GeV.
The selection criteria were optimised to both increase the signal-to-background 
ratio and select a phase space region well described by the Monte Carlo simulation. 
After applying all event selection criteria, $127\,650$ events are 
found in the electron channel and $134\,846$ in the muon channel.


==> ObjectReco.tex <==
Events were selected by a single-lepton (electron or muon) trigger with a threshold on 
the transverse energy ($\ET$) in the electron case or on the transverse momentum ($\pT$) in the muon case.
The $p_{\rm T}$ threshold for the single-muon trigger was 18 GeV, while for electrons it was required  to be $\ET > 20$ GeV for the early part of 
data-taking and $E_{\rm T} > 22$ GeV when the instantaneous luminosity of the LHC increased. 

Proton--proton collision events are identified by requiring that 
the events have at least  one reconstructed vertex with at least three 
associated tracks with transverse momentum $p_{\rm T, track}>0.4$~GeV.
If two or more such vertices are found, the one with the largest sum of $p_{\rm T, track}^2$ is considered to be the primary vertex. 

Electron candidates are formed by associating clusters of cells in the EM calorimeter with tracks reconstructed in the inner detector~\cite{Aad:2014fxa}. The transverse 
energy ($\ET$), calculated from the cluster energy and the track direction, must be greater than 25 GeV,
in order to be in the region with maximum trigger efficiency. 
Candidates are accepted if they lie in the region $|\eta| < 2.47$, excluding the 
transition region between the barrel and endcap EM calorimeters, $1.37< |\eta| <1.52$. 
The candidate must satisfy ``tight'' identification criteria described in ref.~\cite{Aad:2014fxa}.
For the electron-candidate track, the ratio of the transverse impact parameter, $d_0$, 
to its uncertainty, $\sigma (d_0)$, 
must satisfy $|d_0/\sigma (d_0)|< 10$. 
The longitudinal impact parameter, $z_0$, must have an absolute value less than 1~mm.
Both $d_0$ and $z_0$ are measured with respect to the primary vertex.
To ensure isolation from surrounding particles, calorimetric and tracking criteria are applied. The total 
calorimeter $\ET$ in a cone of size $\Delta R = \sqrt{\Delta \phi^2 + \Delta \eta^2} = 0.3$ 
 around the electron candidate, excluding any $\ET$ associated with the candidate itself, must be less than 14\%
of the electron $\ET$ value.  
The calorimeter response is corrected 
for the additional energy deposited by pile-up. 
In addition, the scalar sum of the $\pT$ of the tracks within $\Delta R = 0.3$ of 
the electron candidate (not including the electron track) must be less than 13\% of the electron $\pT$ value. 


Muon candidates are identified~\cite{muon_perf_20112012} by associating tracks 
reconstructed in the muon spectrometer with tracks reconstructed in the inner detector. 
The momentum of the combined muon track is calculated from the momenta of 
the two tracks, correcting for the energy loss in the calorimeter. Muon 
candidates must satisfy
$\pT> 25$~GeV and $|\eta|<2.4$. The $\pT$ threshold is chosen to be well within the plateau of the trigger efficiency. Muon candidates must also be consistent with 
originating from the primary vertex, in order to reject muons from cosmic-ray interactions and to reduce background from heavy-flavour decays. Specifically,  the $d_0$ significance must satisfy $|d_0/\sigma (d_0)|< 3$  and $|z_0|$ must be less than 1~mm.  To reduce misidentification and  improve the muon momentum resolution, requirements on the minimum number of hits in the various detectors are applied to the muon tracks.
Isolated muons are selected with a requirement that the scalar sum of the $\pT$ of the tracks within $\Delta R = 0.3$  of the muon (not including the muon
track) be less than 15\% of the muon $\pT$, and that the total calorimeter $\ET$ in a cone of $\Delta R = 0.3$ around the muon candidate 
(excluding $\ET$ associated with the muon) be less than 14\% of the muon $\pT$.  The electron and muon isolation requirements 
are the same as used in ref.~\cite{ATLAS:2012mec}.

Corrections are applied to MC events in order to account for differences between 
data and MC simulation in the trigger 
and identification efficiencies, 
and in the lepton momentum and energy scale and resolution.  The trigger and reconstruction efficiency scale factors 
are measured  using the tag-and-probe method on events with $Z$-boson candidates %
events~\cite{Aad:2014fxa,muon_perf_20112012}.
The lepton momenta are calibrated with scale factors obtained by comparing the 
reconstructed mass distribution of $Z$ boson candidate events in data with that 
of simulated events~\cite{Aad:2014nim,muon_perf_20112012}.  

Jets are reconstructed from calorimeter energy clusters by using an %
anti-$k_t$ algorithm~\cite{AntiKt, Aad:2011he} with a radius 
parameter of 0.4. 
The selected jets must satisfy 
$E_{\rm T}>25$~GeV and $|\eta| < 2.8$.
Reconstructed jets are corrected for the non-compensating calorimeter response, upstream material and other effects 
using $p_{\rm T}$- and $\eta$-dependent correction factors derived from MC and validated with 
test-beam and collision data~\cite{Aad:2011he}.
Jets consistent with being produced from pile-up interactions are identified using the Jet Vertex Fraction variable (JVF). 
This variable is calculated using tracks that are associated with the jet, and is defined as the ratio of the scalar $p_{\rm T}$ sum of the associated tracks that originate from the primary vertex to the scalar $p_{\rm T}$ sum of all associated tracks. %
Jets that are within $|\eta|<2.5$ are retained if they have JVF larger than 75\% or if they have no associated track. 
The efficiency of this cut is $\sim95\%$ up to $|\eta|<2.5$ and is well modelled by the MC simulation. 
Jets are required to satisfy quality 
criteria and to lie at a distance $\DR >0.5 $ from well-identified leptons.

The $\MET$ is estimated from reconstructed electrons with $|\eta|< 2.47$, 
muons with $|\eta| < 2.7$, jets with $|\eta| < 4.9$, and clusters of energy in the calorimeter not associated with 
reconstructed objects having $|\eta|< 4.5$~\cite{Aad:2012re}. 
The energy clusters are calibrated to the EM scale or the hadronic energy scale according to cluster characteristics. 
The expected energy deposit of identified muons in the calorimeter is subtracted. 


==> SigBkgEstimate.tex <==
The shapes of the expected $\Mjj$ and $\pTjj$ distributions are used as templates for the cross-section fit 
and for the aTGC limit calculation, respectively.
The expected shapes and rates of the distributions for the  $\Wjet$, $\Zjet$, 
$t\bar t$, single-top, and signal processes are obtained 
from the MC simulation samples. 
The $\Wjet$ and $\Zjet$ predicted rates are corrected using scale factors obtained with a data-driven method as explained below. 

Multijet background events can pass the event selection if one of the jets is 
reconstructed as a lepton.
The rate and shape of the multijet background are estimated with data-driven methods 
since the MC simulation does not reliably predict the rate of jets passing the lepton identification. 

The data-driven method consists of two steps: the first one is designed to estimate the 
$\Mjj$, $\pTjj$, and $\MET$ shapes of the multijet background and the second one to measure its rate. 

The first step exploits suitably modified lepton identification criteria to define data samples enriched in 
multijet background and with kinematic characteristics as 
close as possible to those of the standard selection. The lepton identification criteria are modified differently for the muon and electron channels.

For the muon channel, the multijet-enriched sample is obtained by applying the full selection but 
inverting the transverse impact parameter requirement ($|d_0/\sigma(d_0)|>3$). 
The selected sample is composed of muons that do not originate from the primary vertex, as expected for muons produced from heavy-flavour decays in jets.
For the electron channel, the multijet-enriched sample is obtained by applying the full nominal selection
but requiring the electron candidate to satisfy the ``medium''~\cite{Aad:2011mk}  identification criteria but not
the ``tight'' ones.
This results in a sample enriched in events with a jet that mimics an electron. 
Finally, the shape of the multijet background is obtained from the data in these multijet-enriched samples, 
after subtracting the MC-based prediction for non-multijet processes.

The second step uses the $\MET$ shape of the multijet background, determined in the previous step, to obtain the 
multijet rate and a correction to the $\Vjet$ normalisation. This is done fitting the $\MET$ spectra obtained 
with the nominal selection but with the $\MET$ requirement removed.
The fit, performed in the range $0<\MET< 400$~GeV, extracts separate scale factors used to normalise the multijet and $\Vjet$ samples. 
From this fit, the multijet contribution is extrapolated to the signal region ($\MET>$ 30 GeV) and is 
found to represent  5.3\% and 3.7\% of the events for the electron and muon channels respectively. 
The $\Vjet$ scale factors obtained from this fit are close to one and well within the systematic uncertainty of the theoretical prediction both for the electron and muon channel. 

Table~\ref{tab:inclusivesel} shows the expected number of events for the signal and for each background process after 
the full selection is applied. The numbers of events observed in data are also 
listed.  The signal-to-background ratio in the subrange $60 <\Mjj <120$ GeV is about 2\%.
Figure~\ref{fig:MjjbeforeFit} shows the $\Mjj$ distributions for data and the SM prediction 
for the electron and muon channels prior to performing the maximum-likelihood fit to extract the signal $\WWWZ$ yield.
The bottom plots in figure~\ref{fig:MjjbeforeFit} show the ratios of data to 
the SM predictions overlaid with systematic uncertainty bands. The sources of systematic uncertainties and the strategy to 
evaluate them are discussed in section~\ref{sec:sys}. The data distributions  are well within the systematic 
uncertainty bands for all values of dijet mass for both channels.

\begin{figure}[htbp]
\begin{center}
\subfigure[]{
  \label{subfig:MjjPreFitMuon}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_Mjj_E_SysBand.pdf}
}
\subfigure[]{
 \label{subfig:MjjPreFitElec}
 \includegraphics[width=0.47\textwidth,keepaspectratio]{plot_Mjj_MU_SysBand.pdf}
}
\caption{
Distributions of the dijet invariant mass for (a) the electron and (b) the muon channels before the likelihood fit. 
The error bars represent statistical uncertainties, and the stacked histograms are SM predictions. The lower panel displays the ratio of the data to the MC expectation.  The systematic band contains only systematic uncertainties that affect the shape of the background and signal processes.
}
\label{fig:MjjbeforeFit}
\end{center}
\end{figure}

\begin{table}
  \begin{center}
  \caption{Total number of events in data and expected yields for each process in the $e$ and $\mu$ channel. 
The multijet and $\Vjet$ yields are obtained from the fit 
to the $\MET$ distribution as explained in section~\ref{sec:SigBkgEstimate}. Uncertainties for the expected signal yields are based 
on the corresponding cross-section uncertainties, while for multijet and the other backgrounds the uncertainties correspond 
to the total rate uncertainty. 
}
  \label{tab:inclusivesel}
  \begin{small}
    \begin{tabular}{lcc}
      \hline \hline
     Signal processes     &  $e$ & $\mu$ \\ 
      \hline
      $WW$ & 1435 $ \pm $ 70 & 1603 $\pm$ 79 \\
      $WZ$ & 334 $ \pm $ 23 & 370 $\pm$ 26 \\	
      \hline 
      Background processes     &  &  \\ 
      \hline
      $W+$ jets & $(107 \pm 21)\times 10^3$  & $(116 \pm 23)\times 10^3$ \\
      $Z+$ jets & (55 $\pm$ 11)$\times 10^2$ & (46.3 $\pm$ 9.3)$\times 10^2$ \\
      $t \bar t$ & (47.2 $\pm$ 7.1)$\times 10^2$ & (47.2 $\pm$ 7.1)$\times 10^2$ \\
      Single-top & (20.2 $\pm$ 3.0)$\times 10^2$ & (20.5 $\pm$ 3.1)$\times 10^2$ \\
      $\mathrm{Multijet}$ & (67 $\pm$ 10)$\times 10^2 $ & (50.5 $\pm$ 7.6)$\times 10^2$ \\
      $ZZ$ & 19.2 $\pm$ 3.8  & 21.1  $\pm$ 4.2 \\
      \hline 
      Total SM prediction & (128 $\pm$ 17)$\times 10^3$  & (135 $\pm$ 19)$\times 10^3$  \\
      \hline \hline
      Total Data & $127\,650$  & $134\,846$ \\
   	  \hline \hline     
    \end{tabular}
    \end{small}
  \end{center}
\end{table}


==> acknowledgements.tex <==


% Acknowledgements for papers with collision data
% Version 14-Oct-2014

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC,
Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP,
Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC,
China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic;
DNRF, DNSRC and Lundbeck Foundation, Denmark; EPLANET, ERC and NSRF, European Union;
IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, DFG, HGF, MPG and AvH
Foundation, Germany; GSRT and NSRF, Greece; ISF, MINERVA, GIF, I-CORE and Benoziyo Center,
Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO,
Netherlands; BRF and RCN, Norway; MNiSW and NCN, Poland; GRICES and FCT, Portugal; MNE/IFA, Romania; MES of Russia and ROSATOM, Russian Federation; JINR; MSTD,
Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa;
MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SER, SNSF and Cantons of
Bern and Geneva, Switzerland; NSC, Taiwan; TAEK, Turkey; STFC, the Royal
Society and Leverhulme Trust, United Kingdom; DOE and NSF, United States of
America.

The crucial computing support from all WLCG partners is acknowledged
gratefully, in particular from CERN and the ATLAS Tier-1 facilities at
TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France),
KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain),
ASGC (Taiwan), RAL (UK) and BNL (USA) and in the Tier-2 facilities
worldwide.
%----------------------------------------------




==> atlas_authlist.tex <==
% ATLAS Collaboration author list
% Data extracted on 21-Nov-2014 for paper reference STDM-2012-22
\begin{flushleft}
{\Large The ATLAS Collaboration}

\bigskip

G.~Aad$^{\rm 85}$,
B.~Abbott$^{\rm 113}$,
J.~Abdallah$^{\rm 152}$,
S.~Abdel~Khalek$^{\rm 117}$,
O.~Abdinov$^{\rm 11}$,
R.~Aben$^{\rm 107}$,
B.~Abi$^{\rm 114}$,
M.~Abolins$^{\rm 90}$,
O.S.~AbouZeid$^{\rm 159}$,
H.~Abramowicz$^{\rm 154}$,
H.~Abreu$^{\rm 153}$,
R.~Abreu$^{\rm 30}$,
Y.~Abulaiti$^{\rm 147a,147b}$,
B.S.~Acharya$^{\rm 165a,165b}$$^{,a}$,
L.~Adamczyk$^{\rm 38a}$,
D.L.~Adams$^{\rm 25}$,
J.~Adelman$^{\rm 108}$,
S.~Adomeit$^{\rm 100}$,
T.~Adye$^{\rm 131}$,
T.~Agatonovic-Jovin$^{\rm 13a}$,
J.A.~Aguilar-Saavedra$^{\rm 126a,126f}$,
M.~Agustoni$^{\rm 17}$,
S.P.~Ahlen$^{\rm 22}$,
F.~Ahmadov$^{\rm 65}$$^{,b}$,
G.~Aielli$^{\rm 134a,134b}$,
H.~Akerstedt$^{\rm 147a,147b}$,
T.P.A.~{\AA}kesson$^{\rm 81}$,
G.~Akimoto$^{\rm 156}$,
A.V.~Akimov$^{\rm 96}$,
G.L.~Alberghi$^{\rm 20a,20b}$,
J.~Albert$^{\rm 170}$,
S.~Albrand$^{\rm 55}$,
M.J.~Alconada~Verzini$^{\rm 71}$,
M.~Aleksa$^{\rm 30}$,
I.N.~Aleksandrov$^{\rm 65}$,
C.~Alexa$^{\rm 26a}$,
G.~Alexander$^{\rm 154}$,
G.~Alexandre$^{\rm 49}$,
T.~Alexopoulos$^{\rm 10}$,
M.~Alhroob$^{\rm 113}$,
G.~Alimonti$^{\rm 91a}$,
L.~Alio$^{\rm 85}$,
J.~Alison$^{\rm 31}$,
B.M.M.~Allbrooke$^{\rm 18}$,
L.J.~Allison$^{\rm 72}$,
P.P.~Allport$^{\rm 74}$,
A.~Aloisio$^{\rm 104a,104b}$,
A.~Alonso$^{\rm 36}$,
F.~Alonso$^{\rm 71}$,
C.~Alpigiani$^{\rm 76}$,
A.~Altheimer$^{\rm 35}$,
B.~Alvarez~Gonzalez$^{\rm 90}$,
M.G.~Alviggi$^{\rm 104a,104b}$,
K.~Amako$^{\rm 66}$,
Y.~Amaral~Coutinho$^{\rm 24a}$,
C.~Amelung$^{\rm 23}$,
D.~Amidei$^{\rm 89}$,
S.P.~Amor~Dos~Santos$^{\rm 126a,126c}$,
A.~Amorim$^{\rm 126a,126b}$,
S.~Amoroso$^{\rm 48}$,
N.~Amram$^{\rm 154}$,
G.~Amundsen$^{\rm 23}$,
C.~Anastopoulos$^{\rm 140}$,
L.S.~Ancu$^{\rm 49}$,
N.~Andari$^{\rm 30}$,
T.~Andeen$^{\rm 35}$,
C.F.~Anders$^{\rm 58b}$,
G.~Anders$^{\rm 30}$,
K.J.~Anderson$^{\rm 31}$,
A.~Andreazza$^{\rm 91a,91b}$,
V.~Andrei$^{\rm 58a}$,
X.S.~Anduaga$^{\rm 71}$,
S.~Angelidakis$^{\rm 9}$,
I.~Angelozzi$^{\rm 107}$,
P.~Anger$^{\rm 44}$,
A.~Angerami$^{\rm 35}$,
F.~Anghinolfi$^{\rm 30}$,
A.V.~Anisenkov$^{\rm 109}$$^{,c}$,
N.~Anjos$^{\rm 12}$,
A.~Annovi$^{\rm 47}$,
A.~Antonaki$^{\rm 9}$,
M.~Antonelli$^{\rm 47}$,
A.~Antonov$^{\rm 98}$,
J.~Antos$^{\rm 145b}$,
F.~Anulli$^{\rm 133a}$,
M.~Aoki$^{\rm 66}$,
L.~Aperio~Bella$^{\rm 18}$,
R.~Apolle$^{\rm 120}$$^{,d}$,
G.~Arabidze$^{\rm 90}$,
I.~Aracena$^{\rm 144}$,
Y.~Arai$^{\rm 66}$,
J.P.~Araque$^{\rm 126a}$,
A.T.H.~Arce$^{\rm 45}$,
F.A.~Arduh$^{\rm 71}$,
J-F.~Arguin$^{\rm 95}$,
S.~Argyropoulos$^{\rm 42}$,
M.~Arik$^{\rm 19a}$,
A.J.~Armbruster$^{\rm 30}$,
O.~Arnaez$^{\rm 30}$,
V.~Arnal$^{\rm 82}$,
H.~Arnold$^{\rm 48}$,
M.~Arratia$^{\rm 28}$,
O.~Arslan$^{\rm 21}$,
A.~Artamonov$^{\rm 97}$,
G.~Artoni$^{\rm 23}$,
S.~Asai$^{\rm 156}$,
N.~Asbah$^{\rm 42}$,
A.~Ashkenazi$^{\rm 154}$,
B.~{\AA}sman$^{\rm 147a,147b}$,
L.~Asquith$^{\rm 150}$,
K.~Assamagan$^{\rm 25}$,
R.~Astalos$^{\rm 145a}$,
M.~Atkinson$^{\rm 166}$,
N.B.~Atlay$^{\rm 142}$,
B.~Auerbach$^{\rm 6}$,
K.~Augsten$^{\rm 128}$,
M.~Aurousseau$^{\rm 146b}$,
G.~Avolio$^{\rm 30}$,
B.~Axen$^{\rm 15}$,
G.~Azuelos$^{\rm 95}$$^{,e}$,
Y.~Azuma$^{\rm 156}$,
M.A.~Baak$^{\rm 30}$,
A.E.~Baas$^{\rm 58a}$,
C.~Bacci$^{\rm 135a,135b}$,
H.~Bachacou$^{\rm 137}$,
K.~Bachas$^{\rm 155}$,
M.~Backes$^{\rm 30}$,
M.~Backhaus$^{\rm 30}$,
E.~Badescu$^{\rm 26a}$,
P.~Bagiacchi$^{\rm 133a,133b}$,
P.~Bagnaia$^{\rm 133a,133b}$,
Y.~Bai$^{\rm 33a}$,
T.~Bain$^{\rm 35}$,
J.T.~Baines$^{\rm 131}$,
O.K.~Baker$^{\rm 177}$,
P.~Balek$^{\rm 129}$,
F.~Balli$^{\rm 137}$,
E.~Banas$^{\rm 39}$,
Sw.~Banerjee$^{\rm 174}$,
A.A.E.~Bannoura$^{\rm 176}$,
H.S.~Bansil$^{\rm 18}$,
L.~Barak$^{\rm 173}$,
S.P.~Baranov$^{\rm 96}$,
E.L.~Barberio$^{\rm 88}$,
D.~Barberis$^{\rm 50a,50b}$,
M.~Barbero$^{\rm 85}$,
T.~Barillari$^{\rm 101}$,
M.~Barisonzi$^{\rm 176}$,
T.~Barklow$^{\rm 144}$,
N.~Barlow$^{\rm 28}$,
S.L.~Barnes$^{\rm 84}$,
B.M.~Barnett$^{\rm 131}$,
R.M.~Barnett$^{\rm 15}$,
Z.~Barnovska$^{\rm 5}$,
A.~Baroncelli$^{\rm 135a}$,
G.~Barone$^{\rm 49}$,
A.J.~Barr$^{\rm 120}$,
F.~Barreiro$^{\rm 82}$,
J.~Barreiro~Guimar\~{a}es~da~Costa$^{\rm 57}$,
R.~Bartoldus$^{\rm 144}$,
A.E.~Barton$^{\rm 72}$,
P.~Bartos$^{\rm 145a}$,
V.~Bartsch$^{\rm 150}$,
A.~Bassalat$^{\rm 117}$,
A.~Basye$^{\rm 166}$,
R.L.~Bates$^{\rm 53}$,
S.J.~Batista$^{\rm 159}$,
J.R.~Batley$^{\rm 28}$,
M.~Battaglia$^{\rm 138}$,
M.~Battistin$^{\rm 30}$,
F.~Bauer$^{\rm 137}$,
H.S.~Bawa$^{\rm 144}$$^{,f}$,
J.B.~Beacham$^{\rm 110}$,
M.D.~Beattie$^{\rm 72}$,
T.~Beau$^{\rm 80}$,
P.H.~Beauchemin$^{\rm 162}$,
R.~Beccherle$^{\rm 124a,124b}$,
P.~Bechtle$^{\rm 21}$,
H.P.~Beck$^{\rm 17}$$^{,g}$,
K.~Becker$^{\rm 120}$,
S.~Becker$^{\rm 100}$,
M.~Beckingham$^{\rm 171}$,
C.~Becot$^{\rm 117}$,
A.J.~Beddall$^{\rm 19c}$,
A.~Beddall$^{\rm 19c}$,
S.~Bedikian$^{\rm 177}$,
V.A.~Bednyakov$^{\rm 65}$,
C.P.~Bee$^{\rm 149}$,
L.J.~Beemster$^{\rm 107}$,
T.A.~Beermann$^{\rm 176}$,
M.~Begel$^{\rm 25}$,
K.~Behr$^{\rm 120}$,
C.~Belanger-Champagne$^{\rm 87}$,
P.J.~Bell$^{\rm 49}$,
W.H.~Bell$^{\rm 49}$,
G.~Bella$^{\rm 154}$,
L.~Bellagamba$^{\rm 20a}$,
A.~Bellerive$^{\rm 29}$,
M.~Bellomo$^{\rm 86}$,
K.~Belotskiy$^{\rm 98}$,
O.~Beltramello$^{\rm 30}$,
O.~Benary$^{\rm 154}$,
D.~Benchekroun$^{\rm 136a}$,
K.~Bendtz$^{\rm 147a,147b}$,
N.~Benekos$^{\rm 166}$,
Y.~Benhammou$^{\rm 154}$,
E.~Benhar~Noccioli$^{\rm 49}$,
J.A.~Benitez~Garcia$^{\rm 160b}$,
D.P.~Benjamin$^{\rm 45}$,
J.R.~Bensinger$^{\rm 23}$,
S.~Bentvelsen$^{\rm 107}$,
D.~Berge$^{\rm 107}$,
E.~Bergeaas~Kuutmann$^{\rm 167}$,
N.~Berger$^{\rm 5}$,
F.~Berghaus$^{\rm 170}$,
J.~Beringer$^{\rm 15}$,
C.~Bernard$^{\rm 22}$,
P.~Bernat$^{\rm 78}$,
C.~Bernius$^{\rm 110}$,
F.U.~Bernlochner$^{\rm 21}$,
T.~Berry$^{\rm 77}$,
P.~Berta$^{\rm 129}$,
C.~Bertella$^{\rm 83}$,
G.~Bertoli$^{\rm 147a,147b}$,
F.~Bertolucci$^{\rm 124a,124b}$,
C.~Bertsche$^{\rm 113}$,
D.~Bertsche$^{\rm 113}$,
M.I.~Besana$^{\rm 91a}$,
G.J.~Besjes$^{\rm 106}$,
O.~Bessidskaia$^{\rm 147a,147b}$,
M.~Bessner$^{\rm 42}$,
N.~Besson$^{\rm 137}$,
C.~Betancourt$^{\rm 48}$,
S.~Bethke$^{\rm 101}$,
W.~Bhimji$^{\rm 46}$,
R.M.~Bianchi$^{\rm 125}$,
L.~Bianchini$^{\rm 23}$,
M.~Bianco$^{\rm 30}$,
O.~Biebel$^{\rm 100}$,
S.P.~Bieniek$^{\rm 78}$,
K.~Bierwagen$^{\rm 54}$,
M.~Biglietti$^{\rm 135a}$,
J.~Bilbao~De~Mendizabal$^{\rm 49}$,
H.~Bilokon$^{\rm 47}$,
M.~Bindi$^{\rm 54}$,
S.~Binet$^{\rm 117}$,
A.~Bingul$^{\rm 19c}$,
C.~Bini$^{\rm 133a,133b}$,
C.W.~Black$^{\rm 151}$,
J.E.~Black$^{\rm 144}$,
K.M.~Black$^{\rm 22}$,
D.~Blackburn$^{\rm 139}$,
R.E.~Blair$^{\rm 6}$,
J.-B.~Blanchard$^{\rm 137}$,
T.~Blazek$^{\rm 145a}$,
I.~Bloch$^{\rm 42}$,
C.~Blocker$^{\rm 23}$,
W.~Blum$^{\rm 83}$$^{,*}$,
U.~Blumenschein$^{\rm 54}$,
G.J.~Bobbink$^{\rm 107}$,
V.S.~Bobrovnikov$^{\rm 109}$$^{,c}$,
S.S.~Bocchetta$^{\rm 81}$,
A.~Bocci$^{\rm 45}$,
C.~Bock$^{\rm 100}$,
C.R.~Boddy$^{\rm 120}$,
M.~Boehler$^{\rm 48}$,
T.T.~Boek$^{\rm 176}$,
J.A.~Bogaerts$^{\rm 30}$,
A.G.~Bogdanchikov$^{\rm 109}$,
A.~Bogouch$^{\rm 92}$$^{,*}$,
C.~Bohm$^{\rm 147a}$,
V.~Boisvert$^{\rm 77}$,
T.~Bold$^{\rm 38a}$,
V.~Boldea$^{\rm 26a}$,
A.S.~Boldyrev$^{\rm 99}$,
M.~Bomben$^{\rm 80}$,
M.~Bona$^{\rm 76}$,
M.~Boonekamp$^{\rm 137}$,
A.~Borisov$^{\rm 130}$,
G.~Borissov$^{\rm 72}$,
M.~Borri$^{\rm 84}$,
S.~Borroni$^{\rm 42}$,
J.~Bortfeldt$^{\rm 100}$,
V.~Bortolotto$^{\rm 60a}$,
K.~Bos$^{\rm 107}$,
D.~Boscherini$^{\rm 20a}$,
M.~Bosman$^{\rm 12}$,
H.~Boterenbrood$^{\rm 107}$,
J.~Boudreau$^{\rm 125}$,
J.~Bouffard$^{\rm 2}$,
E.V.~Bouhova-Thacker$^{\rm 72}$,
D.~Boumediene$^{\rm 34}$,
C.~Bourdarios$^{\rm 117}$,
N.~Bousson$^{\rm 114}$,
S.~Boutouil$^{\rm 136d}$,
A.~Boveia$^{\rm 31}$,
J.~Boyd$^{\rm 30}$,
I.R.~Boyko$^{\rm 65}$,
I.~Bozic$^{\rm 13a}$,
J.~Bracinik$^{\rm 18}$,
A.~Brandt$^{\rm 8}$,
G.~Brandt$^{\rm 15}$,
O.~Brandt$^{\rm 58a}$,
U.~Bratzler$^{\rm 157}$,
B.~Brau$^{\rm 86}$,
J.E.~Brau$^{\rm 116}$,
H.M.~Braun$^{\rm 176}$$^{,*}$,
S.F.~Brazzale$^{\rm 165a,165c}$,
B.~Brelier$^{\rm 159}$,
K.~Brendlinger$^{\rm 122}$,
A.J.~Brennan$^{\rm 88}$,
R.~Brenner$^{\rm 167}$,
S.~Bressler$^{\rm 173}$,
K.~Bristow$^{\rm 146c}$,
T.M.~Bristow$^{\rm 46}$,
D.~Britton$^{\rm 53}$,
F.M.~Brochu$^{\rm 28}$,
I.~Brock$^{\rm 21}$,
R.~Brock$^{\rm 90}$,
J.~Bronner$^{\rm 101}$,
G.~Brooijmans$^{\rm 35}$,
T.~Brooks$^{\rm 77}$,
W.K.~Brooks$^{\rm 32b}$,
J.~Brosamer$^{\rm 15}$,
E.~Brost$^{\rm 116}$,
J.~Brown$^{\rm 55}$,
P.A.~Bruckman~de~Renstrom$^{\rm 39}$,
D.~Bruncko$^{\rm 145b}$,
R.~Bruneliere$^{\rm 48}$,
S.~Brunet$^{\rm 61}$,
A.~Bruni$^{\rm 20a}$,
G.~Bruni$^{\rm 20a}$,
M.~Bruschi$^{\rm 20a}$,
L.~Bryngemark$^{\rm 81}$,
T.~Buanes$^{\rm 14}$,
Q.~Buat$^{\rm 143}$,
F.~Bucci$^{\rm 49}$,
P.~Buchholz$^{\rm 142}$,
A.G.~Buckley$^{\rm 53}$,
S.I.~Buda$^{\rm 26a}$,
I.A.~Budagov$^{\rm 65}$,
F.~Buehrer$^{\rm 48}$,
L.~Bugge$^{\rm 119}$,
M.K.~Bugge$^{\rm 119}$,
O.~Bulekov$^{\rm 98}$,
A.C.~Bundock$^{\rm 74}$,
H.~Burckhart$^{\rm 30}$,
S.~Burdin$^{\rm 74}$,
B.~Burghgrave$^{\rm 108}$,
S.~Burke$^{\rm 131}$,
I.~Burmeister$^{\rm 43}$,
E.~Busato$^{\rm 34}$,
D.~B\"uscher$^{\rm 48}$,
V.~B\"uscher$^{\rm 83}$,
P.~Bussey$^{\rm 53}$,
C.P.~Buszello$^{\rm 167}$,
B.~Butler$^{\rm 57}$,
J.M.~Butler$^{\rm 22}$,
A.I.~Butt$^{\rm 3}$,
C.M.~Buttar$^{\rm 53}$,
J.M.~Butterworth$^{\rm 78}$,
P.~Butti$^{\rm 107}$,
W.~Buttinger$^{\rm 28}$,
A.~Buzatu$^{\rm 53}$,
M.~Byszewski$^{\rm 10}$,
S.~Cabrera~Urb\'an$^{\rm 168}$,
D.~Caforio$^{\rm 20a,20b}$,
O.~Cakir$^{\rm 4a}$,
P.~Calafiura$^{\rm 15}$,
A.~Calandri$^{\rm 137}$,
G.~Calderini$^{\rm 80}$,
P.~Calfayan$^{\rm 100}$,
L.P.~Caloba$^{\rm 24a}$,
D.~Calvet$^{\rm 34}$,
S.~Calvet$^{\rm 34}$,
R.~Camacho~Toro$^{\rm 49}$,
S.~Camarda$^{\rm 42}$,
D.~Cameron$^{\rm 119}$,
L.M.~Caminada$^{\rm 15}$,
R.~Caminal~Armadans$^{\rm 12}$,
S.~Campana$^{\rm 30}$,
M.~Campanelli$^{\rm 78}$,
A.~Campoverde$^{\rm 149}$,
V.~Canale$^{\rm 104a,104b}$,
A.~Canepa$^{\rm 160a}$,
M.~Cano~Bret$^{\rm 76}$,
J.~Cantero$^{\rm 82}$,
R.~Cantrill$^{\rm 126a}$,
T.~Cao$^{\rm 40}$,
M.D.M.~Capeans~Garrido$^{\rm 30}$,
I.~Caprini$^{\rm 26a}$,
M.~Caprini$^{\rm 26a}$,
M.~Capua$^{\rm 37a,37b}$,
R.~Caputo$^{\rm 83}$,
R.~Cardarelli$^{\rm 134a}$,
T.~Carli$^{\rm 30}$,
G.~Carlino$^{\rm 104a}$,
L.~Carminati$^{\rm 91a,91b}$,
S.~Caron$^{\rm 106}$,
E.~Carquin$^{\rm 32a}$,
G.D.~Carrillo-Montoya$^{\rm 146c}$,
J.R.~Carter$^{\rm 28}$,
J.~Carvalho$^{\rm 126a,126c}$,
D.~Casadei$^{\rm 78}$,
M.P.~Casado$^{\rm 12}$,
M.~Casolino$^{\rm 12}$,
E.~Castaneda-Miranda$^{\rm 146b}$,
A.~Castelli$^{\rm 107}$,
V.~Castillo~Gimenez$^{\rm 168}$,
N.F.~Castro$^{\rm 126a}$,
P.~Catastini$^{\rm 57}$,
A.~Catinaccio$^{\rm 30}$,
J.R.~Catmore$^{\rm 119}$,
A.~Cattai$^{\rm 30}$,
G.~Cattani$^{\rm 134a,134b}$,
J.~Caudron$^{\rm 83}$,
V.~Cavaliere$^{\rm 166}$,
D.~Cavalli$^{\rm 91a}$,
M.~Cavalli-Sforza$^{\rm 12}$,
V.~Cavasinni$^{\rm 124a,124b}$,
F.~Ceradini$^{\rm 135a,135b}$,
B.C.~Cerio$^{\rm 45}$,
K.~Cerny$^{\rm 129}$,
A.S.~Cerqueira$^{\rm 24b}$,
A.~Cerri$^{\rm 150}$,
L.~Cerrito$^{\rm 76}$,
F.~Cerutti$^{\rm 15}$,
M.~Cerv$^{\rm 30}$,
A.~Cervelli$^{\rm 17}$,
S.A.~Cetin$^{\rm 19b}$,
A.~Chafaq$^{\rm 136a}$,
D.~Chakraborty$^{\rm 108}$,
I.~Chalupkova$^{\rm 129}$,
P.~Chang$^{\rm 166}$,
B.~Chapleau$^{\rm 87}$,
J.D.~Chapman$^{\rm 28}$,
D.~Charfeddine$^{\rm 117}$,
D.G.~Charlton$^{\rm 18}$,
C.C.~Chau$^{\rm 159}$,
C.A.~Chavez~Barajas$^{\rm 150}$,
S.~Cheatham$^{\rm 153}$,
A.~Chegwidden$^{\rm 90}$,
S.~Chekanov$^{\rm 6}$,
S.V.~Chekulaev$^{\rm 160a}$,
G.A.~Chelkov$^{\rm 65}$$^{,h}$,
M.A.~Chelstowska$^{\rm 89}$,
C.~Chen$^{\rm 64}$,
H.~Chen$^{\rm 25}$,
K.~Chen$^{\rm 149}$,
L.~Chen$^{\rm 33d}$$^{,i}$,
S.~Chen$^{\rm 33c}$,
X.~Chen$^{\rm 33f}$,
Y.~Chen$^{\rm 67}$,
H.C.~Cheng$^{\rm 89}$,
Y.~Cheng$^{\rm 31}$,
A.~Cheplakov$^{\rm 65}$,
E.~Cheremushkina$^{\rm 130}$,
R.~Cherkaoui~El~Moursli$^{\rm 136e}$,
V.~Chernyatin$^{\rm 25}$$^{,*}$,
E.~Cheu$^{\rm 7}$,
L.~Chevalier$^{\rm 137}$,
V.~Chiarella$^{\rm 47}$,
G.~Chiefari$^{\rm 104a,104b}$,
J.T.~Childers$^{\rm 6}$,
A.~Chilingarov$^{\rm 72}$,
G.~Chiodini$^{\rm 73a}$,
A.S.~Chisholm$^{\rm 18}$,
R.T.~Chislett$^{\rm 78}$,
A.~Chitan$^{\rm 26a}$,
M.V.~Chizhov$^{\rm 65}$,
S.~Chouridou$^{\rm 9}$,
B.K.B.~Chow$^{\rm 100}$,
D.~Chromek-Burckhart$^{\rm 30}$,
M.L.~Chu$^{\rm 152}$,
J.~Chudoba$^{\rm 127}$,
J.J.~Chwastowski$^{\rm 39}$,
L.~Chytka$^{\rm 115}$,
G.~Ciapetti$^{\rm 133a,133b}$,
A.K.~Ciftci$^{\rm 4a}$,
R.~Ciftci$^{\rm 4a}$,
D.~Cinca$^{\rm 53}$,
V.~Cindro$^{\rm 75}$,
A.~Ciocio$^{\rm 15}$,
Z.H.~Citron$^{\rm 173}$,
M.~Citterio$^{\rm 91a}$,
M.~Ciubancan$^{\rm 26a}$,
A.~Clark$^{\rm 49}$,
P.J.~Clark$^{\rm 46}$,
R.N.~Clarke$^{\rm 15}$,
W.~Cleland$^{\rm 125}$,
J.C.~Clemens$^{\rm 85}$,
C.~Clement$^{\rm 147a,147b}$,
Y.~Coadou$^{\rm 85}$,
M.~Cobal$^{\rm 165a,165c}$,
A.~Coccaro$^{\rm 139}$,
J.~Cochran$^{\rm 64}$,
L.~Coffey$^{\rm 23}$,
J.G.~Cogan$^{\rm 144}$,
B.~Cole$^{\rm 35}$,
S.~Cole$^{\rm 108}$,
A.P.~Colijn$^{\rm 107}$,
J.~Collot$^{\rm 55}$,
T.~Colombo$^{\rm 58c}$,
G.~Compostella$^{\rm 101}$,
P.~Conde~Mui\~no$^{\rm 126a,126b}$,
E.~Coniavitis$^{\rm 48}$,
S.H.~Connell$^{\rm 146b}$,
I.A.~Connelly$^{\rm 77}$,
S.M.~Consonni$^{\rm 91a,91b}$,
V.~Consorti$^{\rm 48}$,
S.~Constantinescu$^{\rm 26a}$,
C.~Conta$^{\rm 121a,121b}$,
G.~Conti$^{\rm 57}$,
F.~Conventi$^{\rm 104a}$$^{,j}$,
M.~Cooke$^{\rm 15}$,
B.D.~Cooper$^{\rm 78}$,
A.M.~Cooper-Sarkar$^{\rm 120}$,
N.J.~Cooper-Smith$^{\rm 77}$,
K.~Copic$^{\rm 15}$,
T.~Cornelissen$^{\rm 176}$,
M.~Corradi$^{\rm 20a}$,
F.~Corriveau$^{\rm 87}$$^{,k}$,
A.~Corso-Radu$^{\rm 164}$,
A.~Cortes-Gonzalez$^{\rm 12}$,
G.~Cortiana$^{\rm 101}$,
G.~Costa$^{\rm 91a}$,
M.J.~Costa$^{\rm 168}$,
D.~Costanzo$^{\rm 140}$,
D.~C\^ot\'e$^{\rm 8}$,
G.~Cottin$^{\rm 28}$,
G.~Cowan$^{\rm 77}$,
B.E.~Cox$^{\rm 84}$,
K.~Cranmer$^{\rm 110}$,
G.~Cree$^{\rm 29}$,
S.~Cr\'ep\'e-Renaudin$^{\rm 55}$,
F.~Crescioli$^{\rm 80}$,
W.A.~Cribbs$^{\rm 147a,147b}$,
M.~Crispin~Ortuzar$^{\rm 120}$,
M.~Cristinziani$^{\rm 21}$,
V.~Croft$^{\rm 106}$,
G.~Crosetti$^{\rm 37a,37b}$,
T.~Cuhadar~Donszelmann$^{\rm 140}$,
J.~Cummings$^{\rm 177}$,
M.~Curatolo$^{\rm 47}$,
C.~Cuthbert$^{\rm 151}$,
H.~Czirr$^{\rm 142}$,
P.~Czodrowski$^{\rm 3}$,
S.~D'Auria$^{\rm 53}$,
M.~D'Onofrio$^{\rm 74}$,
M.J.~Da~Cunha~Sargedas~De~Sousa$^{\rm 126a,126b}$,
C.~Da~Via$^{\rm 84}$,
W.~Dabrowski$^{\rm 38a}$,
A.~Dafinca$^{\rm 120}$,
T.~Dai$^{\rm 89}$,
O.~Dale$^{\rm 14}$,
F.~Dallaire$^{\rm 95}$,
C.~Dallapiccola$^{\rm 86}$,
M.~Dam$^{\rm 36}$,
A.C.~Daniells$^{\rm 18}$,
M.~Danninger$^{\rm 169}$,
M.~Dano~Hoffmann$^{\rm 137}$,
V.~Dao$^{\rm 48}$,
G.~Darbo$^{\rm 50a}$,
S.~Darmora$^{\rm 8}$,
J.~Dassoulas$^{\rm 74}$,
A.~Dattagupta$^{\rm 61}$,
W.~Davey$^{\rm 21}$,
C.~David$^{\rm 170}$,
T.~Davidek$^{\rm 129}$,
E.~Davies$^{\rm 120}$$^{,d}$,
M.~Davies$^{\rm 154}$,
O.~Davignon$^{\rm 80}$,
A.R.~Davison$^{\rm 78}$,
P.~Davison$^{\rm 78}$,
Y.~Davygora$^{\rm 58a}$,
E.~Dawe$^{\rm 143}$,
I.~Dawson$^{\rm 140}$,
R.K.~Daya-Ishmukhametova$^{\rm 86}$,
K.~De$^{\rm 8}$,
R.~de~Asmundis$^{\rm 104a}$,
S.~De~Castro$^{\rm 20a,20b}$,
S.~De~Cecco$^{\rm 80}$,
N.~De~Groot$^{\rm 106}$,
P.~de~Jong$^{\rm 107}$,
H.~De~la~Torre$^{\rm 82}$,
F.~De~Lorenzi$^{\rm 64}$,
L.~De~Nooij$^{\rm 107}$,
D.~De~Pedis$^{\rm 133a}$,
A.~De~Salvo$^{\rm 133a}$,
U.~De~Sanctis$^{\rm 150}$,
A.~De~Santo$^{\rm 150}$,
J.B.~De~Vivie~De~Regie$^{\rm 117}$,
W.J.~Dearnaley$^{\rm 72}$,
R.~Debbe$^{\rm 25}$,
C.~Debenedetti$^{\rm 138}$,
B.~Dechenaux$^{\rm 55}$,
D.V.~Dedovich$^{\rm 65}$,
I.~Deigaard$^{\rm 107}$,
J.~Del~Peso$^{\rm 82}$,
T.~Del~Prete$^{\rm 124a,124b}$,
F.~Deliot$^{\rm 137}$,
C.M.~Delitzsch$^{\rm 49}$,
M.~Deliyergiyev$^{\rm 75}$,
A.~Dell'Acqua$^{\rm 30}$,
L.~Dell'Asta$^{\rm 22}$,
M.~Dell'Orso$^{\rm 124a,124b}$,
M.~Della~Pietra$^{\rm 104a}$$^{,j}$,
D.~della~Volpe$^{\rm 49}$,
M.~Delmastro$^{\rm 5}$,
P.A.~Delsart$^{\rm 55}$,
C.~Deluca$^{\rm 107}$,
D.A.~DeMarco$^{\rm 159}$,
S.~Demers$^{\rm 177}$,
M.~Demichev$^{\rm 65}$,
A.~Demilly$^{\rm 80}$,
S.P.~Denisov$^{\rm 130}$,
D.~Derendarz$^{\rm 39}$,
J.E.~Derkaoui$^{\rm 136d}$,
F.~Derue$^{\rm 80}$,
P.~Dervan$^{\rm 74}$,
K.~Desch$^{\rm 21}$,
C.~Deterre$^{\rm 42}$,
P.O.~Deviveiros$^{\rm 30}$,
A.~Dewhurst$^{\rm 131}$,
S.~Dhaliwal$^{\rm 107}$,
A.~Di~Ciaccio$^{\rm 134a,134b}$,
L.~Di~Ciaccio$^{\rm 5}$,
A.~Di~Domenico$^{\rm 133a,133b}$,
C.~Di~Donato$^{\rm 104a,104b}$,
A.~Di~Girolamo$^{\rm 30}$,
B.~Di~Girolamo$^{\rm 30}$,
A.~Di~Mattia$^{\rm 153}$,
B.~Di~Micco$^{\rm 135a,135b}$,
R.~Di~Nardo$^{\rm 47}$,
A.~Di~Simone$^{\rm 48}$,
R.~Di~Sipio$^{\rm 20a,20b}$,
D.~Di~Valentino$^{\rm 29}$,
F.A.~Dias$^{\rm 46}$,
M.A.~Diaz$^{\rm 32a}$,
E.B.~Diehl$^{\rm 89}$,
J.~Dietrich$^{\rm 16}$,
T.A.~Dietzsch$^{\rm 58a}$,
S.~Diglio$^{\rm 85}$,
A.~Dimitrievska$^{\rm 13a}$,
J.~Dingfelder$^{\rm 21}$,
P.~Dita$^{\rm 26a}$,
S.~Dita$^{\rm 26a}$,
F.~Dittus$^{\rm 30}$,
F.~Djama$^{\rm 85}$,
T.~Djobava$^{\rm 51b}$,
J.I.~Djuvsland$^{\rm 58a}$,
M.A.B.~do~Vale$^{\rm 24c}$,
D.~Dobos$^{\rm 30}$,
C.~Doglioni$^{\rm 49}$,
T.~Doherty$^{\rm 53}$,
T.~Dohmae$^{\rm 156}$,
J.~Dolejsi$^{\rm 129}$,
Z.~Dolezal$^{\rm 129}$,
B.A.~Dolgoshein$^{\rm 98}$$^{,*}$,
M.~Donadelli$^{\rm 24d}$,
S.~Donati$^{\rm 124a,124b}$,
P.~Dondero$^{\rm 121a,121b}$,
J.~Donini$^{\rm 34}$,
J.~Dopke$^{\rm 131}$,
A.~Doria$^{\rm 104a}$,
M.T.~Dova$^{\rm 71}$,
A.T.~Doyle$^{\rm 53}$,
M.~Dris$^{\rm 10}$,
J.~Dubbert$^{\rm 89}$,
S.~Dube$^{\rm 15}$,
E.~Dubreuil$^{\rm 34}$,
E.~Duchovni$^{\rm 173}$,
G.~Duckeck$^{\rm 100}$,
O.A.~Ducu$^{\rm 26a}$,
D.~Duda$^{\rm 176}$,
A.~Dudarev$^{\rm 30}$,
F.~Dudziak$^{\rm 64}$,
L.~Duflot$^{\rm 117}$,
L.~Duguid$^{\rm 77}$,
M.~D\"uhrssen$^{\rm 30}$,
M.~Dunford$^{\rm 58a}$,
H.~Duran~Yildiz$^{\rm 4a}$,
M.~D\"uren$^{\rm 52}$,
A.~Durglishvili$^{\rm 51b}$,
D.~Duschinger$^{\rm 44}$,
M.~Dwuznik$^{\rm 38a}$,
M.~Dyndal$^{\rm 38a}$,
J.~Ebke$^{\rm 100}$,
W.~Edson$^{\rm 2}$,
N.C.~Edwards$^{\rm 46}$,
W.~Ehrenfeld$^{\rm 21}$,
T.~Eifert$^{\rm 30}$,
G.~Eigen$^{\rm 14}$,
K.~Einsweiler$^{\rm 15}$,
T.~Ekelof$^{\rm 167}$,
M.~El~Kacimi$^{\rm 136c}$,
M.~Ellert$^{\rm 167}$,
S.~Elles$^{\rm 5}$,
F.~Ellinghaus$^{\rm 83}$,
N.~Ellis$^{\rm 30}$,
J.~Elmsheuser$^{\rm 100}$,
M.~Elsing$^{\rm 30}$,
D.~Emeliyanov$^{\rm 131}$,
Y.~Enari$^{\rm 156}$,
O.C.~Endner$^{\rm 83}$,
M.~Endo$^{\rm 118}$,
R.~Engelmann$^{\rm 149}$,
J.~Erdmann$^{\rm 177}$,
A.~Ereditato$^{\rm 17}$,
D.~Eriksson$^{\rm 147a}$,
G.~Ernis$^{\rm 176}$,
J.~Ernst$^{\rm 2}$,
M.~Ernst$^{\rm 25}$,
J.~Ernwein$^{\rm 137}$,
S.~Errede$^{\rm 166}$,
E.~Ertel$^{\rm 83}$,
M.~Escalier$^{\rm 117}$,
H.~Esch$^{\rm 43}$,
C.~Escobar$^{\rm 125}$,
B.~Esposito$^{\rm 47}$,
A.I.~Etienvre$^{\rm 137}$,
E.~Etzion$^{\rm 154}$,
H.~Evans$^{\rm 61}$,
A.~Ezhilov$^{\rm 123}$,
L.~Fabbri$^{\rm 20a,20b}$,
G.~Facini$^{\rm 31}$,
R.M.~Fakhrutdinov$^{\rm 130}$,
S.~Falciano$^{\rm 133a}$,
R.J.~Falla$^{\rm 78}$,
J.~Faltova$^{\rm 129}$,
Y.~Fang$^{\rm 33a}$,
M.~Fanti$^{\rm 91a,91b}$,
A.~Farbin$^{\rm 8}$,
A.~Farilla$^{\rm 135a}$,
T.~Farooque$^{\rm 12}$,
S.~Farrell$^{\rm 15}$,
S.M.~Farrington$^{\rm 171}$,
P.~Farthouat$^{\rm 30}$,
F.~Fassi$^{\rm 136e}$,
P.~Fassnacht$^{\rm 30}$,
D.~Fassouliotis$^{\rm 9}$,
A.~Favareto$^{\rm 50a,50b}$,
L.~Fayard$^{\rm 117}$,
P.~Federic$^{\rm 145a}$,
O.L.~Fedin$^{\rm 123}$$^{,l}$,
W.~Fedorko$^{\rm 169}$,
S.~Feigl$^{\rm 30}$,
L.~Feligioni$^{\rm 85}$,
C.~Feng$^{\rm 33d}$,
E.J.~Feng$^{\rm 6}$,
H.~Feng$^{\rm 89}$,
A.B.~Fenyuk$^{\rm 130}$,
S.~Fernandez~Perez$^{\rm 30}$,
S.~Ferrag$^{\rm 53}$,
J.~Ferrando$^{\rm 53}$,
A.~Ferrari$^{\rm 167}$,
P.~Ferrari$^{\rm 107}$,
R.~Ferrari$^{\rm 121a}$,
D.E.~Ferreira~de~Lima$^{\rm 53}$,
A.~Ferrer$^{\rm 168}$,
D.~Ferrere$^{\rm 49}$,
C.~Ferretti$^{\rm 89}$,
A.~Ferretto~Parodi$^{\rm 50a,50b}$,
M.~Fiascaris$^{\rm 31}$,
F.~Fiedler$^{\rm 83}$,
A.~Filip\v{c}i\v{c}$^{\rm 75}$,
M.~Filipuzzi$^{\rm 42}$,
F.~Filthaut$^{\rm 106}$,
M.~Fincke-Keeler$^{\rm 170}$,
K.D.~Finelli$^{\rm 151}$,
M.C.N.~Fiolhais$^{\rm 126a,126c}$,
L.~Fiorini$^{\rm 168}$,
A.~Firan$^{\rm 40}$,
A.~Fischer$^{\rm 2}$,
J.~Fischer$^{\rm 176}$,
W.C.~Fisher$^{\rm 90}$,
E.A.~Fitzgerald$^{\rm 23}$,
M.~Flechl$^{\rm 48}$,
I.~Fleck$^{\rm 142}$,
P.~Fleischmann$^{\rm 89}$,
S.~Fleischmann$^{\rm 176}$,
G.T.~Fletcher$^{\rm 140}$,
G.~Fletcher$^{\rm 76}$,
T.~Flick$^{\rm 176}$,
A.~Floderus$^{\rm 81}$,
L.R.~Flores~Castillo$^{\rm 60a}$,
M.J.~Flowerdew$^{\rm 101}$,
A.~Formica$^{\rm 137}$,
A.~Forti$^{\rm 84}$,
D.~Fortin$^{\rm 160a}$,
D.~Fournier$^{\rm 117}$,
H.~Fox$^{\rm 72}$,
S.~Fracchia$^{\rm 12}$,
P.~Francavilla$^{\rm 80}$,
M.~Franchini$^{\rm 20a,20b}$,
S.~Franchino$^{\rm 30}$,
D.~Francis$^{\rm 30}$,
L.~Franconi$^{\rm 119}$,
M.~Franklin$^{\rm 57}$,
M.~Fraternali$^{\rm 121a,121b}$,
S.T.~French$^{\rm 28}$,
C.~Friedrich$^{\rm 42}$,
F.~Friedrich$^{\rm 44}$,
D.~Froidevaux$^{\rm 30}$,
J.A.~Frost$^{\rm 120}$,
C.~Fukunaga$^{\rm 157}$,
E.~Fullana~Torregrosa$^{\rm 83}$,
B.G.~Fulsom$^{\rm 144}$,
J.~Fuster$^{\rm 168}$,
C.~Gabaldon$^{\rm 55}$,
O.~Gabizon$^{\rm 176}$,
A.~Gabrielli$^{\rm 20a,20b}$,
A.~Gabrielli$^{\rm 133a,133b}$,
S.~Gadatsch$^{\rm 107}$,
S.~Gadomski$^{\rm 49}$,
G.~Gagliardi$^{\rm 50a,50b}$,
P.~Gagnon$^{\rm 61}$,
C.~Galea$^{\rm 106}$,
B.~Galhardo$^{\rm 126a,126c}$,
E.J.~Gallas$^{\rm 120}$,
B.J.~Gallop$^{\rm 131}$,
P.~Gallus$^{\rm 128}$,
G.~Galster$^{\rm 36}$,
K.K.~Gan$^{\rm 111}$,
J.~Gao$^{\rm 33b}$$^{,i}$,
Y.S.~Gao$^{\rm 144}$$^{,f}$,
F.M.~Garay~Walls$^{\rm 46}$,
F.~Garberson$^{\rm 177}$,
C.~Garc\'ia$^{\rm 168}$,
J.E.~Garc\'ia~Navarro$^{\rm 168}$,
M.~Garcia-Sciveres$^{\rm 15}$,
R.W.~Gardner$^{\rm 31}$,
N.~Garelli$^{\rm 144}$,
V.~Garonne$^{\rm 30}$,
C.~Gatti$^{\rm 47}$,
G.~Gaudio$^{\rm 121a}$,
B.~Gaur$^{\rm 142}$,
L.~Gauthier$^{\rm 95}$,
P.~Gauzzi$^{\rm 133a,133b}$,
I.L.~Gavrilenko$^{\rm 96}$,
C.~Gay$^{\rm 169}$,
G.~Gaycken$^{\rm 21}$,
E.N.~Gazis$^{\rm 10}$,
P.~Ge$^{\rm 33d}$,
Z.~Gecse$^{\rm 169}$,
C.N.P.~Gee$^{\rm 131}$,
D.A.A.~Geerts$^{\rm 107}$,
Ch.~Geich-Gimbel$^{\rm 21}$,
K.~Gellerstedt$^{\rm 147a,147b}$,
C.~Gemme$^{\rm 50a}$,
A.~Gemmell$^{\rm 53}$,
M.H.~Genest$^{\rm 55}$,
S.~Gentile$^{\rm 133a,133b}$,
M.~George$^{\rm 54}$,
S.~George$^{\rm 77}$,
D.~Gerbaudo$^{\rm 164}$,
A.~Gershon$^{\rm 154}$,
H.~Ghazlane$^{\rm 136b}$,
N.~Ghodbane$^{\rm 34}$,
B.~Giacobbe$^{\rm 20a}$,
S.~Giagu$^{\rm 133a,133b}$,
V.~Giangiobbe$^{\rm 12}$,
P.~Giannetti$^{\rm 124a,124b}$,
F.~Gianotti$^{\rm 30}$,
B.~Gibbard$^{\rm 25}$,
S.M.~Gibson$^{\rm 77}$,
M.~Gilchriese$^{\rm 15}$,
T.P.S.~Gillam$^{\rm 28}$,
D.~Gillberg$^{\rm 30}$,
G.~Gilles$^{\rm 34}$,
D.M.~Gingrich$^{\rm 3}$$^{,e}$,
N.~Giokaris$^{\rm 9}$,
M.P.~Giordani$^{\rm 165a,165c}$,
R.~Giordano$^{\rm 104a,104b}$,
F.M.~Giorgi$^{\rm 20a}$,
F.M.~Giorgi$^{\rm 16}$,
P.F.~Giraud$^{\rm 137}$,
D.~Giugni$^{\rm 91a}$,
C.~Giuliani$^{\rm 48}$,
M.~Giulini$^{\rm 58b}$,
B.K.~Gjelsten$^{\rm 119}$,
S.~Gkaitatzis$^{\rm 155}$,
I.~Gkialas$^{\rm 155}$,
E.L.~Gkougkousis$^{\rm 117}$,
L.K.~Gladilin$^{\rm 99}$,
C.~Glasman$^{\rm 82}$,
J.~Glatzer$^{\rm 30}$,
P.C.F.~Glaysher$^{\rm 46}$,
A.~Glazov$^{\rm 42}$,
G.L.~Glonti$^{\rm 62}$,
M.~Goblirsch-Kolb$^{\rm 101}$,
J.R.~Goddard$^{\rm 76}$,
J.~Godlewski$^{\rm 30}$,
C.~Goeringer$^{\rm 83}$,
S.~Goldfarb$^{\rm 89}$,
T.~Golling$^{\rm 177}$,
D.~Golubkov$^{\rm 130}$,
A.~Gomes$^{\rm 126a,126b,126d}$,
L.S.~Gomez~Fajardo$^{\rm 42}$,
R.~Gon\c{c}alo$^{\rm 126a}$,
J.~Goncalves~Pinto~Firmino~Da~Costa$^{\rm 137}$,
L.~Gonella$^{\rm 21}$,
S.~Gonz\'alez~de~la~Hoz$^{\rm 168}$,
G.~Gonzalez~Parra$^{\rm 12}$,
S.~Gonzalez-Sevilla$^{\rm 49}$,
L.~Goossens$^{\rm 30}$,
P.A.~Gorbounov$^{\rm 97}$,
H.A.~Gordon$^{\rm 25}$,
I.~Gorelov$^{\rm 105}$,
B.~Gorini$^{\rm 30}$,
E.~Gorini$^{\rm 73a,73b}$,
A.~Gori\v{s}ek$^{\rm 75}$,
E.~Gornicki$^{\rm 39}$,
A.T.~Goshaw$^{\rm 45}$,
C.~G\"ossling$^{\rm 43}$,
M.I.~Gostkin$^{\rm 65}$,
M.~Gouighri$^{\rm 136a}$,
D.~Goujdami$^{\rm 136c}$,
M.P.~Goulette$^{\rm 49}$,
A.G.~Goussiou$^{\rm 139}$,
C.~Goy$^{\rm 5}$,
H.M.X.~Grabas$^{\rm 138}$,
L.~Graber$^{\rm 54}$,
I.~Grabowska-Bold$^{\rm 38a}$,
P.~Grafstr\"om$^{\rm 20a,20b}$,
K-J.~Grahn$^{\rm 42}$,
J.~Gramling$^{\rm 49}$,
E.~Gramstad$^{\rm 119}$,
S.~Grancagnolo$^{\rm 16}$,
V.~Grassi$^{\rm 149}$,
V.~Gratchev$^{\rm 123}$,
H.M.~Gray$^{\rm 30}$,
E.~Graziani$^{\rm 135a}$,
O.G.~Grebenyuk$^{\rm 123}$,
Z.D.~Greenwood$^{\rm 79}$$^{,m}$,
K.~Gregersen$^{\rm 78}$,
I.M.~Gregor$^{\rm 42}$,
P.~Grenier$^{\rm 144}$,
J.~Griffiths$^{\rm 8}$,
A.A.~Grillo$^{\rm 138}$,
K.~Grimm$^{\rm 72}$,
S.~Grinstein$^{\rm 12}$$^{,n}$,
Ph.~Gris$^{\rm 34}$,
Y.V.~Grishkevich$^{\rm 99}$,
J.-F.~Grivaz$^{\rm 117}$,
J.P.~Grohs$^{\rm 44}$,
A.~Grohsjean$^{\rm 42}$,
E.~Gross$^{\rm 173}$,
J.~Grosse-Knetter$^{\rm 54}$,
G.C.~Grossi$^{\rm 134a,134b}$,
Z.J.~Grout$^{\rm 150}$,
L.~Guan$^{\rm 33b}$,
J.~Guenther$^{\rm 128}$,
F.~Guescini$^{\rm 49}$,
D.~Guest$^{\rm 177}$,
O.~Gueta$^{\rm 154}$,
C.~Guicheney$^{\rm 34}$,
E.~Guido$^{\rm 50a,50b}$,
T.~Guillemin$^{\rm 117}$,
S.~Guindon$^{\rm 2}$,
U.~Gul$^{\rm 53}$,
C.~Gumpert$^{\rm 44}$,
J.~Guo$^{\rm 35}$,
S.~Gupta$^{\rm 120}$,
P.~Gutierrez$^{\rm 113}$,
N.G.~Gutierrez~Ortiz$^{\rm 53}$,
C.~Gutschow$^{\rm 78}$,
N.~Guttman$^{\rm 154}$,
C.~Guyot$^{\rm 137}$,
C.~Gwenlan$^{\rm 120}$,
C.B.~Gwilliam$^{\rm 74}$,
A.~Haas$^{\rm 110}$,
C.~Haber$^{\rm 15}$,
H.K.~Hadavand$^{\rm 8}$,
N.~Haddad$^{\rm 136e}$,
P.~Haefner$^{\rm 21}$,
S.~Hageb\"ock$^{\rm 21}$,
Z.~Hajduk$^{\rm 39}$,
H.~Hakobyan$^{\rm 178}$,
M.~Haleem$^{\rm 42}$,
D.~Hall$^{\rm 120}$,
G.~Halladjian$^{\rm 90}$,
G.D.~Hallewell$^{\rm 85}$,
K.~Hamacher$^{\rm 176}$,
P.~Hamal$^{\rm 115}$,
K.~Hamano$^{\rm 170}$,
M.~Hamer$^{\rm 54}$,
A.~Hamilton$^{\rm 146a}$,
S.~Hamilton$^{\rm 162}$,
G.N.~Hamity$^{\rm 146c}$,
P.G.~Hamnett$^{\rm 42}$,
L.~Han$^{\rm 33b}$,
K.~Hanagaki$^{\rm 118}$,
K.~Hanawa$^{\rm 156}$,
M.~Hance$^{\rm 15}$,
P.~Hanke$^{\rm 58a}$,
R.~Hanna$^{\rm 137}$,
J.B.~Hansen$^{\rm 36}$,
J.D.~Hansen$^{\rm 36}$,
P.H.~Hansen$^{\rm 36}$,
K.~Hara$^{\rm 161}$,
A.S.~Hard$^{\rm 174}$,
T.~Harenberg$^{\rm 176}$,
F.~Hariri$^{\rm 117}$,
S.~Harkusha$^{\rm 92}$,
D.~Harper$^{\rm 89}$,
R.D.~Harrington$^{\rm 46}$,
O.M.~Harris$^{\rm 139}$,
P.F.~Harrison$^{\rm 171}$,
F.~Hartjes$^{\rm 107}$,
M.~Hasegawa$^{\rm 67}$,
S.~Hasegawa$^{\rm 103}$,
Y.~Hasegawa$^{\rm 141}$,
A.~Hasib$^{\rm 113}$,
S.~Hassani$^{\rm 137}$,
S.~Haug$^{\rm 17}$,
M.~Hauschild$^{\rm 30}$,
R.~Hauser$^{\rm 90}$,
M.~Havranek$^{\rm 127}$,
C.M.~Hawkes$^{\rm 18}$,
R.J.~Hawkings$^{\rm 30}$,
A.D.~Hawkins$^{\rm 81}$,
T.~Hayashi$^{\rm 161}$,
D.~Hayden$^{\rm 90}$,
C.P.~Hays$^{\rm 120}$,
J.M.~Hays$^{\rm 76}$,
H.S.~Hayward$^{\rm 74}$,
S.J.~Haywood$^{\rm 131}$,
S.J.~Head$^{\rm 18}$,
T.~Heck$^{\rm 83}$,
V.~Hedberg$^{\rm 81}$,
L.~Heelan$^{\rm 8}$,
S.~Heim$^{\rm 122}$,
T.~Heim$^{\rm 176}$,
B.~Heinemann$^{\rm 15}$,
L.~Heinrich$^{\rm 110}$,
J.~Hejbal$^{\rm 127}$,
L.~Helary$^{\rm 22}$,
C.~Heller$^{\rm 100}$,
M.~Heller$^{\rm 30}$,
S.~Hellman$^{\rm 147a,147b}$,
D.~Hellmich$^{\rm 21}$,
C.~Helsens$^{\rm 30}$,
J.~Henderson$^{\rm 120}$,
R.C.W.~Henderson$^{\rm 72}$,
Y.~Heng$^{\rm 174}$,
C.~Hengler$^{\rm 42}$,
A.~Henrichs$^{\rm 177}$,
A.M.~Henriques~Correia$^{\rm 30}$,
S.~Henrot-Versille$^{\rm 117}$,
G.H.~Herbert$^{\rm 16}$,
Y.~Hern\'andez~Jim\'enez$^{\rm 168}$,
R.~Herrberg-Schubert$^{\rm 16}$,
G.~Herten$^{\rm 48}$,
R.~Hertenberger$^{\rm 100}$,
L.~Hervas$^{\rm 30}$,
G.G.~Hesketh$^{\rm 78}$,
N.P.~Hessey$^{\rm 107}$,
R.~Hickling$^{\rm 76}$,
E.~Hig\'on-Rodriguez$^{\rm 168}$,
E.~Hill$^{\rm 170}$,
J.C.~Hill$^{\rm 28}$,
K.H.~Hiller$^{\rm 42}$,
S.J.~Hillier$^{\rm 18}$,
I.~Hinchliffe$^{\rm 15}$,
E.~Hines$^{\rm 122}$,
M.~Hirose$^{\rm 158}$,
D.~Hirschbuehl$^{\rm 176}$,
J.~Hobbs$^{\rm 149}$,
N.~Hod$^{\rm 107}$,
M.C.~Hodgkinson$^{\rm 140}$,
P.~Hodgson$^{\rm 140}$,
A.~Hoecker$^{\rm 30}$,
M.R.~Hoeferkamp$^{\rm 105}$,
F.~Hoenig$^{\rm 100}$,
D.~Hoffmann$^{\rm 85}$,
M.~Hohlfeld$^{\rm 83}$,
T.R.~Holmes$^{\rm 15}$,
T.M.~Hong$^{\rm 122}$,
L.~Hooft~van~Huysduynen$^{\rm 110}$,
W.H.~Hopkins$^{\rm 116}$,
Y.~Horii$^{\rm 103}$,
A.J.~Horton$^{\rm 143}$,
J-Y.~Hostachy$^{\rm 55}$,
S.~Hou$^{\rm 152}$,
A.~Hoummada$^{\rm 136a}$,
J.~Howard$^{\rm 120}$,
J.~Howarth$^{\rm 42}$,
M.~Hrabovsky$^{\rm 115}$,
I.~Hristova$^{\rm 16}$,
J.~Hrivnac$^{\rm 117}$,
T.~Hryn'ova$^{\rm 5}$,
A.~Hrynevich$^{\rm 93}$,
C.~Hsu$^{\rm 146c}$,
P.J.~Hsu$^{\rm 152}$,
S.-C.~Hsu$^{\rm 139}$,
D.~Hu$^{\rm 35}$,
X.~Hu$^{\rm 89}$,
Y.~Huang$^{\rm 42}$,
Z.~Hubacek$^{\rm 30}$,
F.~Hubaut$^{\rm 85}$,
F.~Huegging$^{\rm 21}$,
T.B.~Huffman$^{\rm 120}$,
E.W.~Hughes$^{\rm 35}$,
G.~Hughes$^{\rm 72}$,
M.~Huhtinen$^{\rm 30}$,
T.A.~H\"ulsing$^{\rm 83}$,
M.~Hurwitz$^{\rm 15}$,
N.~Huseynov$^{\rm 65}$$^{,b}$,
J.~Huston$^{\rm 90}$,
J.~Huth$^{\rm 57}$,
G.~Iacobucci$^{\rm 49}$,
G.~Iakovidis$^{\rm 10}$,
I.~Ibragimov$^{\rm 142}$,
L.~Iconomidou-Fayard$^{\rm 117}$,
E.~Ideal$^{\rm 177}$,
Z.~Idrissi$^{\rm 136e}$,
P.~Iengo$^{\rm 104a}$,
O.~Igonkina$^{\rm 107}$,
T.~Iizawa$^{\rm 172}$,
Y.~Ikegami$^{\rm 66}$,
K.~Ikematsu$^{\rm 142}$,
M.~Ikeno$^{\rm 66}$,
Y.~Ilchenko$^{\rm 31}$$^{,o}$,
D.~Iliadis$^{\rm 155}$,
N.~Ilic$^{\rm 159}$,
Y.~Inamaru$^{\rm 67}$,
T.~Ince$^{\rm 101}$,
P.~Ioannou$^{\rm 9}$,
M.~Iodice$^{\rm 135a}$,
K.~Iordanidou$^{\rm 9}$,
V.~Ippolito$^{\rm 57}$,
A.~Irles~Quiles$^{\rm 168}$,
C.~Isaksson$^{\rm 167}$,
M.~Ishino$^{\rm 68}$,
M.~Ishitsuka$^{\rm 158}$,
R.~Ishmukhametov$^{\rm 111}$,
C.~Issever$^{\rm 120}$,
S.~Istin$^{\rm 19a}$,
J.M.~Iturbe~Ponce$^{\rm 84}$,
R.~Iuppa$^{\rm 134a,134b}$,
J.~Ivarsson$^{\rm 81}$,
W.~Iwanski$^{\rm 39}$,
H.~Iwasaki$^{\rm 66}$,
J.M.~Izen$^{\rm 41}$,
V.~Izzo$^{\rm 104a}$,
B.~Jackson$^{\rm 122}$,
M.~Jackson$^{\rm 74}$,
P.~Jackson$^{\rm 1}$,
M.R.~Jaekel$^{\rm 30}$,
V.~Jain$^{\rm 2}$,
K.~Jakobs$^{\rm 48}$,
S.~Jakobsen$^{\rm 30}$,
T.~Jakoubek$^{\rm 127}$,
J.~Jakubek$^{\rm 128}$,
D.O.~Jamin$^{\rm 152}$,
D.K.~Jana$^{\rm 79}$,
E.~Jansen$^{\rm 78}$,
H.~Jansen$^{\rm 30}$,
J.~Janssen$^{\rm 21}$,
M.~Janus$^{\rm 171}$,
G.~Jarlskog$^{\rm 81}$,
N.~Javadov$^{\rm 65}$$^{,b}$,
T.~Jav\r{u}rek$^{\rm 48}$,
L.~Jeanty$^{\rm 15}$,
J.~Jejelava$^{\rm 51a}$$^{,p}$,
G.-Y.~Jeng$^{\rm 151}$,
D.~Jennens$^{\rm 88}$,
P.~Jenni$^{\rm 48}$$^{,q}$,
J.~Jentzsch$^{\rm 43}$,
C.~Jeske$^{\rm 171}$,
S.~J\'ez\'equel$^{\rm 5}$,
H.~Ji$^{\rm 174}$,
J.~Jia$^{\rm 149}$,
Y.~Jiang$^{\rm 33b}$,
M.~Jimenez~Belenguer$^{\rm 42}$,
S.~Jin$^{\rm 33a}$,
A.~Jinaru$^{\rm 26a}$,
O.~Jinnouchi$^{\rm 158}$,
M.D.~Joergensen$^{\rm 36}$,
K.E.~Johansson$^{\rm 147a,147b}$,
P.~Johansson$^{\rm 140}$,
K.A.~Johns$^{\rm 7}$,
K.~Jon-And$^{\rm 147a,147b}$,
G.~Jones$^{\rm 171}$,
R.W.L.~Jones$^{\rm 72}$,
T.J.~Jones$^{\rm 74}$,
J.~Jongmanns$^{\rm 58a}$,
P.M.~Jorge$^{\rm 126a,126b}$,
K.D.~Joshi$^{\rm 84}$,
J.~Jovicevic$^{\rm 148}$,
X.~Ju$^{\rm 174}$,
C.A.~Jung$^{\rm 43}$,
P.~Jussel$^{\rm 62}$,
A.~Juste~Rozas$^{\rm 12}$$^{,n}$,
M.~Kaci$^{\rm 168}$,
A.~Kaczmarska$^{\rm 39}$,
M.~Kado$^{\rm 117}$,
H.~Kagan$^{\rm 111}$,
M.~Kagan$^{\rm 144}$,
E.~Kajomovitz$^{\rm 45}$,
C.W.~Kalderon$^{\rm 120}$,
S.~Kama$^{\rm 40}$,
A.~Kamenshchikov$^{\rm 130}$,
N.~Kanaya$^{\rm 156}$,
M.~Kaneda$^{\rm 30}$,
S.~Kaneti$^{\rm 28}$,
V.A.~Kantserov$^{\rm 98}$,
J.~Kanzaki$^{\rm 66}$,
B.~Kaplan$^{\rm 110}$,
A.~Kapliy$^{\rm 31}$,
D.~Kar$^{\rm 53}$,
K.~Karakostas$^{\rm 10}$,
A.~Karamaoun$^{\rm 3}$,
N.~Karastathis$^{\rm 10}$,
M.J.~Kareem$^{\rm 54}$,
M.~Karnevskiy$^{\rm 83}$,
S.N.~Karpov$^{\rm 65}$,
Z.M.~Karpova$^{\rm 65}$,
K.~Karthik$^{\rm 110}$,
V.~Kartvelishvili$^{\rm 72}$,
A.N.~Karyukhin$^{\rm 130}$,
L.~Kashif$^{\rm 174}$,
G.~Kasieczka$^{\rm 58b}$,
R.D.~Kass$^{\rm 111}$,
A.~Kastanas$^{\rm 14}$,
Y.~Kataoka$^{\rm 156}$,
A.~Katre$^{\rm 49}$,
J.~Katzy$^{\rm 42}$,
V.~Kaushik$^{\rm 7}$,
K.~Kawagoe$^{\rm 70}$,
T.~Kawamoto$^{\rm 156}$,
G.~Kawamura$^{\rm 54}$,
S.~Kazama$^{\rm 156}$,
V.F.~Kazanin$^{\rm 109}$,
M.Y.~Kazarinov$^{\rm 65}$,
R.~Keeler$^{\rm 170}$,
R.~Kehoe$^{\rm 40}$,
M.~Keil$^{\rm 54}$,
J.S.~Keller$^{\rm 42}$,
J.J.~Kempster$^{\rm 77}$,
H.~Keoshkerian$^{\rm 5}$,
O.~Kepka$^{\rm 127}$,
B.P.~Ker\v{s}evan$^{\rm 75}$,
S.~Kersten$^{\rm 176}$,
K.~Kessoku$^{\rm 156}$,
J.~Keung$^{\rm 159}$,
R.A.~Keyes$^{\rm 87}$,
F.~Khalil-zada$^{\rm 11}$,
H.~Khandanyan$^{\rm 147a,147b}$,
A.~Khanov$^{\rm 114}$,
A.~Kharlamov$^{\rm 109}$,
A.~Khodinov$^{\rm 98}$,
A.~Khomich$^{\rm 58a}$,
T.J.~Khoo$^{\rm 28}$,
G.~Khoriauli$^{\rm 21}$,
V.~Khovanskiy$^{\rm 97}$,
E.~Khramov$^{\rm 65}$,
J.~Khubua$^{\rm 51b}$,
H.Y.~Kim$^{\rm 8}$,
H.~Kim$^{\rm 147a,147b}$,
S.H.~Kim$^{\rm 161}$,
N.~Kimura$^{\rm 155}$,
O.~Kind$^{\rm 16}$,
B.T.~King$^{\rm 74}$,
M.~King$^{\rm 168}$,
R.S.B.~King$^{\rm 120}$,
S.B.~King$^{\rm 169}$,
J.~Kirk$^{\rm 131}$,
A.E.~Kiryunin$^{\rm 101}$,
T.~Kishimoto$^{\rm 67}$,
D.~Kisielewska$^{\rm 38a}$,
F.~Kiss$^{\rm 48}$,
K.~Kiuchi$^{\rm 161}$,
E.~Kladiva$^{\rm 145b}$,
M.~Klein$^{\rm 74}$,
U.~Klein$^{\rm 74}$,
K.~Kleinknecht$^{\rm 83}$,
P.~Klimek$^{\rm 147a,147b}$,
A.~Klimentov$^{\rm 25}$,
R.~Klingenberg$^{\rm 43}$,
J.A.~Klinger$^{\rm 84}$,
T.~Klioutchnikova$^{\rm 30}$,
P.F.~Klok$^{\rm 106}$,
E.-E.~Kluge$^{\rm 58a}$,
P.~Kluit$^{\rm 107}$,
S.~Kluth$^{\rm 101}$,
E.~Kneringer$^{\rm 62}$,
E.B.F.G.~Knoops$^{\rm 85}$,
A.~Knue$^{\rm 53}$,
D.~Kobayashi$^{\rm 158}$,
T.~Kobayashi$^{\rm 156}$,
M.~Kobel$^{\rm 44}$,
M.~Kocian$^{\rm 144}$,
P.~Kodys$^{\rm 129}$,
T.~Koffas$^{\rm 29}$,
E.~Koffeman$^{\rm 107}$,
L.A.~Kogan$^{\rm 120}$,
S.~Kohlmann$^{\rm 176}$,
Z.~Kohout$^{\rm 128}$,
T.~Kohriki$^{\rm 66}$,
T.~Koi$^{\rm 144}$,
H.~Kolanoski$^{\rm 16}$,
I.~Koletsou$^{\rm 5}$,
J.~Koll$^{\rm 90}$,
A.A.~Komar$^{\rm 96}$$^{,*}$,
Y.~Komori$^{\rm 156}$,
T.~Kondo$^{\rm 66}$,
N.~Kondrashova$^{\rm 42}$,
K.~K\"oneke$^{\rm 48}$,
A.C.~K\"onig$^{\rm 106}$,
S.~K{\"o}nig$^{\rm 83}$,
T.~Kono$^{\rm 66}$$^{,r}$,
R.~Konoplich$^{\rm 110}$$^{,s}$,
N.~Konstantinidis$^{\rm 78}$,
R.~Kopeliansky$^{\rm 153}$,
S.~Koperny$^{\rm 38a}$,
L.~K\"opke$^{\rm 83}$,
A.K.~Kopp$^{\rm 48}$,
K.~Korcyl$^{\rm 39}$,
K.~Kordas$^{\rm 155}$,
A.~Korn$^{\rm 78}$,
A.A.~Korol$^{\rm 109}$$^{,c}$,
I.~Korolkov$^{\rm 12}$,
E.V.~Korolkova$^{\rm 140}$,
V.A.~Korotkov$^{\rm 130}$,
O.~Kortner$^{\rm 101}$,
S.~Kortner$^{\rm 101}$,
V.V.~Kostyukhin$^{\rm 21}$,
V.M.~Kotov$^{\rm 65}$,
A.~Kotwal$^{\rm 45}$,
A.~Kourkoumeli-Charalampidi$^{\rm 155}$,
C.~Kourkoumelis$^{\rm 9}$,
V.~Kouskoura$^{\rm 25}$,
A.~Koutsman$^{\rm 160a}$,
R.~Kowalewski$^{\rm 170}$,
T.Z.~Kowalski$^{\rm 38a}$,
W.~Kozanecki$^{\rm 137}$,
A.S.~Kozhin$^{\rm 130}$,
V.A.~Kramarenko$^{\rm 99}$,
G.~Kramberger$^{\rm 75}$,
D.~Krasnopevtsev$^{\rm 98}$,
M.W.~Krasny$^{\rm 80}$,
A.~Krasznahorkay$^{\rm 30}$,
J.K.~Kraus$^{\rm 21}$,
A.~Kravchenko$^{\rm 25}$,
S.~Kreiss$^{\rm 110}$,
M.~Kretz$^{\rm 58c}$,
J.~Kretzschmar$^{\rm 74}$,
K.~Kreutzfeldt$^{\rm 52}$,
P.~Krieger$^{\rm 159}$,
K.~Kroeninger$^{\rm 54}$,
H.~Kroha$^{\rm 101}$,
J.~Kroll$^{\rm 122}$,
J.~Kroseberg$^{\rm 21}$,
J.~Krstic$^{\rm 13a}$,
U.~Kruchonak$^{\rm 65}$,
H.~Kr\"uger$^{\rm 21}$,
T.~Kruker$^{\rm 17}$,
N.~Krumnack$^{\rm 64}$,
Z.V.~Krumshteyn$^{\rm 65}$,
A.~Kruse$^{\rm 174}$,
M.C.~Kruse$^{\rm 45}$,
M.~Kruskal$^{\rm 22}$,
T.~Kubota$^{\rm 88}$,
H.~Kucuk$^{\rm 78}$,
S.~Kuday$^{\rm 4c}$,
S.~Kuehn$^{\rm 48}$,
A.~Kugel$^{\rm 58c}$,
A.~Kuhl$^{\rm 138}$,
T.~Kuhl$^{\rm 42}$,
V.~Kukhtin$^{\rm 65}$,
Y.~Kulchitsky$^{\rm 92}$,
S.~Kuleshov$^{\rm 32b}$,
M.~Kuna$^{\rm 133a,133b}$,
T.~Kunigo$^{\rm 68}$,
A.~Kupco$^{\rm 127}$,
H.~Kurashige$^{\rm 67}$,
Y.A.~Kurochkin$^{\rm 92}$,
R.~Kurumida$^{\rm 67}$,
V.~Kus$^{\rm 127}$,
E.S.~Kuwertz$^{\rm 148}$,
M.~Kuze$^{\rm 158}$,
J.~Kvita$^{\rm 115}$,
D.~Kyriazopoulos$^{\rm 140}$,
A.~La~Rosa$^{\rm 49}$,
L.~La~Rotonda$^{\rm 37a,37b}$,
C.~Lacasta$^{\rm 168}$,
F.~Lacava$^{\rm 133a,133b}$,
J.~Lacey$^{\rm 29}$,
H.~Lacker$^{\rm 16}$,
D.~Lacour$^{\rm 80}$,
V.R.~Lacuesta$^{\rm 168}$,
E.~Ladygin$^{\rm 65}$,
R.~Lafaye$^{\rm 5}$,
B.~Laforge$^{\rm 80}$,
T.~Lagouri$^{\rm 177}$,
S.~Lai$^{\rm 48}$,
H.~Laier$^{\rm 58a}$,
L.~Lambourne$^{\rm 78}$,
S.~Lammers$^{\rm 61}$,
C.L.~Lampen$^{\rm 7}$,
W.~Lampl$^{\rm 7}$,
E.~Lan\c{c}on$^{\rm 137}$,
U.~Landgraf$^{\rm 48}$,
M.P.J.~Landon$^{\rm 76}$,
V.S.~Lang$^{\rm 58a}$,
A.J.~Lankford$^{\rm 164}$,
F.~Lanni$^{\rm 25}$,
K.~Lantzsch$^{\rm 30}$,
S.~Laplace$^{\rm 80}$,
C.~Lapoire$^{\rm 21}$,
J.F.~Laporte$^{\rm 137}$,
T.~Lari$^{\rm 91a}$,
F.~Lasagni~Manghi$^{\rm 20a,20b}$,
M.~Lassnig$^{\rm 30}$,
P.~Laurelli$^{\rm 47}$,
W.~Lavrijsen$^{\rm 15}$,
A.T.~Law$^{\rm 138}$,
P.~Laycock$^{\rm 74}$,
O.~Le~Dortz$^{\rm 80}$,
E.~Le~Guirriec$^{\rm 85}$,
E.~Le~Menedeu$^{\rm 12}$,
T.~LeCompte$^{\rm 6}$,
F.~Ledroit-Guillon$^{\rm 55}$,
C.A.~Lee$^{\rm 146b}$,
H.~Lee$^{\rm 107}$,
S.C.~Lee$^{\rm 152}$,
L.~Lee$^{\rm 1}$,
G.~Lefebvre$^{\rm 80}$,
M.~Lefebvre$^{\rm 170}$,
F.~Legger$^{\rm 100}$,
C.~Leggett$^{\rm 15}$,
A.~Lehan$^{\rm 74}$,
G.~Lehmann~Miotto$^{\rm 30}$,
X.~Lei$^{\rm 7}$,
W.A.~Leight$^{\rm 29}$,
A.~Leisos$^{\rm 155}$,
A.G.~Leister$^{\rm 177}$,
M.A.L.~Leite$^{\rm 24d}$,
R.~Leitner$^{\rm 129}$,
D.~Lellouch$^{\rm 173}$,
B.~Lemmer$^{\rm 54}$,
K.J.C.~Leney$^{\rm 78}$,
T.~Lenz$^{\rm 21}$,
G.~Lenzen$^{\rm 176}$,
B.~Lenzi$^{\rm 30}$,
R.~Leone$^{\rm 7}$,
S.~Leone$^{\rm 124a,124b}$,
C.~Leonidopoulos$^{\rm 46}$,
S.~Leontsinis$^{\rm 10}$,
C.~Leroy$^{\rm 95}$,
C.G.~Lester$^{\rm 28}$,
C.M.~Lester$^{\rm 122}$,
M.~Levchenko$^{\rm 123}$,
J.~Lev\^eque$^{\rm 5}$,
D.~Levin$^{\rm 89}$,
L.J.~Levinson$^{\rm 173}$,
M.~Levy$^{\rm 18}$,
A.~Lewis$^{\rm 120}$,
G.H.~Lewis$^{\rm 110}$,
A.M.~Leyko$^{\rm 21}$,
M.~Leyton$^{\rm 41}$,
B.~Li$^{\rm 33b}$$^{,t}$,
B.~Li$^{\rm 85}$,
H.~Li$^{\rm 149}$,
H.L.~Li$^{\rm 31}$,
L.~Li$^{\rm 45}$,
L.~Li$^{\rm 33e}$,
S.~Li$^{\rm 45}$,
Y.~Li$^{\rm 33c}$$^{,u}$,
Z.~Liang$^{\rm 138}$,
H.~Liao$^{\rm 34}$,
B.~Liberti$^{\rm 134a}$,
P.~Lichard$^{\rm 30}$,
K.~Lie$^{\rm 166}$,
J.~Liebal$^{\rm 21}$,
W.~Liebig$^{\rm 14}$,
C.~Limbach$^{\rm 21}$,
A.~Limosani$^{\rm 151}$,
S.C.~Lin$^{\rm 152}$$^{,v}$,
T.H.~Lin$^{\rm 83}$,
F.~Linde$^{\rm 107}$,
B.E.~Lindquist$^{\rm 149}$,
J.T.~Linnemann$^{\rm 90}$,
E.~Lipeles$^{\rm 122}$,
A.~Lipniacka$^{\rm 14}$,
M.~Lisovyi$^{\rm 42}$,
T.M.~Liss$^{\rm 166}$,
D.~Lissauer$^{\rm 25}$,
A.~Lister$^{\rm 169}$,
A.M.~Litke$^{\rm 138}$,
B.~Liu$^{\rm 152}$,
D.~Liu$^{\rm 152}$,
J.B.~Liu$^{\rm 33b}$,
K.~Liu$^{\rm 33b}$$^{,w}$,
L.~Liu$^{\rm 89}$,
M.~Liu$^{\rm 45}$,
M.~Liu$^{\rm 33b}$,
Y.~Liu$^{\rm 33b}$,
M.~Livan$^{\rm 121a,121b}$,
A.~Lleres$^{\rm 55}$,
J.~Llorente~Merino$^{\rm 82}$,
S.L.~Lloyd$^{\rm 76}$,
F.~Lo~Sterzo$^{\rm 152}$,
E.~Lobodzinska$^{\rm 42}$,
P.~Loch$^{\rm 7}$,
W.S.~Lockman$^{\rm 138}$,
F.K.~Loebinger$^{\rm 84}$,
A.E.~Loevschall-Jensen$^{\rm 36}$,
A.~Loginov$^{\rm 177}$,
T.~Lohse$^{\rm 16}$,
K.~Lohwasser$^{\rm 42}$,
M.~Lokajicek$^{\rm 127}$,
V.P.~Lombardo$^{\rm 5}$,
B.A.~Long$^{\rm 22}$,
J.D.~Long$^{\rm 89}$,
R.E.~Long$^{\rm 72}$,
L.~Lopes$^{\rm 126a}$,
D.~Lopez~Mateos$^{\rm 57}$,
B.~Lopez~Paredes$^{\rm 140}$,
I.~Lopez~Paz$^{\rm 12}$,
J.~Lorenz$^{\rm 100}$,
N.~Lorenzo~Martinez$^{\rm 61}$,
M.~Losada$^{\rm 163}$,
P.~Loscutoff$^{\rm 15}$,
X.~Lou$^{\rm 41}$,
A.~Lounis$^{\rm 117}$,
J.~Love$^{\rm 6}$,
P.A.~Love$^{\rm 72}$,
A.J.~Lowe$^{\rm 144}$$^{,f}$,
F.~Lu$^{\rm 33a}$,
N.~Lu$^{\rm 89}$,
H.J.~Lubatti$^{\rm 139}$,
C.~Luci$^{\rm 133a,133b}$,
A.~Lucotte$^{\rm 55}$,
F.~Luehring$^{\rm 61}$,
W.~Lukas$^{\rm 62}$,
L.~Luminari$^{\rm 133a}$,
O.~Lundberg$^{\rm 147a,147b}$,
B.~Lund-Jensen$^{\rm 148}$,
M.~Lungwitz$^{\rm 83}$,
D.~Lynn$^{\rm 25}$,
R.~Lysak$^{\rm 127}$,
E.~Lytken$^{\rm 81}$,
H.~Ma$^{\rm 25}$,
L.L.~Ma$^{\rm 33d}$,
G.~Maccarrone$^{\rm 47}$,
A.~Macchiolo$^{\rm 101}$,
J.~Machado~Miguens$^{\rm 126a,126b}$,
D.~Macina$^{\rm 30}$,
D.~Madaffari$^{\rm 85}$,
R.~Madar$^{\rm 48}$,
H.J.~Maddocks$^{\rm 72}$,
W.F.~Mader$^{\rm 44}$,
A.~Madsen$^{\rm 167}$,
M.~Maeno$^{\rm 8}$,
T.~Maeno$^{\rm 25}$,
A.~Maevskiy$^{\rm 99}$,
E.~Magradze$^{\rm 54}$,
K.~Mahboubi$^{\rm 48}$,
J.~Mahlstedt$^{\rm 107}$,
S.~Mahmoud$^{\rm 74}$,
C.~Maiani$^{\rm 137}$,
C.~Maidantchik$^{\rm 24a}$,
A.A.~Maier$^{\rm 101}$,
A.~Maio$^{\rm 126a,126b,126d}$,
S.~Majewski$^{\rm 116}$,
Y.~Makida$^{\rm 66}$,
N.~Makovec$^{\rm 117}$,
P.~Mal$^{\rm 137}$$^{,x}$,
B.~Malaescu$^{\rm 80}$,
Pa.~Malecki$^{\rm 39}$,
V.P.~Maleev$^{\rm 123}$,
F.~Malek$^{\rm 55}$,
U.~Mallik$^{\rm 63}$,
D.~Malon$^{\rm 6}$,
C.~Malone$^{\rm 144}$,
S.~Maltezos$^{\rm 10}$,
V.M.~Malyshev$^{\rm 109}$,
S.~Malyukov$^{\rm 30}$,
J.~Mamuzic$^{\rm 13b}$,
B.~Mandelli$^{\rm 30}$,
L.~Mandelli$^{\rm 91a}$,
I.~Mandi\'{c}$^{\rm 75}$,
R.~Mandrysch$^{\rm 63}$,
J.~Maneira$^{\rm 126a,126b}$,
A.~Manfredini$^{\rm 101}$,
L.~Manhaes~de~Andrade~Filho$^{\rm 24b}$,
J.A.~Manjarres~Ramos$^{\rm 160b}$,
A.~Mann$^{\rm 100}$,
P.M.~Manning$^{\rm 138}$,
A.~Manousakis-Katsikakis$^{\rm 9}$,
B.~Mansoulie$^{\rm 137}$,
R.~Mantifel$^{\rm 87}$,
L.~Mapelli$^{\rm 30}$,
L.~March$^{\rm 146c}$,
J.F.~Marchand$^{\rm 29}$,
G.~Marchiori$^{\rm 80}$,
M.~Marcisovsky$^{\rm 127}$,
C.P.~Marino$^{\rm 170}$,
M.~Marjanovic$^{\rm 13a}$,
F.~Marroquim$^{\rm 24a}$,
S.P.~Marsden$^{\rm 84}$,
Z.~Marshall$^{\rm 15}$,
L.F.~Marti$^{\rm 17}$,
S.~Marti-Garcia$^{\rm 168}$,
B.~Martin$^{\rm 30}$,
B.~Martin$^{\rm 90}$,
T.A.~Martin$^{\rm 171}$,
V.J.~Martin$^{\rm 46}$,
B.~Martin~dit~Latour$^{\rm 14}$,
H.~Martinez$^{\rm 137}$,
M.~Martinez$^{\rm 12}$$^{,n}$,
S.~Martin-Haugh$^{\rm 131}$,
A.C.~Martyniuk$^{\rm 78}$,
M.~Marx$^{\rm 139}$,
F.~Marzano$^{\rm 133a}$,
A.~Marzin$^{\rm 30}$,
L.~Masetti$^{\rm 83}$,
T.~Mashimo$^{\rm 156}$,
R.~Mashinistov$^{\rm 96}$,
J.~Masik$^{\rm 84}$,
A.L.~Maslennikov$^{\rm 109}$$^{,c}$,
I.~Massa$^{\rm 20a,20b}$,
L.~Massa$^{\rm 20a,20b}$,
N.~Massol$^{\rm 5}$,
P.~Mastrandrea$^{\rm 149}$,
A.~Mastroberardino$^{\rm 37a,37b}$,
T.~Masubuchi$^{\rm 156}$,
P.~M\"attig$^{\rm 176}$,
J.~Mattmann$^{\rm 83}$,
J.~Maurer$^{\rm 26a}$,
S.J.~Maxfield$^{\rm 74}$,
D.A.~Maximov$^{\rm 109}$$^{,c}$,
R.~Mazini$^{\rm 152}$,
L.~Mazzaferro$^{\rm 134a,134b}$,
G.~Mc~Goldrick$^{\rm 159}$,
S.P.~Mc~Kee$^{\rm 89}$,
A.~McCarn$^{\rm 89}$,
R.L.~McCarthy$^{\rm 149}$,
T.G.~McCarthy$^{\rm 29}$,
N.A.~McCubbin$^{\rm 131}$,
K.W.~McFarlane$^{\rm 56}$$^{,*}$,
J.A.~Mcfayden$^{\rm 78}$,
G.~Mchedlidze$^{\rm 54}$,
S.J.~McMahon$^{\rm 131}$,
R.A.~McPherson$^{\rm 170}$$^{,k}$,
J.~Mechnich$^{\rm 107}$,
M.~Medinnis$^{\rm 42}$,
S.~Meehan$^{\rm 31}$,
S.~Mehlhase$^{\rm 100}$,
A.~Mehta$^{\rm 74}$,
K.~Meier$^{\rm 58a}$,
C.~Meineck$^{\rm 100}$,
B.~Meirose$^{\rm 41}$,
C.~Melachrinos$^{\rm 31}$,
B.R.~Mellado~Garcia$^{\rm 146c}$,
F.~Meloni$^{\rm 17}$,
A.~Mengarelli$^{\rm 20a,20b}$,
S.~Menke$^{\rm 101}$,
E.~Meoni$^{\rm 162}$,
K.M.~Mercurio$^{\rm 57}$,
S.~Mergelmeyer$^{\rm 21}$,
N.~Meric$^{\rm 137}$,
P.~Mermod$^{\rm 49}$,
L.~Merola$^{\rm 104a,104b}$,
C.~Meroni$^{\rm 91a}$,
F.S.~Merritt$^{\rm 31}$,
H.~Merritt$^{\rm 111}$,
A.~Messina$^{\rm 30}$$^{,y}$,
J.~Metcalfe$^{\rm 25}$,
A.S.~Mete$^{\rm 164}$,
C.~Meyer$^{\rm 83}$,
C.~Meyer$^{\rm 122}$,
J-P.~Meyer$^{\rm 137}$,
J.~Meyer$^{\rm 30}$,
R.P.~Middleton$^{\rm 131}$,
S.~Migas$^{\rm 74}$,
S.~Miglioranzi$^{\rm 165a,165c}$,
L.~Mijovi\'{c}$^{\rm 21}$,
G.~Mikenberg$^{\rm 173}$,
M.~Mikestikova$^{\rm 127}$,
M.~Miku\v{z}$^{\rm 75}$,
A.~Milic$^{\rm 30}$,
D.W.~Miller$^{\rm 31}$,
C.~Mills$^{\rm 46}$,
A.~Milov$^{\rm 173}$,
D.A.~Milstead$^{\rm 147a,147b}$,
A.A.~Minaenko$^{\rm 130}$,
Y.~Minami$^{\rm 156}$,
I.A.~Minashvili$^{\rm 65}$,
A.I.~Mincer$^{\rm 110}$,
B.~Mindur$^{\rm 38a}$,
M.~Mineev$^{\rm 65}$,
Y.~Ming$^{\rm 174}$,
L.M.~Mir$^{\rm 12}$,
G.~Mirabelli$^{\rm 133a}$,
T.~Mitani$^{\rm 172}$,
J.~Mitrevski$^{\rm 100}$,
V.A.~Mitsou$^{\rm 168}$,
A.~Miucci$^{\rm 49}$,
P.S.~Miyagawa$^{\rm 140}$,
J.U.~Mj\"ornmark$^{\rm 81}$,
T.~Moa$^{\rm 147a,147b}$,
K.~Mochizuki$^{\rm 85}$,
S.~Mohapatra$^{\rm 35}$,
W.~Mohr$^{\rm 48}$,
S.~Molander$^{\rm 147a,147b}$,
R.~Moles-Valls$^{\rm 168}$,
K.~M\"onig$^{\rm 42}$,
C.~Monini$^{\rm 55}$,
J.~Monk$^{\rm 36}$,
E.~Monnier$^{\rm 85}$,
J.~Montejo~Berlingen$^{\rm 12}$,
F.~Monticelli$^{\rm 71}$,
S.~Monzani$^{\rm 133a,133b}$,
R.W.~Moore$^{\rm 3}$,
N.~Morange$^{\rm 63}$,
D.~Moreno$^{\rm 163}$,
M.~Moreno~Ll\'acer$^{\rm 54}$,
P.~Morettini$^{\rm 50a}$,
M.~Morgenstern$^{\rm 44}$,
M.~Morii$^{\rm 57}$,
V.~Morisbak$^{\rm 119}$,
S.~Moritz$^{\rm 83}$,
A.K.~Morley$^{\rm 148}$,
G.~Mornacchi$^{\rm 30}$,
J.D.~Morris$^{\rm 76}$,
A.~Morton$^{\rm 42}$,
L.~Morvaj$^{\rm 103}$,
H.G.~Moser$^{\rm 101}$,
M.~Mosidze$^{\rm 51b}$,
J.~Moss$^{\rm 111}$,
K.~Motohashi$^{\rm 158}$,
R.~Mount$^{\rm 144}$,
E.~Mountricha$^{\rm 25}$,
S.V.~Mouraviev$^{\rm 96}$$^{,*}$,
E.J.W.~Moyse$^{\rm 86}$,
S.~Muanza$^{\rm 85}$,
R.D.~Mudd$^{\rm 18}$,
F.~Mueller$^{\rm 58a}$,
J.~Mueller$^{\rm 125}$,
K.~Mueller$^{\rm 21}$,
T.~Mueller$^{\rm 28}$,
T.~Mueller$^{\rm 83}$,
D.~Muenstermann$^{\rm 49}$,
Y.~Munwes$^{\rm 154}$,
J.A.~Murillo~Quijada$^{\rm 18}$,
W.J.~Murray$^{\rm 171,131}$,
H.~Musheghyan$^{\rm 54}$,
E.~Musto$^{\rm 153}$,
A.G.~Myagkov$^{\rm 130}$$^{,z}$,
M.~Myska$^{\rm 128}$,
O.~Nackenhorst$^{\rm 54}$,
J.~Nadal$^{\rm 54}$,
K.~Nagai$^{\rm 120}$,
R.~Nagai$^{\rm 158}$,
Y.~Nagai$^{\rm 85}$,
K.~Nagano$^{\rm 66}$,
A.~Nagarkar$^{\rm 111}$,
Y.~Nagasaka$^{\rm 59}$,
K.~Nagata$^{\rm 161}$,
M.~Nagel$^{\rm 101}$,
A.M.~Nairz$^{\rm 30}$,
Y.~Nakahama$^{\rm 30}$,
K.~Nakamura$^{\rm 66}$,
T.~Nakamura$^{\rm 156}$,
I.~Nakano$^{\rm 112}$,
H.~Namasivayam$^{\rm 41}$,
G.~Nanava$^{\rm 21}$,
R.F.~Naranjo~Garcia$^{\rm 42}$,
R.~Narayan$^{\rm 58b}$,
T.~Nattermann$^{\rm 21}$,
T.~Naumann$^{\rm 42}$,
G.~Navarro$^{\rm 163}$,
R.~Nayyar$^{\rm 7}$,
H.A.~Neal$^{\rm 89}$,
P.Yu.~Nechaeva$^{\rm 96}$,
T.J.~Neep$^{\rm 84}$,
P.D.~Nef$^{\rm 144}$,
A.~Negri$^{\rm 121a,121b}$,
G.~Negri$^{\rm 30}$,
M.~Negrini$^{\rm 20a}$,
S.~Nektarijevic$^{\rm 49}$,
C.~Nellist$^{\rm 117}$,
A.~Nelson$^{\rm 164}$,
T.K.~Nelson$^{\rm 144}$,
S.~Nemecek$^{\rm 127}$,
P.~Nemethy$^{\rm 110}$,
A.A.~Nepomuceno$^{\rm 24a}$,
M.~Nessi$^{\rm 30}$$^{,aa}$,
M.S.~Neubauer$^{\rm 166}$,
M.~Neumann$^{\rm 176}$,
R.M.~Neves$^{\rm 110}$,
P.~Nevski$^{\rm 25}$,
P.R.~Newman$^{\rm 18}$,
D.H.~Nguyen$^{\rm 6}$,
R.B.~Nickerson$^{\rm 120}$,
R.~Nicolaidou$^{\rm 137}$,
B.~Nicquevert$^{\rm 30}$,
J.~Nielsen$^{\rm 138}$,
N.~Nikiforou$^{\rm 35}$,
A.~Nikiforov$^{\rm 16}$,
V.~Nikolaenko$^{\rm 130}$$^{,z}$,
I.~Nikolic-Audit$^{\rm 80}$,
K.~Nikolics$^{\rm 49}$,
K.~Nikolopoulos$^{\rm 18}$,
P.~Nilsson$^{\rm 25}$,
Y.~Ninomiya$^{\rm 156}$,
A.~Nisati$^{\rm 133a}$,
R.~Nisius$^{\rm 101}$,
T.~Nobe$^{\rm 158}$,
M.~Nomachi$^{\rm 118}$,
I.~Nomidis$^{\rm 29}$,
S.~Norberg$^{\rm 113}$,
M.~Nordberg$^{\rm 30}$,
O.~Novgorodova$^{\rm 44}$,
S.~Nowak$^{\rm 101}$,
M.~Nozaki$^{\rm 66}$,
L.~Nozka$^{\rm 115}$,
K.~Ntekas$^{\rm 10}$,
G.~Nunes~Hanninger$^{\rm 88}$,
T.~Nunnemann$^{\rm 100}$,
E.~Nurse$^{\rm 78}$,
F.~Nuti$^{\rm 88}$,
B.J.~O'Brien$^{\rm 46}$,
F.~O'grady$^{\rm 7}$,
D.C.~O'Neil$^{\rm 143}$,
V.~O'Shea$^{\rm 53}$,
F.G.~Oakham$^{\rm 29}$$^{,e}$,
H.~Oberlack$^{\rm 101}$,
T.~Obermann$^{\rm 21}$,
J.~Ocariz$^{\rm 80}$,
A.~Ochi$^{\rm 67}$,
I.~Ochoa$^{\rm 78}$,
S.~Oda$^{\rm 70}$,
S.~Odaka$^{\rm 66}$,
H.~Ogren$^{\rm 61}$,
A.~Oh$^{\rm 84}$,
S.H.~Oh$^{\rm 45}$,
C.C.~Ohm$^{\rm 15}$,
H.~Ohman$^{\rm 167}$,
H.~Oide$^{\rm 30}$,
W.~Okamura$^{\rm 118}$,
H.~Okawa$^{\rm 161}$,
Y.~Okumura$^{\rm 31}$,
T.~Okuyama$^{\rm 156}$,
A.~Olariu$^{\rm 26a}$,
A.G.~Olchevski$^{\rm 65}$,
S.A.~Olivares~Pino$^{\rm 46}$,
D.~Oliveira~Damazio$^{\rm 25}$,
E.~Oliver~Garcia$^{\rm 168}$,
A.~Olszewski$^{\rm 39}$,
J.~Olszowska$^{\rm 39}$,
A.~Onofre$^{\rm 126a,126e}$,
P.U.E.~Onyisi$^{\rm 31}$$^{,o}$,
C.J.~Oram$^{\rm 160a}$,
M.J.~Oreglia$^{\rm 31}$,
Y.~Oren$^{\rm 154}$,
D.~Orestano$^{\rm 135a,135b}$,
N.~Orlando$^{\rm 73a,73b}$,
C.~Oropeza~Barrera$^{\rm 53}$,
R.S.~Orr$^{\rm 159}$,
B.~Osculati$^{\rm 50a,50b}$,
R.~Ospanov$^{\rm 122}$,
G.~Otero~y~Garzon$^{\rm 27}$,
H.~Otono$^{\rm 70}$,
M.~Ouchrif$^{\rm 136d}$,
E.A.~Ouellette$^{\rm 170}$,
F.~Ould-Saada$^{\rm 119}$,
A.~Ouraou$^{\rm 137}$,
K.P.~Oussoren$^{\rm 107}$,
Q.~Ouyang$^{\rm 33a}$,
A.~Ovcharova$^{\rm 15}$,
M.~Owen$^{\rm 84}$,
V.E.~Ozcan$^{\rm 19a}$,
N.~Ozturk$^{\rm 8}$,
K.~Pachal$^{\rm 120}$,
A.~Pacheco~Pages$^{\rm 12}$,
C.~Padilla~Aranda$^{\rm 12}$,
M.~Pag\'{a}\v{c}ov\'{a}$^{\rm 48}$,
S.~Pagan~Griso$^{\rm 15}$,
E.~Paganis$^{\rm 140}$,
C.~Pahl$^{\rm 101}$,
F.~Paige$^{\rm 25}$,
P.~Pais$^{\rm 86}$,
K.~Pajchel$^{\rm 119}$,
G.~Palacino$^{\rm 160b}$,
S.~Palestini$^{\rm 30}$,
M.~Palka$^{\rm 38b}$,
D.~Pallin$^{\rm 34}$,
A.~Palma$^{\rm 126a,126b}$,
J.D.~Palmer$^{\rm 18}$,
Y.B.~Pan$^{\rm 174}$,
E.~Panagiotopoulou$^{\rm 10}$,
J.G.~Panduro~Vazquez$^{\rm 77}$,
P.~Pani$^{\rm 107}$,
N.~Panikashvili$^{\rm 89}$,
S.~Panitkin$^{\rm 25}$,
D.~Pantea$^{\rm 26a}$,
L.~Paolozzi$^{\rm 134a,134b}$,
Th.D.~Papadopoulou$^{\rm 10}$,
K.~Papageorgiou$^{\rm 155}$,
A.~Paramonov$^{\rm 6}$,
D.~Paredes~Hernandez$^{\rm 155}$,
M.A.~Parker$^{\rm 28}$,
F.~Parodi$^{\rm 50a,50b}$,
J.A.~Parsons$^{\rm 35}$,
U.~Parzefall$^{\rm 48}$,
E.~Pasqualucci$^{\rm 133a}$,
S.~Passaggio$^{\rm 50a}$,
A.~Passeri$^{\rm 135a}$,
F.~Pastore$^{\rm 135a,135b}$$^{,*}$,
Fr.~Pastore$^{\rm 77}$,
G.~P\'asztor$^{\rm 29}$,
S.~Pataraia$^{\rm 176}$,
N.D.~Patel$^{\rm 151}$,
J.R.~Pater$^{\rm 84}$,
S.~Patricelli$^{\rm 104a,104b}$,
T.~Pauly$^{\rm 30}$,
J.~Pearce$^{\rm 170}$,
L.E.~Pedersen$^{\rm 36}$,
M.~Pedersen$^{\rm 119}$,
S.~Pedraza~Lopez$^{\rm 168}$,
R.~Pedro$^{\rm 126a,126b}$,
S.V.~Peleganchuk$^{\rm 109}$,
D.~Pelikan$^{\rm 167}$,
H.~Peng$^{\rm 33b}$,
B.~Penning$^{\rm 31}$,
J.~Penwell$^{\rm 61}$,
D.V.~Perepelitsa$^{\rm 25}$,
E.~Perez~Codina$^{\rm 160a}$,
M.T.~P\'erez~Garc\'ia-Esta\~n$^{\rm 168}$,
L.~Perini$^{\rm 91a,91b}$,
H.~Pernegger$^{\rm 30}$,
S.~Perrella$^{\rm 104a,104b}$,
R.~Peschke$^{\rm 42}$,
V.D.~Peshekhonov$^{\rm 65}$,
K.~Peters$^{\rm 30}$,
R.F.Y.~Peters$^{\rm 84}$,
B.A.~Petersen$^{\rm 30}$,
T.C.~Petersen$^{\rm 36}$,
E.~Petit$^{\rm 42}$,
A.~Petridis$^{\rm 147a,147b}$,
C.~Petridou$^{\rm 155}$,
E.~Petrolo$^{\rm 133a}$,
F.~Petrucci$^{\rm 135a,135b}$,
N.E.~Pettersson$^{\rm 158}$,
R.~Pezoa$^{\rm 32b}$,
P.W.~Phillips$^{\rm 131}$,
G.~Piacquadio$^{\rm 144}$,
E.~Pianori$^{\rm 171}$,
A.~Picazio$^{\rm 49}$,
E.~Piccaro$^{\rm 76}$,
M.~Piccinini$^{\rm 20a,20b}$,
M.A.~Pickering$^{\rm 120}$,
R.~Piegaia$^{\rm 27}$,
D.T.~Pignotti$^{\rm 111}$,
J.E.~Pilcher$^{\rm 31}$,
A.D.~Pilkington$^{\rm 78}$,
J.~Pina$^{\rm 126a,126b,126d}$,
M.~Pinamonti$^{\rm 165a,165c}$$^{,ab}$,
A.~Pinder$^{\rm 120}$,
J.L.~Pinfold$^{\rm 3}$,
A.~Pingel$^{\rm 36}$,
B.~Pinto$^{\rm 126a}$,
S.~Pires$^{\rm 80}$,
M.~Pitt$^{\rm 173}$,
C.~Pizio$^{\rm 91a,91b}$,
L.~Plazak$^{\rm 145a}$,
M.-A.~Pleier$^{\rm 25}$,
V.~Pleskot$^{\rm 129}$,
E.~Plotnikova$^{\rm 65}$,
P.~Plucinski$^{\rm 147a,147b}$,
D.~Pluth$^{\rm 64}$,
S.~Poddar$^{\rm 58a}$,
F.~Podlyski$^{\rm 34}$,
R.~Poettgen$^{\rm 83}$,
L.~Poggioli$^{\rm 117}$,
D.~Pohl$^{\rm 21}$,
M.~Pohl$^{\rm 49}$,
G.~Polesello$^{\rm 121a}$,
A.~Policicchio$^{\rm 37a,37b}$,
R.~Polifka$^{\rm 159}$,
A.~Polini$^{\rm 20a}$,
C.S.~Pollard$^{\rm 53}$,
V.~Polychronakos$^{\rm 25}$,
K.~Pomm\`es$^{\rm 30}$,
L.~Pontecorvo$^{\rm 133a}$,
B.G.~Pope$^{\rm 90}$,
G.A.~Popeneciu$^{\rm 26b}$,
D.S.~Popovic$^{\rm 13a}$,
A.~Poppleton$^{\rm 30}$,
X.~Portell~Bueso$^{\rm 12}$,
S.~Pospisil$^{\rm 128}$,
K.~Potamianos$^{\rm 15}$,
I.N.~Potrap$^{\rm 65}$,
C.J.~Potter$^{\rm 150}$,
C.T.~Potter$^{\rm 116}$,
G.~Poulard$^{\rm 30}$,
J.~Poveda$^{\rm 61}$,
V.~Pozdnyakov$^{\rm 65}$,
P.~Pralavorio$^{\rm 85}$,
A.~Pranko$^{\rm 15}$,
S.~Prasad$^{\rm 30}$,
R.~Pravahan$^{\rm 8}$,
S.~Prell$^{\rm 64}$,
D.~Price$^{\rm 84}$,
J.~Price$^{\rm 74}$,
L.E.~Price$^{\rm 6}$,
D.~Prieur$^{\rm 125}$,
M.~Primavera$^{\rm 73a}$,
S.~Prince$^{\rm 87}$,
M.~Proissl$^{\rm 46}$,
K.~Prokofiev$^{\rm 47}$,
F.~Prokoshin$^{\rm 32b}$,
E.~Protopapadaki$^{\rm 137}$,
S.~Protopopescu$^{\rm 25}$,
J.~Proudfoot$^{\rm 6}$,
M.~Przybycien$^{\rm 38a}$,
H.~Przysiezniak$^{\rm 5}$,
E.~Ptacek$^{\rm 116}$,
D.~Puddu$^{\rm 135a,135b}$,
E.~Pueschel$^{\rm 86}$,
D.~Puldon$^{\rm 149}$,
M.~Purohit$^{\rm 25}$$^{,ac}$,
P.~Puzo$^{\rm 117}$,
J.~Qian$^{\rm 89}$,
G.~Qin$^{\rm 53}$,
Y.~Qin$^{\rm 84}$,
A.~Quadt$^{\rm 54}$,
D.R.~Quarrie$^{\rm 15}$,
W.B.~Quayle$^{\rm 165a,165b}$,
M.~Queitsch-Maitland$^{\rm 84}$,
D.~Quilty$^{\rm 53}$,
A.~Qureshi$^{\rm 160b}$,
V.~Radeka$^{\rm 25}$,
V.~Radescu$^{\rm 42}$,
S.K.~Radhakrishnan$^{\rm 149}$,
P.~Radloff$^{\rm 116}$,
P.~Rados$^{\rm 88}$,
F.~Ragusa$^{\rm 91a,91b}$,
G.~Rahal$^{\rm 179}$,
S.~Rajagopalan$^{\rm 25}$,
M.~Rammensee$^{\rm 30}$,
C.~Rangel-Smith$^{\rm 167}$,
K.~Rao$^{\rm 164}$,
F.~Rauscher$^{\rm 100}$,
T.C.~Rave$^{\rm 48}$,
T.~Ravenscroft$^{\rm 53}$,
M.~Raymond$^{\rm 30}$,
A.L.~Read$^{\rm 119}$,
N.P.~Readioff$^{\rm 74}$,
D.M.~Rebuzzi$^{\rm 121a,121b}$,
A.~Redelbach$^{\rm 175}$,
G.~Redlinger$^{\rm 25}$,
R.~Reece$^{\rm 138}$,
K.~Reeves$^{\rm 41}$,
L.~Rehnisch$^{\rm 16}$,
H.~Reisin$^{\rm 27}$,
M.~Relich$^{\rm 164}$,
C.~Rembser$^{\rm 30}$,
H.~Ren$^{\rm 33a}$,
Z.L.~Ren$^{\rm 152}$,
A.~Renaud$^{\rm 117}$,
M.~Rescigno$^{\rm 133a}$,
S.~Resconi$^{\rm 91a}$,
O.L.~Rezanova$^{\rm 109}$$^{,c}$,
P.~Reznicek$^{\rm 129}$,
R.~Rezvani$^{\rm 95}$,
R.~Richter$^{\rm 101}$,
M.~Ridel$^{\rm 80}$,
P.~Rieck$^{\rm 16}$,
J.~Rieger$^{\rm 54}$,
M.~Rijssenbeek$^{\rm 149}$,
A.~Rimoldi$^{\rm 121a,121b}$,
L.~Rinaldi$^{\rm 20a}$,
E.~Ritsch$^{\rm 62}$,
I.~Riu$^{\rm 12}$,
F.~Rizatdinova$^{\rm 114}$,
E.~Rizvi$^{\rm 76}$,
S.H.~Robertson$^{\rm 87}$$^{,k}$,
A.~Robichaud-Veronneau$^{\rm 87}$,
D.~Robinson$^{\rm 28}$,
J.E.M.~Robinson$^{\rm 84}$,
A.~Robson$^{\rm 53}$,
C.~Roda$^{\rm 124a,124b}$,
L.~Rodrigues$^{\rm 30}$,
S.~Roe$^{\rm 30}$,
O.~R{\o}hne$^{\rm 119}$,
S.~Rolli$^{\rm 162}$,
A.~Romaniouk$^{\rm 98}$,
M.~Romano$^{\rm 20a,20b}$,
E.~Romero~Adam$^{\rm 168}$,
N.~Rompotis$^{\rm 139}$,
M.~Ronzani$^{\rm 48}$,
L.~Roos$^{\rm 80}$,
E.~Ros$^{\rm 168}$,
S.~Rosati$^{\rm 133a}$,
K.~Rosbach$^{\rm 49}$,
M.~Rose$^{\rm 77}$,
P.~Rose$^{\rm 138}$,
P.L.~Rosendahl$^{\rm 14}$,
O.~Rosenthal$^{\rm 142}$,
V.~Rossetti$^{\rm 147a,147b}$,
E.~Rossi$^{\rm 104a,104b}$,
L.P.~Rossi$^{\rm 50a}$,
R.~Rosten$^{\rm 139}$,
M.~Rotaru$^{\rm 26a}$,
I.~Roth$^{\rm 173}$,
J.~Rothberg$^{\rm 139}$,
D.~Rousseau$^{\rm 117}$,
C.R.~Royon$^{\rm 137}$,
A.~Rozanov$^{\rm 85}$,
Y.~Rozen$^{\rm 153}$,
X.~Ruan$^{\rm 146c}$,
F.~Rubbo$^{\rm 12}$,
I.~Rubinskiy$^{\rm 42}$,
V.I.~Rud$^{\rm 99}$,
C.~Rudolph$^{\rm 44}$,
M.S.~Rudolph$^{\rm 159}$,
F.~R\"uhr$^{\rm 48}$,
A.~Ruiz-Martinez$^{\rm 30}$,
Z.~Rurikova$^{\rm 48}$,
N.A.~Rusakovich$^{\rm 65}$,
A.~Ruschke$^{\rm 100}$,
H.L.~Russell$^{\rm 139}$,
J.P.~Rutherfoord$^{\rm 7}$,
N.~Ruthmann$^{\rm 48}$,
Y.F.~Ryabov$^{\rm 123}$,
M.~Rybar$^{\rm 129}$,
G.~Rybkin$^{\rm 117}$,
N.C.~Ryder$^{\rm 120}$,
A.F.~Saavedra$^{\rm 151}$,
G.~Sabato$^{\rm 107}$,
S.~Sacerdoti$^{\rm 27}$,
A.~Saddique$^{\rm 3}$,
I.~Sadeh$^{\rm 154}$,
H.F-W.~Sadrozinski$^{\rm 138}$,
R.~Sadykov$^{\rm 65}$,
F.~Safai~Tehrani$^{\rm 133a}$,
H.~Sakamoto$^{\rm 156}$,
Y.~Sakurai$^{\rm 172}$,
G.~Salamanna$^{\rm 135a,135b}$,
A.~Salamon$^{\rm 134a}$,
M.~Saleem$^{\rm 113}$,
D.~Salek$^{\rm 107}$,
P.H.~Sales~De~Bruin$^{\rm 139}$,
D.~Salihagic$^{\rm 101}$,
A.~Salnikov$^{\rm 144}$,
J.~Salt$^{\rm 168}$,
D.~Salvatore$^{\rm 37a,37b}$,
F.~Salvatore$^{\rm 150}$,
A.~Salvucci$^{\rm 106}$,
A.~Salzburger$^{\rm 30}$,
D.~Sampsonidis$^{\rm 155}$,
A.~Sanchez$^{\rm 104a,104b}$,
J.~S\'anchez$^{\rm 168}$,
V.~Sanchez~Martinez$^{\rm 168}$,
H.~Sandaker$^{\rm 14}$,
R.L.~Sandbach$^{\rm 76}$,
H.G.~Sander$^{\rm 83}$,
M.P.~Sanders$^{\rm 100}$,
M.~Sandhoff$^{\rm 176}$,
T.~Sandoval$^{\rm 28}$,
C.~Sandoval$^{\rm 163}$,
R.~Sandstroem$^{\rm 101}$,
D.P.C.~Sankey$^{\rm 131}$,
A.~Sansoni$^{\rm 47}$,
C.~Santoni$^{\rm 34}$,
R.~Santonico$^{\rm 134a,134b}$,
H.~Santos$^{\rm 126a}$,
I.~Santoyo~Castillo$^{\rm 150}$,
K.~Sapp$^{\rm 125}$,
A.~Sapronov$^{\rm 65}$,
J.G.~Saraiva$^{\rm 126a,126d}$,
B.~Sarrazin$^{\rm 21}$,
G.~Sartisohn$^{\rm 176}$,
O.~Sasaki$^{\rm 66}$,
Y.~Sasaki$^{\rm 156}$,
G.~Sauvage$^{\rm 5}$$^{,*}$,
E.~Sauvan$^{\rm 5}$,
P.~Savard$^{\rm 159}$$^{,e}$,
D.O.~Savu$^{\rm 30}$,
C.~Sawyer$^{\rm 120}$,
L.~Sawyer$^{\rm 79}$$^{,m}$,
D.H.~Saxon$^{\rm 53}$,
J.~Saxon$^{\rm 31}$,
C.~Sbarra$^{\rm 20a}$,
A.~Sbrizzi$^{\rm 20a,20b}$,
T.~Scanlon$^{\rm 78}$,
D.A.~Scannicchio$^{\rm 164}$,
M.~Scarcella$^{\rm 151}$,
V.~Scarfone$^{\rm 37a,37b}$,
J.~Schaarschmidt$^{\rm 173}$,
P.~Schacht$^{\rm 101}$,
D.~Schaefer$^{\rm 30}$,
R.~Schaefer$^{\rm 42}$,
S.~Schaepe$^{\rm 21}$,
S.~Schaetzel$^{\rm 58b}$,
U.~Sch\"afer$^{\rm 83}$,
A.C.~Schaffer$^{\rm 117}$,
D.~Schaile$^{\rm 100}$,
R.D.~Schamberger$^{\rm 149}$,
V.~Scharf$^{\rm 58a}$,
V.A.~Schegelsky$^{\rm 123}$,
D.~Scheirich$^{\rm 129}$,
M.~Schernau$^{\rm 164}$,
M.I.~Scherzer$^{\rm 35}$,
C.~Schiavi$^{\rm 50a,50b}$,
J.~Schieck$^{\rm 100}$,
C.~Schillo$^{\rm 48}$,
M.~Schioppa$^{\rm 37a,37b}$,
S.~Schlenker$^{\rm 30}$,
E.~Schmidt$^{\rm 48}$,
K.~Schmieden$^{\rm 30}$,
C.~Schmitt$^{\rm 83}$,
S.~Schmitt$^{\rm 58b}$,
B.~Schneider$^{\rm 17}$,
Y.J.~Schnellbach$^{\rm 74}$,
U.~Schnoor$^{\rm 44}$,
L.~Schoeffel$^{\rm 137}$,
A.~Schoening$^{\rm 58b}$,
B.D.~Schoenrock$^{\rm 90}$,
A.L.S.~Schorlemmer$^{\rm 54}$,
M.~Schott$^{\rm 83}$,
D.~Schouten$^{\rm 160a}$,
J.~Schovancova$^{\rm 25}$,
S.~Schramm$^{\rm 159}$,
M.~Schreyer$^{\rm 175}$,
C.~Schroeder$^{\rm 83}$,
N.~Schuh$^{\rm 83}$,
M.J.~Schultens$^{\rm 21}$,
H.-C.~Schultz-Coulon$^{\rm 58a}$,
H.~Schulz$^{\rm 16}$,
M.~Schumacher$^{\rm 48}$,
B.A.~Schumm$^{\rm 138}$,
Ph.~Schune$^{\rm 137}$,
C.~Schwanenberger$^{\rm 84}$,
A.~Schwartzman$^{\rm 144}$,
T.A.~Schwarz$^{\rm 89}$,
Ph.~Schwegler$^{\rm 101}$,
Ph.~Schwemling$^{\rm 137}$,
R.~Schwienhorst$^{\rm 90}$,
J.~Schwindling$^{\rm 137}$,
T.~Schwindt$^{\rm 21}$,
M.~Schwoerer$^{\rm 5}$,
F.G.~Sciacca$^{\rm 17}$,
E.~Scifo$^{\rm 117}$,
G.~Sciolla$^{\rm 23}$,
F.~Scuri$^{\rm 124a,124b}$,
F.~Scutti$^{\rm 21}$,
J.~Searcy$^{\rm 89}$,
G.~Sedov$^{\rm 42}$,
E.~Sedykh$^{\rm 123}$,
P.~Seema$^{\rm 21}$,
S.C.~Seidel$^{\rm 105}$,
A.~Seiden$^{\rm 138}$,
F.~Seifert$^{\rm 128}$,
J.M.~Seixas$^{\rm 24a}$,
G.~Sekhniaidze$^{\rm 104a}$,
S.J.~Sekula$^{\rm 40}$,
K.E.~Selbach$^{\rm 46}$,
D.M.~Seliverstov$^{\rm 123}$$^{,*}$,
G.~Sellers$^{\rm 74}$,
N.~Semprini-Cesari$^{\rm 20a,20b}$,
C.~Serfon$^{\rm 30}$,
L.~Serin$^{\rm 117}$,
L.~Serkin$^{\rm 54}$,
T.~Serre$^{\rm 85}$,
R.~Seuster$^{\rm 160a}$,
H.~Severini$^{\rm 113}$,
T.~Sfiligoj$^{\rm 75}$,
F.~Sforza$^{\rm 101}$,
A.~Sfyrla$^{\rm 30}$,
E.~Shabalina$^{\rm 54}$,
M.~Shamim$^{\rm 116}$,
L.Y.~Shan$^{\rm 33a}$,
R.~Shang$^{\rm 166}$,
J.T.~Shank$^{\rm 22}$,
M.~Shapiro$^{\rm 15}$,
P.B.~Shatalov$^{\rm 97}$,
K.~Shaw$^{\rm 165a,165b}$,
C.Y.~Shehu$^{\rm 150}$,
P.~Sherwood$^{\rm 78}$,
L.~Shi$^{\rm 152}$$^{,ad}$,
S.~Shimizu$^{\rm 67}$,
C.O.~Shimmin$^{\rm 164}$,
M.~Shimojima$^{\rm 102}$,
M.~Shiyakova$^{\rm 65}$,
A.~Shmeleva$^{\rm 96}$,
D.~Shoaleh~Saadi$^{\rm 95}$,
M.J.~Shochet$^{\rm 31}$,
D.~Short$^{\rm 120}$,
S.~Shrestha$^{\rm 111}$,
E.~Shulga$^{\rm 98}$,
M.A.~Shupe$^{\rm 7}$,
S.~Shushkevich$^{\rm 42}$,
P.~Sicho$^{\rm 127}$,
O.~Sidiropoulou$^{\rm 155}$,
D.~Sidorov$^{\rm 114}$,
A.~Sidoti$^{\rm 133a}$,
F.~Siegert$^{\rm 44}$,
Dj.~Sijacki$^{\rm 13a}$,
J.~Silva$^{\rm 126a,126d}$,
Y.~Silver$^{\rm 154}$,
D.~Silverstein$^{\rm 144}$,
S.B.~Silverstein$^{\rm 147a}$,
V.~Simak$^{\rm 128}$,
O.~Simard$^{\rm 5}$,
Lj.~Simic$^{\rm 13a}$,
S.~Simion$^{\rm 117}$,
E.~Simioni$^{\rm 83}$,
B.~Simmons$^{\rm 78}$,
D.~Simon$^{\rm 34}$,
R.~Simoniello$^{\rm 91a,91b}$,
P.~Sinervo$^{\rm 159}$,
N.B.~Sinev$^{\rm 116}$,
G.~Siragusa$^{\rm 175}$,
A.~Sircar$^{\rm 79}$,
A.N.~Sisakyan$^{\rm 65}$$^{,*}$,
S.Yu.~Sivoklokov$^{\rm 99}$,
J.~Sj\"{o}lin$^{\rm 147a,147b}$,
T.B.~Sjursen$^{\rm 14}$,
H.P.~Skottowe$^{\rm 57}$,
P.~Skubic$^{\rm 113}$,
M.~Slater$^{\rm 18}$,
T.~Slavicek$^{\rm 128}$,
M.~Slawinska$^{\rm 107}$,
K.~Sliwa$^{\rm 162}$,
V.~Smakhtin$^{\rm 173}$,
B.H.~Smart$^{\rm 46}$,
L.~Smestad$^{\rm 14}$,
S.Yu.~Smirnov$^{\rm 98}$,
Y.~Smirnov$^{\rm 98}$,
L.N.~Smirnova$^{\rm 99}$$^{,ae}$,
O.~Smirnova$^{\rm 81}$,
K.M.~Smith$^{\rm 53}$,
M.~Smizanska$^{\rm 72}$,
K.~Smolek$^{\rm 128}$,
A.A.~Snesarev$^{\rm 96}$,
G.~Snidero$^{\rm 76}$,
S.~Snyder$^{\rm 25}$,
R.~Sobie$^{\rm 170}$$^{,k}$,
F.~Socher$^{\rm 44}$,
A.~Soffer$^{\rm 154}$,
D.A.~Soh$^{\rm 152}$$^{,ad}$,
C.A.~Solans$^{\rm 30}$,
M.~Solar$^{\rm 128}$,
J.~Solc$^{\rm 128}$,
E.Yu.~Soldatov$^{\rm 98}$,
U.~Soldevila$^{\rm 168}$,
A.A.~Solodkov$^{\rm 130}$,
A.~Soloshenko$^{\rm 65}$,
O.V.~Solovyanov$^{\rm 130}$,
V.~Solovyev$^{\rm 123}$,
P.~Sommer$^{\rm 48}$,
H.Y.~Song$^{\rm 33b}$,
N.~Soni$^{\rm 1}$,
A.~Sood$^{\rm 15}$,
A.~Sopczak$^{\rm 128}$,
B.~Sopko$^{\rm 128}$,
V.~Sopko$^{\rm 128}$,
V.~Sorin$^{\rm 12}$,
M.~Sosebee$^{\rm 8}$,
R.~Soualah$^{\rm 165a,165c}$,
P.~Soueid$^{\rm 95}$,
A.M.~Soukharev$^{\rm 109}$$^{,c}$,
D.~South$^{\rm 42}$,
S.~Spagnolo$^{\rm 73a,73b}$,
F.~Span\`o$^{\rm 77}$,
W.R.~Spearman$^{\rm 57}$,
F.~Spettel$^{\rm 101}$,
R.~Spighi$^{\rm 20a}$,
G.~Spigo$^{\rm 30}$,
L.A.~Spiller$^{\rm 88}$,
M.~Spousta$^{\rm 129}$,
T.~Spreitzer$^{\rm 159}$,
R.D.~St.~Denis$^{\rm 53}$$^{,*}$,
S.~Staerz$^{\rm 44}$,
J.~Stahlman$^{\rm 122}$,
R.~Stamen$^{\rm 58a}$,
S.~Stamm$^{\rm 16}$,
E.~Stanecka$^{\rm 39}$,
C.~Stanescu$^{\rm 135a}$,
M.~Stanescu-Bellu$^{\rm 42}$,
M.M.~Stanitzki$^{\rm 42}$,
S.~Stapnes$^{\rm 119}$,
E.A.~Starchenko$^{\rm 130}$,
J.~Stark$^{\rm 55}$,
P.~Staroba$^{\rm 127}$,
P.~Starovoitov$^{\rm 42}$,
R.~Staszewski$^{\rm 39}$,
P.~Stavina$^{\rm 145a}$$^{,*}$,
P.~Steinberg$^{\rm 25}$,
B.~Stelzer$^{\rm 143}$,
H.J.~Stelzer$^{\rm 30}$,
O.~Stelzer-Chilton$^{\rm 160a}$,
H.~Stenzel$^{\rm 52}$,
S.~Stern$^{\rm 101}$,
G.A.~Stewart$^{\rm 53}$,
J.A.~Stillings$^{\rm 21}$,
M.C.~Stockton$^{\rm 87}$,
M.~Stoebe$^{\rm 87}$,
G.~Stoicea$^{\rm 26a}$,
P.~Stolte$^{\rm 54}$,
S.~Stonjek$^{\rm 101}$,
A.R.~Stradling$^{\rm 8}$,
A.~Straessner$^{\rm 44}$,
M.E.~Stramaglia$^{\rm 17}$,
J.~Strandberg$^{\rm 148}$,
S.~Strandberg$^{\rm 147a,147b}$,
A.~Strandlie$^{\rm 119}$,
E.~Strauss$^{\rm 144}$,
M.~Strauss$^{\rm 113}$,
P.~Strizenec$^{\rm 145b}$,
R.~Str\"ohmer$^{\rm 175}$,
D.M.~Strom$^{\rm 116}$,
R.~Stroynowski$^{\rm 40}$,
A.~Strubig$^{\rm 106}$,
S.A.~Stucci$^{\rm 17}$,
B.~Stugu$^{\rm 14}$,
N.A.~Styles$^{\rm 42}$,
D.~Su$^{\rm 144}$,
J.~Su$^{\rm 125}$,
R.~Subramaniam$^{\rm 79}$,
A.~Succurro$^{\rm 12}$,
Y.~Sugaya$^{\rm 118}$,
C.~Suhr$^{\rm 108}$,
M.~Suk$^{\rm 128}$,
V.V.~Sulin$^{\rm 96}$,
S.~Sultansoy$^{\rm 4d}$,
T.~Sumida$^{\rm 68}$,
S.~Sun$^{\rm 57}$,
X.~Sun$^{\rm 33a}$,
J.E.~Sundermann$^{\rm 48}$,
K.~Suruliz$^{\rm 150}$,
G.~Susinno$^{\rm 37a,37b}$,
M.R.~Sutton$^{\rm 150}$,
Y.~Suzuki$^{\rm 66}$,
M.~Svatos$^{\rm 127}$,
S.~Swedish$^{\rm 169}$,
M.~Swiatlowski$^{\rm 144}$,
I.~Sykora$^{\rm 145a}$,
T.~Sykora$^{\rm 129}$,
D.~Ta$^{\rm 90}$,
C.~Taccini$^{\rm 135a,135b}$,
K.~Tackmann$^{\rm 42}$,
J.~Taenzer$^{\rm 159}$,
A.~Taffard$^{\rm 164}$,
R.~Tafirout$^{\rm 160a}$,
N.~Taiblum$^{\rm 154}$,
H.~Takai$^{\rm 25}$,
R.~Takashima$^{\rm 69}$,
H.~Takeda$^{\rm 67}$,
T.~Takeshita$^{\rm 141}$,
Y.~Takubo$^{\rm 66}$,
M.~Talby$^{\rm 85}$,
A.A.~Talyshev$^{\rm 109}$$^{,c}$,
J.Y.C.~Tam$^{\rm 175}$,
K.G.~Tan$^{\rm 88}$,
J.~Tanaka$^{\rm 156}$,
R.~Tanaka$^{\rm 117}$,
S.~Tanaka$^{\rm 132}$,
S.~Tanaka$^{\rm 66}$,
A.J.~Tanasijczuk$^{\rm 143}$,
B.B.~Tannenwald$^{\rm 111}$,
N.~Tannoury$^{\rm 21}$,
S.~Tapprogge$^{\rm 83}$,
S.~Tarem$^{\rm 153}$,
F.~Tarrade$^{\rm 29}$,
G.F.~Tartarelli$^{\rm 91a}$,
P.~Tas$^{\rm 129}$,
M.~Tasevsky$^{\rm 127}$,
T.~Tashiro$^{\rm 68}$,
E.~Tassi$^{\rm 37a,37b}$,
A.~Tavares~Delgado$^{\rm 126a,126b}$,
Y.~Tayalati$^{\rm 136d}$,
F.E.~Taylor$^{\rm 94}$,
G.N.~Taylor$^{\rm 88}$,
W.~Taylor$^{\rm 160b}$,
F.A.~Teischinger$^{\rm 30}$,
M.~Teixeira~Dias~Castanheira$^{\rm 76}$,
P.~Teixeira-Dias$^{\rm 77}$,
K.K.~Temming$^{\rm 48}$,
H.~Ten~Kate$^{\rm 30}$,
P.K.~Teng$^{\rm 152}$,
J.J.~Teoh$^{\rm 118}$,
S.~Terada$^{\rm 66}$,
K.~Terashi$^{\rm 156}$,
J.~Terron$^{\rm 82}$,
S.~Terzo$^{\rm 101}$,
M.~Testa$^{\rm 47}$,
R.J.~Teuscher$^{\rm 159}$$^{,k}$,
J.~Therhaag$^{\rm 21}$,
T.~Theveneaux-Pelzer$^{\rm 34}$,
J.P.~Thomas$^{\rm 18}$,
J.~Thomas-Wilsker$^{\rm 77}$,
E.N.~Thompson$^{\rm 35}$,
P.D.~Thompson$^{\rm 18}$,
R.J.~Thompson$^{\rm 84}$,
A.S.~Thompson$^{\rm 53}$,
L.A.~Thomsen$^{\rm 36}$,
E.~Thomson$^{\rm 122}$,
M.~Thomson$^{\rm 28}$,
W.M.~Thong$^{\rm 88}$,
R.P.~Thun$^{\rm 89}$$^{,*}$,
F.~Tian$^{\rm 35}$,
M.J.~Tibbetts$^{\rm 15}$,
V.O.~Tikhomirov$^{\rm 96}$$^{,af}$,
Yu.A.~Tikhonov$^{\rm 109}$$^{,c}$,
S.~Timoshenko$^{\rm 98}$,
E.~Tiouchichine$^{\rm 85}$,
P.~Tipton$^{\rm 177}$,
S.~Tisserant$^{\rm 85}$,
T.~Todorov$^{\rm 5}$,
S.~Todorova-Nova$^{\rm 129}$,
J.~Tojo$^{\rm 70}$,
S.~Tok\'ar$^{\rm 145a}$,
K.~Tokushuku$^{\rm 66}$,
K.~Tollefson$^{\rm 90}$,
E.~Tolley$^{\rm 57}$,
L.~Tomlinson$^{\rm 84}$,
M.~Tomoto$^{\rm 103}$,
L.~Tompkins$^{\rm 31}$,
K.~Toms$^{\rm 105}$,
N.D.~Topilin$^{\rm 65}$,
E.~Torrence$^{\rm 116}$,
H.~Torres$^{\rm 143}$,
E.~Torr\'o~Pastor$^{\rm 168}$,
J.~Toth$^{\rm 85}$$^{,ag}$,
F.~Touchard$^{\rm 85}$,
D.R.~Tovey$^{\rm 140}$,
H.L.~Tran$^{\rm 117}$,
T.~Trefzger$^{\rm 175}$,
L.~Tremblet$^{\rm 30}$,
A.~Tricoli$^{\rm 30}$,
I.M.~Trigger$^{\rm 160a}$,
S.~Trincaz-Duvoid$^{\rm 80}$,
M.F.~Tripiana$^{\rm 12}$,
W.~Trischuk$^{\rm 159}$,
B.~Trocm\'e$^{\rm 55}$,
C.~Troncon$^{\rm 91a}$,
M.~Trottier-McDonald$^{\rm 15}$,
M.~Trovatelli$^{\rm 135a,135b}$,
P.~True$^{\rm 90}$,
M.~Trzebinski$^{\rm 39}$,
A.~Trzupek$^{\rm 39}$,
C.~Tsarouchas$^{\rm 30}$,
J.C-L.~Tseng$^{\rm 120}$,
P.V.~Tsiareshka$^{\rm 92}$,
D.~Tsionou$^{\rm 137}$,
G.~Tsipolitis$^{\rm 10}$,
N.~Tsirintanis$^{\rm 9}$,
S.~Tsiskaridze$^{\rm 12}$,
V.~Tsiskaridze$^{\rm 48}$,
E.G.~Tskhadadze$^{\rm 51a}$,
I.I.~Tsukerman$^{\rm 97}$,
V.~Tsulaia$^{\rm 15}$,
S.~Tsuno$^{\rm 66}$,
D.~Tsybychev$^{\rm 149}$,
A.~Tudorache$^{\rm 26a}$,
V.~Tudorache$^{\rm 26a}$,
A.N.~Tuna$^{\rm 122}$,
S.A.~Tupputi$^{\rm 20a,20b}$,
S.~Turchikhin$^{\rm 99}$$^{,ae}$,
D.~Turecek$^{\rm 128}$,
I.~Turk~Cakir$^{\rm 4c}$,
R.~Turra$^{\rm 91a,91b}$,
A.J.~Turvey$^{\rm 40}$,
P.M.~Tuts$^{\rm 35}$,
A.~Tykhonov$^{\rm 49}$,
M.~Tylmad$^{\rm 147a,147b}$,
M.~Tyndel$^{\rm 131}$,
K.~Uchida$^{\rm 21}$,
I.~Ueda$^{\rm 156}$,
R.~Ueno$^{\rm 29}$,
M.~Ughetto$^{\rm 85}$,
M.~Ugland$^{\rm 14}$,
M.~Uhlenbrock$^{\rm 21}$,
F.~Ukegawa$^{\rm 161}$,
G.~Unal$^{\rm 30}$,
A.~Undrus$^{\rm 25}$,
G.~Unel$^{\rm 164}$,
F.C.~Ungaro$^{\rm 48}$,
Y.~Unno$^{\rm 66}$,
C.~Unverdorben$^{\rm 100}$,
J.~Urban$^{\rm 145b}$,
D.~Urbaniec$^{\rm 35}$,
P.~Urquijo$^{\rm 88}$,
G.~Usai$^{\rm 8}$,
A.~Usanova$^{\rm 62}$,
L.~Vacavant$^{\rm 85}$,
V.~Vacek$^{\rm 128}$,
B.~Vachon$^{\rm 87}$,
N.~Valencic$^{\rm 107}$,
S.~Valentinetti$^{\rm 20a,20b}$,
A.~Valero$^{\rm 168}$,
L.~Valery$^{\rm 34}$,
S.~Valkar$^{\rm 129}$,
E.~Valladolid~Gallego$^{\rm 168}$,
S.~Vallecorsa$^{\rm 49}$,
J.A.~Valls~Ferrer$^{\rm 168}$,
W.~Van~Den~Wollenberg$^{\rm 107}$,
P.C.~Van~Der~Deijl$^{\rm 107}$,
R.~van~der~Geer$^{\rm 107}$,
H.~van~der~Graaf$^{\rm 107}$,
R.~Van~Der~Leeuw$^{\rm 107}$,
D.~van~der~Ster$^{\rm 30}$,
N.~van~Eldik$^{\rm 30}$,
P.~van~Gemmeren$^{\rm 6}$,
J.~Van~Nieuwkoop$^{\rm 143}$,
I.~van~Vulpen$^{\rm 107}$,
M.C.~van~Woerden$^{\rm 30}$,
M.~Vanadia$^{\rm 133a,133b}$,
W.~Vandelli$^{\rm 30}$,
R.~Vanguri$^{\rm 122}$,
A.~Vaniachine$^{\rm 6}$,
P.~Vankov$^{\rm 42}$,
F.~Vannucci$^{\rm 80}$,
G.~Vardanyan$^{\rm 178}$,
R.~Vari$^{\rm 133a}$,
E.W.~Varnes$^{\rm 7}$,
T.~Varol$^{\rm 86}$,
D.~Varouchas$^{\rm 80}$,
A.~Vartapetian$^{\rm 8}$,
K.E.~Varvell$^{\rm 151}$,
F.~Vazeille$^{\rm 34}$,
T.~Vazquez~Schroeder$^{\rm 54}$,
J.~Veatch$^{\rm 7}$,
F.~Veloso$^{\rm 126a,126c}$,
T.~Velz$^{\rm 21}$,
S.~Veneziano$^{\rm 133a}$,
A.~Ventura$^{\rm 73a,73b}$,
D.~Ventura$^{\rm 86}$,
M.~Venturi$^{\rm 170}$,
N.~Venturi$^{\rm 159}$,
A.~Venturini$^{\rm 23}$,
V.~Vercesi$^{\rm 121a}$,
M.~Verducci$^{\rm 133a,133b}$,
W.~Verkerke$^{\rm 107}$,
J.C.~Vermeulen$^{\rm 107}$,
A.~Vest$^{\rm 44}$,
M.C.~Vetterli$^{\rm 143}$$^{,e}$,
O.~Viazlo$^{\rm 81}$,
I.~Vichou$^{\rm 166}$,
T.~Vickey$^{\rm 146c}$$^{,ah}$,
O.E.~Vickey~Boeriu$^{\rm 146c}$,
G.H.A.~Viehhauser$^{\rm 120}$,
S.~Viel$^{\rm 169}$,
R.~Vigne$^{\rm 30}$,
M.~Villa$^{\rm 20a,20b}$,
M.~Villaplana~Perez$^{\rm 91a,91b}$,
E.~Vilucchi$^{\rm 47}$,
M.G.~Vincter$^{\rm 29}$,
V.B.~Vinogradov$^{\rm 65}$,
J.~Virzi$^{\rm 15}$,
I.~Vivarelli$^{\rm 150}$,
F.~Vives~Vaque$^{\rm 3}$,
S.~Vlachos$^{\rm 10}$,
D.~Vladoiu$^{\rm 100}$,
M.~Vlasak$^{\rm 128}$,
A.~Vogel$^{\rm 21}$,
M.~Vogel$^{\rm 32a}$,
P.~Vokac$^{\rm 128}$,
G.~Volpi$^{\rm 124a,124b}$,
M.~Volpi$^{\rm 88}$,
H.~von~der~Schmitt$^{\rm 101}$,
H.~von~Radziewski$^{\rm 48}$,
E.~von~Toerne$^{\rm 21}$,
V.~Vorobel$^{\rm 129}$,
K.~Vorobev$^{\rm 98}$,
M.~Vos$^{\rm 168}$,
R.~Voss$^{\rm 30}$,
J.H.~Vossebeld$^{\rm 74}$,
N.~Vranjes$^{\rm 137}$,
M.~Vranjes~Milosavljevic$^{\rm 13a}$,
V.~Vrba$^{\rm 127}$,
M.~Vreeswijk$^{\rm 107}$,
T.~Vu~Anh$^{\rm 48}$,
R.~Vuillermet$^{\rm 30}$,
I.~Vukotic$^{\rm 31}$,
Z.~Vykydal$^{\rm 128}$,
P.~Wagner$^{\rm 21}$,
W.~Wagner$^{\rm 176}$,
H.~Wahlberg$^{\rm 71}$,
S.~Wahrmund$^{\rm 44}$,
J.~Wakabayashi$^{\rm 103}$,
J.~Walder$^{\rm 72}$,
R.~Walker$^{\rm 100}$,
W.~Walkowiak$^{\rm 142}$,
R.~Wall$^{\rm 177}$,
P.~Waller$^{\rm 74}$,
B.~Walsh$^{\rm 177}$,
C.~Wang$^{\rm 33c}$,
C.~Wang$^{\rm 45}$,
F.~Wang$^{\rm 174}$,
H.~Wang$^{\rm 15}$,
H.~Wang$^{\rm 40}$,
J.~Wang$^{\rm 42}$,
J.~Wang$^{\rm 33a}$,
K.~Wang$^{\rm 87}$,
R.~Wang$^{\rm 105}$,
S.M.~Wang$^{\rm 152}$,
T.~Wang$^{\rm 21}$,
X.~Wang$^{\rm 177}$,
C.~Wanotayaroj$^{\rm 116}$,
A.~Warburton$^{\rm 87}$,
C.P.~Ward$^{\rm 28}$,
D.R.~Wardrope$^{\rm 78}$,
M.~Warsinsky$^{\rm 48}$,
A.~Washbrook$^{\rm 46}$,
C.~Wasicki$^{\rm 42}$,
P.M.~Watkins$^{\rm 18}$,
A.T.~Watson$^{\rm 18}$,
I.J.~Watson$^{\rm 151}$,
M.F.~Watson$^{\rm 18}$,
G.~Watts$^{\rm 139}$,
S.~Watts$^{\rm 84}$,
B.M.~Waugh$^{\rm 78}$,
S.~Webb$^{\rm 84}$,
M.S.~Weber$^{\rm 17}$,
S.W.~Weber$^{\rm 175}$,
J.S.~Webster$^{\rm 31}$,
A.R.~Weidberg$^{\rm 120}$,
B.~Weinert$^{\rm 61}$,
J.~Weingarten$^{\rm 54}$,
C.~Weiser$^{\rm 48}$,
H.~Weits$^{\rm 107}$,
P.S.~Wells$^{\rm 30}$,
T.~Wenaus$^{\rm 25}$,
D.~Wendland$^{\rm 16}$,
Z.~Weng$^{\rm 152}$$^{,ad}$,
T.~Wengler$^{\rm 30}$,
S.~Wenig$^{\rm 30}$,
N.~Wermes$^{\rm 21}$,
M.~Werner$^{\rm 48}$,
P.~Werner$^{\rm 30}$,
M.~Wessels$^{\rm 58a}$,
J.~Wetter$^{\rm 162}$,
K.~Whalen$^{\rm 29}$,
A.~White$^{\rm 8}$,
M.J.~White$^{\rm 1}$,
R.~White$^{\rm 32b}$,
S.~White$^{\rm 124a,124b}$,
D.~Whiteson$^{\rm 164}$,
D.~Wicke$^{\rm 176}$,
F.J.~Wickens$^{\rm 131}$,
W.~Wiedenmann$^{\rm 174}$,
M.~Wielers$^{\rm 131}$,
P.~Wienemann$^{\rm 21}$,
C.~Wiglesworth$^{\rm 36}$,
L.A.M.~Wiik-Fuchs$^{\rm 21}$,
P.A.~Wijeratne$^{\rm 78}$,
A.~Wildauer$^{\rm 101}$,
M.A.~Wildt$^{\rm 42}$$^{,ai}$,
H.G.~Wilkens$^{\rm 30}$,
H.H.~Williams$^{\rm 122}$,
S.~Williams$^{\rm 28}$,
C.~Willis$^{\rm 90}$,
S.~Willocq$^{\rm 86}$,
A.~Wilson$^{\rm 89}$,
J.A.~Wilson$^{\rm 18}$,
I.~Wingerter-Seez$^{\rm 5}$,
F.~Winklmeier$^{\rm 116}$,
B.T.~Winter$^{\rm 21}$,
M.~Wittgen$^{\rm 144}$,
T.~Wittig$^{\rm 43}$,
J.~Wittkowski$^{\rm 100}$,
S.J.~Wollstadt$^{\rm 83}$,
M.W.~Wolter$^{\rm 39}$,
H.~Wolters$^{\rm 126a,126c}$,
B.K.~Wosiek$^{\rm 39}$,
J.~Wotschack$^{\rm 30}$,
M.J.~Woudstra$^{\rm 84}$,
K.W.~Wozniak$^{\rm 39}$,
M.~Wright$^{\rm 53}$,
M.~Wu$^{\rm 55}$,
S.L.~Wu$^{\rm 174}$,
X.~Wu$^{\rm 49}$,
Y.~Wu$^{\rm 89}$,
E.~Wulf$^{\rm 35}$,
T.R.~Wyatt$^{\rm 84}$,
B.M.~Wynne$^{\rm 46}$,
S.~Xella$^{\rm 36}$,
M.~Xiao$^{\rm 137}$,
D.~Xu$^{\rm 33a}$,
L.~Xu$^{\rm 33b}$$^{,aj}$,
B.~Yabsley$^{\rm 151}$,
S.~Yacoob$^{\rm 146b}$$^{,ak}$,
R.~Yakabe$^{\rm 67}$,
M.~Yamada$^{\rm 66}$,
H.~Yamaguchi$^{\rm 156}$,
Y.~Yamaguchi$^{\rm 118}$,
A.~Yamamoto$^{\rm 66}$,
S.~Yamamoto$^{\rm 156}$,
T.~Yamamura$^{\rm 156}$,
T.~Yamanaka$^{\rm 156}$,
K.~Yamauchi$^{\rm 103}$,
Y.~Yamazaki$^{\rm 67}$,
Z.~Yan$^{\rm 22}$,
H.~Yang$^{\rm 33e}$,
H.~Yang$^{\rm 174}$,
Y.~Yang$^{\rm 111}$,
S.~Yanush$^{\rm 93}$,
L.~Yao$^{\rm 33a}$,
W-M.~Yao$^{\rm 15}$,
Y.~Yasu$^{\rm 66}$,
E.~Yatsenko$^{\rm 42}$,
K.H.~Yau~Wong$^{\rm 21}$,
J.~Ye$^{\rm 40}$,
S.~Ye$^{\rm 25}$,
I.~Yeletskikh$^{\rm 65}$,
A.L.~Yen$^{\rm 57}$,
E.~Yildirim$^{\rm 42}$,
M.~Yilmaz$^{\rm 4b}$,
R.~Yoosoofmiya$^{\rm 125}$,
K.~Yorita$^{\rm 172}$,
R.~Yoshida$^{\rm 6}$,
K.~Yoshihara$^{\rm 156}$,
C.~Young$^{\rm 144}$,
C.J.S.~Young$^{\rm 30}$,
S.~Youssef$^{\rm 22}$,
D.R.~Yu$^{\rm 15}$,
J.~Yu$^{\rm 8}$,
J.M.~Yu$^{\rm 89}$,
J.~Yu$^{\rm 114}$,
L.~Yuan$^{\rm 67}$,
A.~Yurkewicz$^{\rm 108}$,
I.~Yusuff$^{\rm 28}$$^{,al}$,
B.~Zabinski$^{\rm 39}$,
R.~Zaidan$^{\rm 63}$,
A.M.~Zaitsev$^{\rm 130}$$^{,z}$,
A.~Zaman$^{\rm 149}$,
S.~Zambito$^{\rm 23}$,
L.~Zanello$^{\rm 133a,133b}$,
D.~Zanzi$^{\rm 88}$,
C.~Zeitnitz$^{\rm 176}$,
M.~Zeman$^{\rm 128}$,
A.~Zemla$^{\rm 38a}$,
K.~Zengel$^{\rm 23}$,
O.~Zenin$^{\rm 130}$,
T.~\v{Z}eni\v{s}$^{\rm 145a}$,
D.~Zerwas$^{\rm 117}$,
G.~Zevi~della~Porta$^{\rm 57}$,
D.~Zhang$^{\rm 89}$,
F.~Zhang$^{\rm 174}$,
H.~Zhang$^{\rm 90}$,
J.~Zhang$^{\rm 6}$,
L.~Zhang$^{\rm 152}$,
R.~Zhang$^{\rm 33b}$,
X.~Zhang$^{\rm 33d}$,
Z.~Zhang$^{\rm 117}$,
Y.~Zhao$^{\rm 33d}$,
Z.~Zhao$^{\rm 33b}$,
A.~Zhemchugov$^{\rm 65}$,
J.~Zhong$^{\rm 120}$,
B.~Zhou$^{\rm 89}$,
L.~Zhou$^{\rm 35}$,
L.~Zhou$^{\rm 40}$,
N.~Zhou$^{\rm 164}$,
C.G.~Zhu$^{\rm 33d}$,
H.~Zhu$^{\rm 33a}$,
J.~Zhu$^{\rm 89}$,
Y.~Zhu$^{\rm 33b}$,
X.~Zhuang$^{\rm 33a}$,
K.~Zhukov$^{\rm 96}$,
A.~Zibell$^{\rm 175}$,
D.~Zieminska$^{\rm 61}$,
N.I.~Zimine$^{\rm 65}$,
C.~Zimmermann$^{\rm 83}$,
R.~Zimmermann$^{\rm 21}$,
S.~Zimmermann$^{\rm 21}$,
S.~Zimmermann$^{\rm 48}$,
Z.~Zinonos$^{\rm 54}$,
M.~Ziolkowski$^{\rm 142}$,
G.~Zobernig$^{\rm 174}$,
A.~Zoccoli$^{\rm 20a,20b}$,
M.~zur~Nedden$^{\rm 16}$,
G.~Zurzolo$^{\rm 104a,104b}$,
L.~Zwalinski$^{\rm 30}$.
\bigskip
\\
$^{1}$ Department of Physics, University of Adelaide, Adelaide, Australia\\
$^{2}$ Physics Department, SUNY Albany, Albany NY, United States of America\\
$^{3}$ Department of Physics, University of Alberta, Edmonton AB, Canada\\
$^{4}$ $^{(a)}$ Department of Physics, Ankara University, Ankara; $^{(b)}$ Department of Physics, Gazi University, Ankara; $^{(c)}$ Istanbul Aydin University, Istanbul; $^{(d)}$ Division of Physics, TOBB University of Economics and Technology, Ankara, Turkey\\
$^{5}$ LAPP, CNRS/IN2P3 and Universit{\'e} de Savoie, Annecy-le-Vieux, France\\
$^{6}$ High Energy Physics Division, Argonne National Laboratory, Argonne IL, United States of America\\
$^{7}$ Department of Physics, University of Arizona, Tucson AZ, United States of America\\
$^{8}$ Department of Physics, The University of Texas at Arlington, Arlington TX, United States of America\\
$^{9}$ Physics Department, University of Athens, Athens, Greece\\
$^{10}$ Physics Department, National Technical University of Athens, Zografou, Greece\\
$^{11}$ Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{12}$ Institut de F{\'\i}sica d'Altes Energies and Departament de F{\'\i}sica de la Universitat Aut{\`o}noma de Barcelona, Barcelona, Spain\\
$^{13}$ $^{(a)}$ Institute of Physics, University of Belgrade, Belgrade; $^{(b)}$ Vinca Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia\\
$^{14}$ Department for Physics and Technology, University of Bergen, Bergen, Norway\\
$^{15}$ Physics Division, Lawrence Berkeley National Laboratory and University of California, Berkeley CA, United States of America\\
$^{16}$ Department of Physics, Humboldt University, Berlin, Germany\\
$^{17}$ Albert Einstein Center for Fundamental Physics and Laboratory for High Energy Physics, University of Bern, Bern, Switzerland\\
$^{18}$ School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{19}$ $^{(a)}$ Department of Physics, Bogazici University, Istanbul; $^{(b)}$ Department of Physics, Dogus University, Istanbul; $^{(c)}$ Department of Physics Engineering, Gaziantep University, Gaziantep, Turkey\\
$^{20}$ $^{(a)}$ INFN Sezione di Bologna; $^{(b)}$ Dipartimento di Fisica e Astronomia, Universit{\`a} di Bologna, Bologna, Italy\\
$^{21}$ Physikalisches Institut, University of Bonn, Bonn, Germany\\
$^{22}$ Department of Physics, Boston University, Boston MA, United States of America\\
$^{23}$ Department of Physics, Brandeis University, Waltham MA, United States of America\\
$^{24}$ $^{(a)}$ Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro; $^{(b)}$ Electrical Circuits Department, Federal University of Juiz de Fora (UFJF), Juiz de Fora; $^{(c)}$ Federal University of Sao Joao del Rei (UFSJ), Sao Joao del Rei; $^{(d)}$ Instituto de Fisica, Universidade de Sao Paulo, Sao Paulo, Brazil\\
$^{25}$ Physics Department, Brookhaven National Laboratory, Upton NY, United States of America\\
$^{26}$ $^{(a)}$ National Institute of Physics and Nuclear Engineering, Bucharest; $^{(b)}$ National Institute for Research and Development of Isotopic and Molecular Technologies, Physics Department, Cluj Napoca; $^{(c)}$ University Politehnica Bucharest, Bucharest; $^{(d)}$ West University in Timisoara, Timisoara, Romania\\
$^{27}$ Departamento de F{\'\i}sica, Universidad de Buenos Aires, Buenos Aires, Argentina\\
$^{28}$ Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{29}$ Department of Physics, Carleton University, Ottawa ON, Canada\\
$^{30}$ CERN, Geneva, Switzerland\\
$^{31}$ Enrico Fermi Institute, University of Chicago, Chicago IL, United States of America\\
$^{32}$ $^{(a)}$ Departamento de F{\'\i}sica, Pontificia Universidad Cat{\'o}lica de Chile, Santiago; $^{(b)}$ Departamento de F{\'\i}sica, Universidad T{\'e}cnica Federico Santa Mar{\'\i}a, Valpara{\'\i}so, Chile\\
$^{33}$ $^{(a)}$ Institute of High Energy Physics, Chinese Academy of Sciences, Beijing; $^{(b)}$ Department of Modern Physics, University of Science and Technology of China, Anhui; $^{(c)}$ Department of Physics, Nanjing University, Jiangsu; $^{(d)}$ School of Physics, Shandong University, Shandong; $^{(e)}$ Physics Department, Shanghai Jiao Tong University, Shanghai; $^{(f)}$ Physics Department, Tsinghua University, Beijing 100084, China\\
$^{34}$ Laboratoire de Physique Corpusculaire, Clermont Universit{\'e} and Universit{\'e} Blaise Pascal and CNRS/IN2P3, Clermont-Ferrand, France\\
$^{35}$ Nevis Laboratory, Columbia University, Irvington NY, United States of America\\
$^{36}$ Niels Bohr Institute, University of Copenhagen, Kobenhavn, Denmark\\
$^{37}$ $^{(a)}$ INFN Gruppo Collegato di Cosenza, Laboratori Nazionali di Frascati; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} della Calabria, Rende, Italy\\
$^{38}$ $^{(a)}$ AGH University of Science and Technology, Faculty of Physics and Applied Computer Science, Krakow; $^{(b)}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Krakow, Poland\\
$^{39}$ The Henryk Niewodniczanski Institute of Nuclear Physics, Polish Academy of Sciences, Krakow, Poland\\
$^{40}$ Physics Department, Southern Methodist University, Dallas TX, United States of America\\
$^{41}$ Physics Department, University of Texas at Dallas, Richardson TX, United States of America\\
$^{42}$ DESY, Hamburg and Zeuthen, Germany\\
$^{43}$ Institut f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{44}$ Institut f{\"u}r Kern-{~}und Teilchenphysik, Technische Universit{\"a}t Dresden, Dresden, Germany\\
$^{45}$ Department of Physics, Duke University, Durham NC, United States of America\\
$^{46}$ SUPA - School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{47}$ INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{48}$ Fakult{\"a}t f{\"u}r Mathematik und Physik, Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany\\
$^{49}$ Section de Physique, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{50}$ $^{(a)}$ INFN Sezione di Genova; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Genova, Genova, Italy\\
$^{51}$ $^{(a)}$ E. Andronikashvili Institute of Physics, Iv. Javakhishvili Tbilisi State University, Tbilisi; $^{(b)}$ High Energy Physics Institute, Tbilisi State University, Tbilisi, Georgia\\
$^{52}$ II Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen, Germany\\
$^{53}$ SUPA - School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{54}$ II Physikalisches Institut, Georg-August-Universit{\"a}t, G{\"o}ttingen, Germany\\
$^{55}$ Laboratoire de Physique Subatomique et de Cosmologie, Universit{\'e}  Grenoble-Alpes, CNRS/IN2P3, Grenoble, France\\
$^{56}$ Department of Physics, Hampton University, Hampton VA, United States of America\\
$^{57}$ Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge MA, United States of America\\
$^{58}$ $^{(a)}$ Kirchhoff-Institut f{\"u}r Physik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(b)}$ Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(c)}$ ZITI Institut f{\"u}r technische Informatik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Mannheim, Germany\\
$^{59}$ Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima, Japan\\
$^{60}$ $^{(a)}$ Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong; $^{(b)}$ Department of Physics, The University of Hong Kong, Hong Kong; $^{(c)}$ Department of Physics, The Hong Kong University of Science and Technology, Clear Water Bay, Kowloon, Hong Kong, China\\
$^{61}$ Department of Physics, Indiana University, Bloomington IN, United States of America\\
$^{62}$ Institut f{\"u}r Astro-{~}und Teilchenphysik, Leopold-Franzens-Universit{\"a}t, Innsbruck, Austria\\
$^{63}$ University of Iowa, Iowa City IA, United States of America\\
$^{64}$ Department of Physics and Astronomy, Iowa State University, Ames IA, United States of America\\
$^{65}$ Joint Institute for Nuclear Research, JINR Dubna, Dubna, Russia\\
$^{66}$ KEK, High Energy Accelerator Research Organization, Tsukuba, Japan\\
$^{67}$ Graduate School of Science, Kobe University, Kobe, Japan\\
$^{68}$ Faculty of Science, Kyoto University, Kyoto, Japan\\
$^{69}$ Kyoto University of Education, Kyoto, Japan\\
$^{70}$ Department of Physics, Kyushu University, Fukuoka, Japan\\
$^{71}$ Instituto de F{\'\i}sica La Plata, Universidad Nacional de La Plata and CONICET, La Plata, Argentina\\
$^{72}$ Physics Department, Lancaster University, Lancaster, United Kingdom\\
$^{73}$ $^{(a)}$ INFN Sezione di Lecce; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} del Salento, Lecce, Italy\\
$^{74}$ Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{75}$ Department of Physics, Jo{\v{z}}ef Stefan Institute and University of Ljubljana, Ljubljana, Slovenia\\
$^{76}$ School of Physics and Astronomy, Queen Mary University of London, London, United Kingdom\\
$^{77}$ Department of Physics, Royal Holloway University of London, Surrey, United Kingdom\\
$^{78}$ Department of Physics and Astronomy, University College London, London, United Kingdom\\
$^{79}$ Louisiana Tech University, Ruston LA, United States of America\\
$^{80}$ Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies, UPMC and Universit{\'e} Paris-Diderot and CNRS/IN2P3, Paris, France\\
$^{81}$ Fysiska institutionen, Lunds universitet, Lund, Sweden\\
$^{82}$ Departamento de Fisica Teorica C-15, Universidad Autonoma de Madrid, Madrid, Spain\\
$^{83}$ Institut f{\"u}r Physik, Universit{\"a}t Mainz, Mainz, Germany\\
$^{84}$ School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{85}$ CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{86}$ Department of Physics, University of Massachusetts, Amherst MA, United States of America\\
$^{87}$ Department of Physics, McGill University, Montreal QC, Canada\\
$^{88}$ School of Physics, University of Melbourne, Victoria, Australia\\
$^{89}$ Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{90}$ Department of Physics and Astronomy, Michigan State University, East Lansing MI, United States of America\\
$^{91}$ $^{(a)}$ INFN Sezione di Milano; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Milano, Milano, Italy\\
$^{92}$ B.I. Stepanov Institute of Physics, National Academy of Sciences of Belarus, Minsk, Republic of Belarus\\
$^{93}$ National Scientific and Educational Centre for Particle and High Energy Physics, Minsk, Republic of Belarus\\
$^{94}$ Department of Physics, Massachusetts Institute of Technology, Cambridge MA, United States of America\\
$^{95}$ Group of Particle Physics, University of Montreal, Montreal QC, Canada\\
$^{96}$ P.N. Lebedev Institute of Physics, Academy of Sciences, Moscow, Russia\\
$^{97}$ Institute for Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$^{98}$ National Research Nuclear University MEPhI, Moscow, Russia\\
$^{99}$ D.V.Skobeltsyn Institute of Nuclear Physics, M.V.Lomonosov Moscow State University, Moscow, Russia\\
$^{100}$ Fakult{\"a}t f{\"u}r Physik, Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen, M{\"u}nchen, Germany\\
$^{101}$ Max-Planck-Institut f{\"u}r Physik (Werner-Heisenberg-Institut), M{\"u}nchen, Germany\\
$^{102}$ Nagasaki Institute of Applied Science, Nagasaki, Japan\\
$^{103}$ Graduate School of Science and Kobayashi-Maskawa Institute, Nagoya University, Nagoya, Japan\\
$^{104}$ $^{(a)}$ INFN Sezione di Napoli; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Napoli, Napoli, Italy\\
$^{105}$ Department of Physics and Astronomy, University of New Mexico, Albuquerque NM, United States of America\\
$^{106}$ Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen, Netherlands\\
$^{107}$ Nikhef National Institute for Subatomic Physics and University of Amsterdam, Amsterdam, Netherlands\\
$^{108}$ Department of Physics, Northern Illinois University, DeKalb IL, United States of America\\
$^{109}$ Budker Institute of Nuclear Physics, SB RAS, Novosibirsk, Russia\\
$^{110}$ Department of Physics, New York University, New York NY, United States of America\\
$^{111}$ Ohio State University, Columbus OH, United States of America\\
$^{112}$ Faculty of Science, Okayama University, Okayama, Japan\\
$^{113}$ Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK, United States of America\\
$^{114}$ Department of Physics, Oklahoma State University, Stillwater OK, United States of America\\
$^{115}$ Palack{\'y} University, RCPTM, Olomouc, Czech Republic\\
$^{116}$ Center for High Energy Physics, University of Oregon, Eugene OR, United States of America\\
$^{117}$ LAL, Universit{\'e} Paris-Sud and CNRS/IN2P3, Orsay, France\\
$^{118}$ Graduate School of Science, Osaka University, Osaka, Japan\\
$^{119}$ Department of Physics, University of Oslo, Oslo, Norway\\
$^{120}$ Department of Physics, Oxford University, Oxford, United Kingdom\\
$^{121}$ $^{(a)}$ INFN Sezione di Pavia; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Pavia, Pavia, Italy\\
$^{122}$ Department of Physics, University of Pennsylvania, Philadelphia PA, United States of America\\
$^{123}$ Petersburg Nuclear Physics Institute, Gatchina, Russia\\
$^{124}$ $^{(a)}$ INFN Sezione di Pisa; $^{(b)}$ Dipartimento di Fisica E. Fermi, Universit{\`a} di Pisa, Pisa, Italy\\
$^{125}$ Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA, United States of America\\
$^{126}$ $^{(a)}$ Laboratorio de Instrumentacao e Fisica Experimental de Particulas - LIP, Lisboa; $^{(b)}$ Faculdade de Ci{\^e}ncias, Universidade de Lisboa, Lisboa; $^{(c)}$ Department of Physics, University of Coimbra, Coimbra; $^{(d)}$ Centro de F{\'\i}sica Nuclear da Universidade de Lisboa, Lisboa; $^{(e)}$ Departamento de Fisica, Universidade do Minho, Braga; $^{(f)}$ Departamento de Fisica Teorica y del Cosmos and CAFPE, Universidad de Granada, Granada (Spain); $^{(g)}$ Dep Fisica and CEFITEC of Faculdade de Ciencias e Tecnologia, Universidade Nova de Lisboa, Caparica, Portugal\\
$^{127}$ Institute of Physics, Academy of Sciences of the Czech Republic, Praha, Czech Republic\\
$^{128}$ Czech Technical University in Prague, Praha, Czech Republic\\
$^{129}$ Faculty of Mathematics and Physics, Charles University in Prague, Praha, Czech Republic\\
$^{130}$ State Research Center Institute for High Energy Physics, Protvino, Russia\\
$^{131}$ Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{132}$ Ritsumeikan University, Kusatsu, Shiga, Japan\\
$^{133}$ $^{(a)}$ INFN Sezione di Roma; $^{(b)}$ Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, Roma, Italy\\
$^{134}$ $^{(a)}$ INFN Sezione di Roma Tor Vergata; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{135}$ $^{(a)}$ INFN Sezione di Roma Tre; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} Roma Tre, Roma, Italy\\
$^{136}$ $^{(a)}$ Facult{\'e} des Sciences Ain Chock, R{\'e}seau Universitaire de Physique des Hautes Energies - Universit{\'e} Hassan II, Casablanca; $^{(b)}$ Centre National de l'Energie des Sciences Techniques Nucleaires, Rabat; $^{(c)}$ Facult{\'e} des Sciences Semlalia, Universit{\'e} Cadi Ayyad, LPHEA-Marrakech; $^{(d)}$ Facult{\'e} des Sciences, Universit{\'e} Mohamed Premier and LPTPM, Oujda; $^{(e)}$ Facult{\'e} des sciences, Universit{\'e} Mohammed V-Agdal, Rabat, Morocco\\
$^{137}$ DSM/IRFU (Institut de Recherches sur les Lois Fondamentales de l'Univers), CEA Saclay (Commissariat {\`a} l'Energie Atomique et aux Energies Alternatives), Gif-sur-Yvette, France\\
$^{138}$ Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz CA, United States of America\\
$^{139}$ Department of Physics, University of Washington, Seattle WA, United States of America\\
$^{140}$ Department of Physics and Astronomy, University of Sheffield, Sheffield, United Kingdom\\
$^{141}$ Department of Physics, Shinshu University, Nagano, Japan\\
$^{142}$ Fachbereich Physik, Universit{\"a}t Siegen, Siegen, Germany\\
$^{143}$ Department of Physics, Simon Fraser University, Burnaby BC, Canada\\
$^{144}$ SLAC National Accelerator Laboratory, Stanford CA, United States of America\\
$^{145}$ $^{(a)}$ Faculty of Mathematics, Physics {\&} Informatics, Comenius University, Bratislava; $^{(b)}$ Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice, Slovak Republic\\
$^{146}$ $^{(a)}$ Department of Physics, University of Cape Town, Cape Town; $^{(b)}$ Department of Physics, University of Johannesburg, Johannesburg; $^{(c)}$ School of Physics, University of the Witwatersrand, Johannesburg, South Africa\\
$^{147}$ $^{(a)}$ Department of Physics, Stockholm University; $^{(b)}$ The Oskar Klein Centre, Stockholm, Sweden\\
$^{148}$ Physics Department, Royal Institute of Technology, Stockholm, Sweden\\
$^{149}$ Departments of Physics {\&} Astronomy and Chemistry, Stony Brook University, Stony Brook NY, United States of America\\
$^{150}$ Department of Physics and Astronomy, University of Sussex, Brighton, United Kingdom\\
$^{151}$ School of Physics, University of Sydney, Sydney, Australia\\
$^{152}$ Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{153}$ Department of Physics, Technion: Israel Institute of Technology, Haifa, Israel\\
$^{154}$ Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, Tel Aviv, Israel\\
$^{155}$ Department of Physics, Aristotle University of Thessaloniki, Thessaloniki, Greece\\
$^{156}$ International Center for Elementary Particle Physics and Department of Physics, The University of Tokyo, Tokyo, Japan\\
$^{157}$ Graduate School of Science and Technology, Tokyo Metropolitan University, Tokyo, Japan\\
$^{158}$ Department of Physics, Tokyo Institute of Technology, Tokyo, Japan\\
$^{159}$ Department of Physics, University of Toronto, Toronto ON, Canada\\
$^{160}$ $^{(a)}$ TRIUMF, Vancouver BC; $^{(b)}$ Department of Physics and Astronomy, York University, Toronto ON, Canada\\
$^{161}$ Faculty of Pure and Applied Sciences, University of Tsukuba, Tsukuba, Japan\\
$^{162}$ Department of Physics and Astronomy, Tufts University, Medford MA, United States of America\\
$^{163}$ Centro de Investigaciones, Universidad Antonio Narino, Bogota, Colombia\\
$^{164}$ Department of Physics and Astronomy, University of California Irvine, Irvine CA, United States of America\\
$^{165}$ $^{(a)}$ INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine; $^{(b)}$ ICTP, Trieste; $^{(c)}$ Dipartimento di Chimica, Fisica e Ambiente, Universit{\`a} di Udine, Udine, Italy\\
$^{166}$ Department of Physics, University of Illinois, Urbana IL, United States of America\\
$^{167}$ Department of Physics and Astronomy, University of Uppsala, Uppsala, Sweden\\
$^{168}$ Instituto de F{\'\i}sica Corpuscular (IFIC) and Departamento de F{\'\i}sica At{\'o}mica, Molecular y Nuclear and Departamento de Ingenier{\'\i}a Electr{\'o}nica and Instituto de Microelectr{\'o}nica de Barcelona (IMB-CNM), University of Valencia and CSIC, Valencia, Spain\\
$^{169}$ Department of Physics, University of British Columbia, Vancouver BC, Canada\\
$^{170}$ Department of Physics and Astronomy, University of Victoria, Victoria BC, Canada\\
$^{171}$ Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{172}$ Waseda University, Tokyo, Japan\\
$^{173}$ Department of Particle Physics, The Weizmann Institute of Science, Rehovot, Israel\\
$^{174}$ Department of Physics, University of Wisconsin, Madison WI, United States of America\\
$^{175}$ Fakult{\"a}t f{\"u}r Physik und Astronomie, Julius-Maximilians-Universit{\"a}t, W{\"u}rzburg, Germany\\
$^{176}$ Fachbereich C Physik, Bergische Universit{\"a}t Wuppertal, Wuppertal, Germany\\
$^{177}$ Department of Physics, Yale University, New Haven CT, United States of America\\
$^{178}$ Yerevan Physics Institute, Yerevan, Armenia\\
$^{179}$ Centre de Calcul de l'Institut National de Physique Nucl{\'e}aire et de Physique des Particules (IN2P3), Villeurbanne, France\\
$^{a}$ Also at Department of Physics, King's College London, London, United Kingdom\\
$^{b}$ Also at Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{c}$ Also at Novosibirsk State University, Novosibirsk, Russia\\
$^{d}$ Also at Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{e}$ Also at TRIUMF, Vancouver BC, Canada\\
$^{f}$ Also at Department of Physics, California State University, Fresno CA, United States of America\\
$^{g}$ Also at Department of Physics, University of Fribourg, Fribourg, Switzerland\\
$^{h}$ Also at Tomsk State University, Tomsk, Russia\\
$^{i}$ Also at CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{j}$ Also at Universit{\`a} di Napoli Parthenope, Napoli, Italy\\
$^{k}$ Also at Institute of Particle Physics (IPP), Canada\\
$^{l}$ Also at Department of Physics, St. Petersburg State Polytechnical University, St. Petersburg, Russia\\
$^{m}$ Also at Louisiana Tech University, Ruston LA, United States of America\\
$^{n}$ Also at Institucio Catalana de Recerca i Estudis Avancats, ICREA, Barcelona, Spain\\
$^{o}$ Also at Department of Physics, The University of Texas at Austin, Austin TX, United States of America\\
$^{p}$ Also at Institute of Theoretical Physics, Ilia State University, Tbilisi, Georgia\\
$^{q}$ Also at CERN, Geneva, Switzerland\\
$^{r}$ Also at Ochadai Academic Production, Ochanomizu University, Tokyo, Japan\\
$^{s}$ Also at Manhattan College, New York NY, United States of America\\
$^{t}$ Also at Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{u}$ Also at LAL, Universit{\'e} Paris-Sud and CNRS/IN2P3, Orsay, France\\
$^{v}$ Also at Academia Sinica Grid Computing, Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{w}$ Also at Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies, UPMC and Universit{\'e} Paris-Diderot and CNRS/IN2P3, Paris, France\\
$^{x}$ Also at School of Physical Sciences, National Institute of Science Education and Research, Bhubaneswar, India\\
$^{y}$ Also at Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, Roma, Italy\\
$^{z}$ Also at Moscow Institute of Physics and Technology State University, Dolgoprudny, Russia\\
$^{aa}$ Also at Section de Physique, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{ab}$ Also at International School for Advanced Studies (SISSA), Trieste, Italy\\
$^{ac}$ Also at Department of Physics and Astronomy, University of South Carolina, Columbia SC, United States of America\\
$^{ad}$ Also at School of Physics and Engineering, Sun Yat-sen University, Guangzhou, China\\
$^{ae}$ Also at Faculty of Physics, M.V.Lomonosov Moscow State University, Moscow, Russia\\
$^{af}$ Also at National Research Nuclear University MEPhI, Moscow, Russia\\
$^{ag}$ Also at Institute for Particle and Nuclear Physics, Wigner Research Centre for Physics, Budapest, Hungary\\
$^{ah}$ Also at Department of Physics, Oxford University, Oxford, United Kingdom\\
$^{ai}$ Also at Institut f{\"u}r Experimentalphysik, Universit{\"a}t Hamburg, Hamburg, Germany\\
$^{aj}$ Also at Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{ak}$ Also at Discipline of Physics, University of KwaZulu-Natal, Durban, South Africa\\
$^{al}$ Also at University of Malaya, Department of Physics, Kuala Lumpur, Malaysia\\
$^{*}$ Deceased
\end{flushleft}

% Created with ./xml2latex.py

==> mainWW_prd.tex <==


\section{Introduction}
The study of vector boson pair production at the Large
Hadron Collider (LHC) provides an important test of the electroweak 
sector of the Standard Model (SM) at the highest available energies.
Deviations  observed in the total or differential cross sections 
from the SM 
predictions may arise from anomalous triple gauge boson 
interactions~\cite{HISZ:1993} or from new particles decaying into 
vector bosons~\cite{Dixon:1999di}. Vector boson pair production is also an 
important source of background in studies of the Higgs boson and 
in searches for signals of physics beyond the SM. 

The cross sections for $WW$ and $WZ$ production at the LHC have previously 
been measured in fully leptonic 
final states~\cite{ATLAS:2012mec,Aad:2012twa,Chatrchyan:2013oev,Chatrchyan:2013yaa}. 
The semileptonic final states suffer from larger 
backgrounds from $W$ or $Z$ boson production in 
association with jets, but benefit from significantly larger branching fractions 
than the fully leptonic states 
and thus represent important complementary measurements. 
In this paper the $WW+WZ$ cross section is measured in the $\lvjj$ ($\ell=e,\mu$) final 
state using a data sample of proton--proton ($pp$) collisions with an 
integrated luminosity of  4.6 fb$^{-1}$ 
collected by the ATLAS detector at the LHC. 
In addition, the reconstructed dijet transverse momentum distribution is used to set limits 
on anomalous contributions to the 
triple gauge coupling vertices (aTGCs), after requiring that the dijet invariant 
mass is close to the mass of the $W$ or $Z$ boson.

The combined $WW+WZ$ production cross section (hereafter, $\WWWZ$ cross section, where $V=W,Z$)
has been measured in the $\lvjj$  
final state in proton--antiproton collisions at the Tevatron  collider by both the %
CDF~\cite{CDF:diboson} and D0~\cite{D0:diboson} collaborations, and 
more recently in $pp$ collisions by the CMS~\cite{Chatrchyan:2012bd} collaboration.  Limits on
anomalous triple gauge couplings in $\WVtolvjj$ production have also been presented
by CDF~\cite{Aaltonen:2007sd}, D0~\cite{Abazov:2012ze}, and CMS~\cite{Chatrchyan:2012bd}.

This paper is organised as follows. 
The overall analysis strategy is described in section~\ref{sec:AnalysisStrategy} and a short 
description of the ATLAS detector is given in section~\ref{sec:ATLASDetector}. 
The Monte Carlo (MC) simulation used for the signal and background modelling is summarized in section~\ref{sec:SimulatedSamples}. Details 
of the object and event reconstruction and of the event selection are given in 
sections~\ref{sec:Reconstruction} and~\ref{sec:EventSelection} respectively. 
The method to estimate the signal and background processes is discussed in section~\ref{sec:SigBkgEstimate}.
The cross section measurement is detailed in section~\ref{sec:xsecAndFitMethod}
and the systematic uncertainties are described in section~\ref{sec:sys}. The results of the 
cross-section measurement are summarized in section~\ref{sec:CrossSectionResults}, and 
the extraction of the anomalous triple gauge coupling limits is discussed in section~\ref{sec:atgc}. 
Finally, conclusions are drawn in section~\ref{sec:Conclusions}.

\section{Analysis strategy}\label{sec:AnalysisStrategy}
\input{AnalysisStrategy}
\section{The ATLAS detector}\label{sec:ATLASDetector}
 The ATLAS detector~\cite{atlas-det} is a general-purpose particle detector with cylindrical geometry\footnote{ATLAS uses a right-handed coordinate system with its origin at the nominal interaction point (IP) in the centre of the detector and the $z$-axis coinciding with the axis of the beam pipe. The $x$-axis points from the interaction point to the centre of the LHC ring,
and the $y$-axis points upward. Cylindrical coordinates $(r,\phi)$ are used in the transverse plane, $\phi$ being the azimuthal angle around
the beam pipe. The pseudorapidity $\eta$ is defined in terms of the polar angle $\theta$ as 
$\eta = - \ln [ \tan(\theta/2)]$.}  
 which consists of several sub-detectors surrounding the interaction point, and covering almost the full solid angle. The trajectories and momenta of charged particles 
are measured within the pseudorapidity region $|\eta|<$~2.5 by multi-layer silicon pixel and microstrip detectors and a transition radiation tracker. The tracking system is located in a superconducting solenoid producing a 2~T magnetic field and is surrounded by a high-granularity liquid-argon (LAr) sampling 
electromagnetic (EM) calorimeter with coverage up to $|\eta|=3.2$. The EM calorimeter is split into a barrel section ($|\eta|<1.475$) 
and endcaps ($1.375<|\eta|<3.2$).
A scintillating tile hadronic % 
calorimeter using steel as absorber provides coverage in the range $|\eta|<1.7$. In the forward region, LAr calorimeters 
provide electromagnetic and hadronic measurements and extend the coverage to $|\eta|<4.9$. 
The muon spectrometer surrounds the ATLAS calorimeter system and it operates in a toroidal magnetic field provided by air-core superconducting magnets and includes tracking chambers for precise muon momentum measurement up to $|\eta|=2.7$ and trigger chambers covering the range $|\eta|<2.4$. The online event selection is based on a three-level 
trigger system. The hardware-based Level-1 trigger uses a subset of the detector data to reduce the event rate from 20 MHz to below 75 kHz. Two subsequent software-level triggers further reduce the rate to about 300 Hz using the complete detector information.  
\section{Simulated event samples}\label{sec:SimulatedSamples}
\input{samples}

\section{Object and event reconstruction}\label{sec:Reconstruction}
\input{ObjectReco}

\section{Event selection}\label{sec:EventSelection}
\input{EventSelection}

\section{Signal and background estimation}
\label{sec:SigBkgEstimate}
\input{SigBkgEstimate}

\section{Cross-section definition and fit method}
\label{sec:xsecAndFitMethod}
\input{CrossSection_alt}

\section{\label{sec:atgc} Anomalous triple gauge couplings}
\input{AnomalousCouplings}


\clearpage
\section{Conclusion}\label{sec:Conclusions}
\input{theConclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> shortcuts.tex <==
%%----------------------------------
%
% all shortcuts go here
% this allows parallel compilation for JHEP and for ATLAS review in a single step
%
%%----------------------------------

%Spelling convention to follow:
%diboson (not di-boson)
%dijet  (not di-jet)
%maximum-likelihood
%cross section
%phase space


\def\alpgen{{\sc alpgen}}
\def\herwig{{\sc herwig}}
\def\jimmy{{\sc jimmy}}
\def\mcatnlo{{\sc mc@nlo}}
\def\pythia{{\sc pythia}}
\def\powheg{{\sc powheg}}
\def\acermc{{\sc acermc}}
\def\mcfm{{\sc mcfm}}
\def\madgraph{{\sc madgraph}}
\def\sherpa{{\sc sherpa}}
\def\toppp{{\sc top++2.0}}

\newcommand{\DR}{\ensuremath{\Delta R}}
\newcommand{\ourLumi}{\ensuremath{4.6 \pm 0.1~\mathrm{fb}^{-1}\xspace}}
\newcommand{\MT}{m_{\mathrm{T}}}
\newcommand{\Mjj}{m_{\mathrm{jj}}}
\newcommand{\pTjj}{\ensuremath{p_{{\rm T}jj}}}
\def\DRjj{\ensuremath{\Delta R(j_1,j_2)}}
\def\DEtajj{\ensuremath{\Delta\eta(j_1,j_2)}}
\newcommand{\Zjet}{Z+\mathrm{jets}}
\newcommand{\Wjet}{W+\mathrm{jets}}
\newcommand{\Vjet}{W/Z+\mathrm{jets}}
\def\lambdaz{\ensuremath{\lambda_Z}}
\def\lambdag{\ensuremath{\lambda_\gamma}}
\def\kz{\ensuremath{\kappa_Z}}
\def\kg{\ensuremath{\kappa_\gamma}}
\def\dkz{\ensuremath{\Delta\kz}}
\def\dkg{\ensuremath{\Delta\kg}}
\def\dkv{\ensuremath{\Delta\kappa_V}}
\def\gz{\ensuremath{g^Z_1}}
\def\dgz{\ensuremath{\Delta\gz}}
\def\dgg{\ensuremath{\Delta g^\gamma_1}}
\def\dgv{\ensuremath{\Delta g^V_1}}

\def\cwp{\ensuremath{c_W}}
\def\cbp{\ensuremath{c_B}}
\def\cwwwp{\ensuremath{c_{WWW}}}

\def\cwf{\ensuremath{\frac{\cwp}{\Lambda^2}}}
\def\cbf{\ensuremath{\frac{\cbp}{\Lambda^2}}}
\def\cwwwf{\ensuremath{\frac{\cwwwp}{\Lambda^2}}}

\def\cw{\ensuremath{\cwp/\Lambda^2}}
\def\cb{\ensuremath{\cbp/\Lambda^2}}
\def\cwww{\ensuremath{\cwwwp/\Lambda^2}}

\def\tevminSq{\ensuremath{\rm TeV^{-2}}}

\def\amp{\ensuremath{A}}
\def\Lumi{\ensuremath{\mathcal {L}}}
\def\BR{\ensuremath{\mathcal {B}}}
\def\lkl{\ensuremath{L}}
\def\BRWW{\ensuremath{\mathcal {B}^{WW}}}
\def\BRWZ{\ensuremath{\mathcal {B}^{WZ}}}
\def\sigmaWV{\ensuremath{\sigma(WW+WZ)}}
\def\lvjj{\ensuremath{\ell\nu \mathrm{jj}}}
\def\WVtolvjj{\ensuremath{WV \to \ell\nu \mathrm{jj}}}
\def\WWtolvjj{\ensuremath{WW \to \ell\nu \mathrm{jj}}}
\def\WZtolvjj{\ensuremath{WZ \to \ell\nu \mathrm{jj}}}
\def\WWtolvqq{\ensuremath{WW \to \ell\nu q \bar{q}^\prime}}
\def\WZtolvqq{\ensuremath{WZ \to \ell\nu q \bar q}}
\def\WWWZ{\ensuremath{WV}}
\def\ggWW{\ensuremath{ gg \to WW}}
\def\HWW{\ensuremath{ H \to WW}}

\def\WWtolvlv{\ensuremath{WW \to \ell\nu \ell\nu}}
\def\WZtolvll{\ensuremath{WZ \to \ell\nu \ell\ell}}


\def\Nmeas{\ensuremath{N^{WV}_{\ell}}}
\def\sigmafid{\ensuremath{\sigma_{\rm fid}}}
\def\sigmatot{\ensuremath{\sigma_{\rm tot}}}
\def\Dfid{\ensuremath{D_{\rm fid}}}
\def\Dtot{\ensuremath{D_{\rm tot}}}
\def\fWWfid{\ensuremath{f^{WW}_{\rm fid}}}
\def\fWWtot{\ensuremath{f^{WW}_{\rm tot}}}


\def\xSecWVresultfid{\ensuremath{1.37 \pm 0.14 \ \mathrm{(stat.)} \pm 0.37 \ \mathrm{(syst.) \ pb} } }
\def\xSecWVresulttot{\ensuremath{68 \pm 7 \ \mathrm{(stat.)} \pm 19 \ \mathrm{(syst.) \ pb} } }
\def\xSecWVpredictiontot{\ensuremath{61.1 \pm 2.2 \ \mathrm{pb} } }
\def\xSecWWpredictiontot{\ensuremath{43.7 \pm 1.9 \ \mathrm{pb} } }
\def\xSecWZpredictiontot{\ensuremath{17.4 \pm 1.1 \ \mathrm{pb} } }


\def\expectSignif{\ensuremath{3.2\sigma}}
\def\obsSignif{\ensuremath{3.4\sigma}}



==> systematics.tex <==
 
The total systematic uncertainties on the fiducial and total cross sections
are obtained by summing in quadrature the uncertainties on the signal 
yield, on the factors $\Dfid$ or $\Dtot$, and on the integrated luminosity.  

Systematic uncertainties that affect the fitted 
signal yield are accounted for by including nuisance parameters with Gaussian constraints in the
maximum-likelihood fit  (``profiled'' systematic uncertainties),  with a few
exceptions that are described below. 
The nuisance parameters describe the estimated rate or shape variations of the templates for the various processes.
Systematic uncertainties arising from the same 
source 
are assumed to be $100\%$ correlated between the electron and muon channels. 
Uncertainties from different sources are assumed to be independent. 



Two of the largest systematic uncertainties are the 
jet energy scale (JES) and jet energy resolution (JER)
uncertainties, determined
as described in refs.~\cite{Aad:2011he} and \cite{Aad:2012ag}. 
The JES uncertainty also includes the effect of energy deposits due to pile-up, 
and the uncertainties on the JES and JER are propagated to the $\MET$.
The main impact of the JES and JER uncertainties on the measurement of the 
signal yield is due to the
effect of these uncertainties on the shapes of the background distributions. 

The largest contribution to the background is from the production of 
a $W$ or $Z$ boson in association with jets; this background was modelled
using \alpgen.
Variations of the factorisation and 
normalisation scales are considered in evaluating the systematic uncertainty;
also, the parameters that describe the matching scheme 
in the matrix element to initial/final-state radiation (ISR/FSR) particles are varied. 
Alternative $\Vjet$ samples generated with \sherpa~\cite{Gleisberg:2008ta} were also analysed;
the $\Mjj$ and $\pTjj$ distributions from these samples are 
consistent with the \alpgen\ samples within the aforementioned \alpgen\
generator uncertainties, so no additional systematic uncertainty is assigned
for \alpgen-\sherpa\ differences.
The total rate uncertainty assigned to the $\Vjet$ processes is $20\%$ and it includes rate changes due to
cross-section, MC modelling, JES, and JER uncertainties.

The uncertainties on the modelling of the $\ttbar$ and single-top processes include 
shape and rate uncertainties due to variation of the ISR/FSR description. 
These are calculated with dedicated samples generated with \acermc. 
The total rate uncertainty assigned to the single-top and $\ttbar$ processes 
is $15\%$ and includes contributions from cross-section, MC modelling, 
JES, and JER uncertainties.

The multijet rate and shape uncertainties are determined by cross-checking 
the data-driven multijet estimation method in a multijet validation region 
with modified selection criteria:  $\met < 25 \gev$ and $\MT > 10 \gev$.
The uncertainty on the multijet rate is determined to be $15\%$.  Shape 
and rate uncertainties for the electron and muon channels are assumed 
to be uncorrelated. The shape uncertainties are described in the likelihood 
fit by means of two independent nuisance parameters, one for
the electron channel and one for the muon channel. 
The effect of the multijet rate uncertainty on the
extracted signal yield is estimated using pseudo-experiments as mentioned below.

The signal shape modelling uncertainty (including sources such as fragmentation, 
parton-shower, underlying-event and hadronisation modelling) 
is assessed by considering alternative templates obtained with samples produced with the \pythia\ 
generator. Varying the PDF is found to have a negligible impact 
on the shape of the $\Mjj$ and $\pTjj$ distributions.

Some uncertainties on the fitted signal yield were not described
through nuisance parameters, either in order to limit the 
number of parameters in the fit, or because of the difficulty of
fully parameterising the possible systematic variation in
terms of a nuisance parameter.
In such cases the impact of these uncertainties on the signal yield is estimated using 
an ensemble of pseudo-experiments.
These uncertainties include the multijet rate uncertainty and the 
uncertainty due to the size of the MC event samples.
The finite size of the MC event samples produces an uncertainty since it limits the precision with 
which the $\Mjj$ templates are known. This systematic uncertainty is one of the largest, and is
dominated by the size of the event sample for the $\Wjet$ process. 

The total uncertainty on the signal yield is obtained by summing contributions 
from the profiled and non-profiled sources in quadrature.

The fiducial and total cross sections are also affected by uncertainties on the values  
of $\Dfid$ and $\Dtot$, respectively. The following sources of 
uncertainty are considered for these factors: JES, JER, PDF, signal modelling (fragmentation, underlying-event, parton-shower, hadronisation, loss of spin-correlation information), 
lepton trigger and reconstruction efficiencies, and lepton energy scale. The largest 
contributions to the $\Dfid$ and $\Dtot$ uncertainties come from the JES and JER uncertainties while the 
uncertainties affecting the leptons give very small contributions. 

Table~\ref{tab:BreakDownSystematics} summarizes the percent contributions to the systematic 
uncertainties on the cross sections from the different sources. In the case of profiled systematic uncertainties, the contribution 
of each individual source to the total uncertainty on $\Nmeas$ is estimated by repeating 
the fit while fixing the nuisance parameter associated with the source under consideration to its best-fit value. 
The uncertainty on $\Nmeas$ from this modified fit is subtracted in quadrature from
the uncertainty on $\Nmeas$ given by the nominal fit, and the result is taken to be the
systematic uncertainty due to the source in question.
The data statistics uncertainty is calculated as the fit 
uncertainty on $\Nmeas$ when all nuisance parameters are fixed to their best-fit values.
The largest source of  uncertainty is the $\Vjet$ rate, dominated by the $\Wjet$ rate uncertainty.

\begin{table}
  \begin{center}
  \caption{Statistical and systematic 
uncertainties, in \%, on the measured fiducial and total cross sections. The uncertainties
are split according to the quantity ($\Nmeas, \Dfid, \Dtot$, \Lumi) they are affecting. } 
    \begin{tabular}{lcc}
      \hline \hline
     Source     & $\sigmafid$ & $\sigmatot$ \\
      \hline
& \multicolumn{2}{c}{$\Nmeas$}\\
\hline
Data statistics& \multicolumn{2}{c}{$\pm 10$}\\
\hline
MC statistics &\multicolumn{2}{c}{$\pm 12$}\\
$\Vjet$ rate and shape modelling & \multicolumn{2}{c}{$\pm $17} \\
Multijet shape and rate & \multicolumn{2}{c}{$\pm $8}\\
Top rate and initial/final-state radiation shape modelling &\multicolumn{2}{c}{$\pm $6}\\
Jet energy scale (background and signal shapes) & \multicolumn{2}{c}{$\pm $9} \\
Jet energy resolution (background and signal shapes) &\multicolumn{2}{c}{$\pm $11}\\
$\WWWZ$ shape modelling &\multicolumn{2}{c}{$\pm $5}\\
\hline
& $\Dfid$ & $\Dtot$ \\
\hline
JES/JER uncertainty & $\pm $6 & $\pm $6\\
Signal modelling &$\pm $4 & $\pm $5 \\
Jet veto scale dependence & - & $\pm $5 \\
Others (loss of spin-corr information, lepton uncertainties, PDF)  &$\pm $1 & $\pm $4 \\
\hline 
Luminosity & \multicolumn{2}{c}{$\pm 1.8$} \\
\hline
Total systematic uncertainty & $\pm 27 $ & $\pm 28$ \\
      \hline \hline

    \end{tabular}
 \label{tab:BreakDownSystematics}
  \end{center}
\end{table}



==> theAbstract.tex <==

The production of a $W$ boson decaying to $e\nu$ or $\mu\nu$ 
in association with a $W$ or $Z$ boson
decaying to two jets is studied using $4.6~\mathrm{fb}^{-1}$ of proton--proton 
collision data at $\sqrt{\rm{s}} = 7$ TeV recorded with the ATLAS 
detector at the LHC.  The combined $WW+WZ$ cross section is measured 
with a significance of 3.4$\sigma$ and 
is found to be $68 \pm 7 \ \mathrm{(stat.)} \pm 19 \ \mathrm{(syst.)} \ pb$,
in agreement with the Standard Model expectation of  $61.1 \pm 2.2 \ \mathrm{pb}$.
The distribution of the transverse momentum of the dijet system is
used to set limits on anomalous contributions to the triple gauge coupling vertices and
on parameters of an effective-field-theory model.



==> theConclusion.tex <==
A measurement of the $pp\to WV$ cross section ($V=W,Z$) 
at $\rts = 7$ TeV is performed with $\ourLumi$ of data 
collected by ATLAS at the LHC, using the $\WVtolvjj$ ($\ell$=e,$\mu$) decay channels. The total $WW+WZ$ 
cross section is measured to be $\sigmaWV = \xSecWVresulttot$, where the observed significance
of the signal is $\obsSignif$.  This measurement is consistent with the \mcatnlo\ cross-section prediction
of $\xSecWVpredictiontot$.   In addition, a fiducial cross section is measured in a phase space
corresponding closely to the event selection used in the analysis, and is found to be
$\sigmafid = \xSecWVresultfid$.

The same process is also used to place limits on anomalous triple gauge couplings
(aTGCs) and on the coefficients of dimension-6 operators of an effective-field-theory.
Within the LEP scenario, the observed $95 \%$~CL limits on the anomalous triple gauge parameters are 
$-0.039 < \lambda < 0.040$, $ -0.21 < \dkg < 0.22$, and $-0.055 < \dgz < 0.071$.   
The limits on anomalous couplings are similar to those 
obtained by other diboson analyses.





==> title.tex <==

Measurement of the $WW+WZ$ cross section and limits on anomalous triple gauge couplings
using final states with
one lepton, missing transverse momentum, and two jets with the ATLAS detector 
at $\sqrt{\rm{s}} = 7$ TeV 


